Local Certification of Vertex and Edge Connectivity

Local certification is a framework for verifying global graph properties using only local information. In this model, a prover assigns short labels, called certificates, to the vertices of a graph. Each vertex then exchanges certificates with its neighbors and performs a purely local check to determine whether the graph satisfies the desired property. This line of research has led to efficient certification schemes for a broad range of graph classes, including minor-closed families, topological graph classes, and graphs defined by forbidden subgraphs. In this paper, we study the local certification of graph connectivity. Prior work by Bousquet, Feuilloley, and Pierron (JPDC 2024) showed that $2$-vertex-connectivity, $2$-edge-connectivity, and $3$-vertex-connectivity admit $O(\log n)$-bit certificates, leveraging structural characterizations such as ear decompositions. We go substantially beyond these cases and investigate general $k$-vertex-connectivity and $k$-edge-connectivity. We develop new approaches that exploit connections between connectivity and combinatorial structures, including branchings, Eulerian subgraphs, and independent spanning trees. For $k$-edge-connectivity, we obtain an $O_k(\log n)$-bit certification scheme and prove a matching $\Omega_k(\log n)$ lower bound for every $k\ge 3$. The lower bound also applies to $k$-vertex-connectivity. For $k$-vertex-connectivity, we obtain $\tilde{O}_k(\sqrt{n})$-bit certificates for every $k$ under a conjecture of Itai and Zehavi. We further show that, for $k=2$, the logarithmic barrier can be broken on sparse graph classes: $2$-edge-connectivity admits constant-size certificates in bounded-expansion graphs, and $2$-vertex-connectivity admits constant-size certificates in bounded-degree graphs. In contrast, for $2$-vertex-connectivity in general graphs, we prove an $\Omega(\log(\log^\ast n))$-bit lower bound.

==> 2-conn_backup.tex <==
\section{Constant-bit certification for $2$-connectivity on bounded degree graphs}\label{sec: 2-conn-bdd-deg}
In this section, we show that certifying both $2$-edge-connectivity and $2$-vertex connectivity can be done in constant bits on bounded degree graphs. %\mtt{We presume that the input graph $G$ is connected. }\yijun{I think it's standard assumption in this area, and it also doesn't make sense to consider disconnected graphs for local certification. If unclear, can say it explicitly in intro/prelim.}\yx{I add it in the prel}

\subsection{$2$-edge-connectivity}
It is known that the edges of a bridgeless graph can be covered by three (possibly disconnected) Eulerian subgraphs.
\begin{lemma}[\cite{AT85}]\label{lem: Eulerian-cover}
    An undirected graph $G$ is $2$-edge-connected if and only if its edge set $E(G)$ can be covered by three (possibly disconnected) Eulerian subgraphs $(V(G),C_i)$ for $i \in [3]$; that is, $C_1 \cup C_2 \cup C_3 = E(G)$.
    %For any $2$-edge-connected graph $G$, there exist $3$ Eulerian subgraphs $C_1,C_2,C_3$ such that $E(G)=E(C_1)\cup E(C_2)\cup E(C_3)$.
\end{lemma}

Using this Eulerian subgraph covering, we have an $O(\Delta^2)$-bit edge-certification for $2$-edge-connectivity.
\thmTwoEC*
%\begin{theorem}\label{thm: 2-edge-conn}
    %There exists an $O(\Delta^2)$-bit local certification scheme for $2$-edge-connectivity on bounded-degree graphs.
%\end{theorem}
\begin{proof}
    For each $i\in[3]$, color all the edges in $C_i$ with color $i$. Each vertex then checks that ($1.$) for each color $i\in[3]$, the number of incident edges that are colored $i$ is even, and ($2.$) every edge is colored by at least a color in $[3]$.

    According to \Cref{lem: edge-cert-bdd-deg}, we can transform this $O(1)$-bit edge-certification scheme to an $O(\Delta^2)$-bit vertex certification scheme.
\end{proof}


\subsection{$2$-vertex-connectivity}
We show that $2$-vertex-connectivity can be certified with $O(1)$ bits on bounded degree graphs via a reduction to $2$-edge-connectivity. 
\thmTwoVC*
%\begin{theorem}\label{thm: 2-vertex-conn}
    %There exists an $O(\Delta^2\cdot 2^{\Delta})$-bit local certification scheme for $2$-vertex-connectivity on bounded-degree graphs.
%\end{theorem}

The intuition is to transform the graph $G$ into a set of graphs by making the vertices of $G$ into edges and reconnecting with its neighborhood in a way such that $G$ is $2$-vertex-connected if and only if all the transformed graphs are $2$-edge-connected.

\paragraph{Transforming a $2$-vertex-connected graph into a $2$-edge-connected graph}
Given a $2$-vertex-connected graph $G=(V,E)$, we construct a graph $G'=(V',E')$ by the following operation:
\begin{itemize}
    \item For each vertex $v\in G$, make it into a super vertex $\psi(v)=\{v_0,v_1\}$. Add the vertices $v_0,v_1$ to $V'$, and add an edge $\{v_0,v_1\}$ to $E'$.
    \item For each vertex $v\in G$, partition $N(v)$, the neighborhood of $v$, into two non-empty subsets $N_0(v),N_1(v)$.
    \item For each pair of vertices $\{u,v\}\in E$ and $i,j\in\{0,1\}$, add an edge $\{u_i,v_j\}$ to $E'$ if and only if $v\in N_i(u)$ and $u\in N_j(v)$.
\end{itemize}

According to the rules of how we construct $G'$, we have the following observation:
\begin{observation}\label{obs: 2-ve-to-2-ec}
    For each pair of vertices $u,v\in G$, $\{u,v\}\in E$ if and only if there exists some edge $\{u_i,v_j\}\in E'$ between $\psi(u)$ and $\psi(v)$.
\end{observation}

We claim that if the original graph $G$ is $2$-vertex-connected, then the resulting graph $G'$ is $2$-edge-connected.
\begin{claim}\label{claim: 2-conn-1}
    If $G$ is $2$-vertex-connected, then $G'$ is $2$-edge-connected.
\end{claim}
\begin{proof}
    Suppose that $G'$ is not $2$-edge-connected, then there exists a bridge $e=\{x,y\}\in E'$ that splits the graph into two connected components $X$ and $Y$ where $x\in X,y\in Y$. Suppose that $x\in \psi(u)$ and $y\in \psi(v)$ for some $u,v\in V$, then for each $w\in V$, $w\not\in\{u,v\}$ the two vertices in $\psi(w)\subseteq V'$ must belong to the same side of the cut $(X,Y)$. Let $S=\{s\in V:\psi(s)\subseteq X\}$ and $T=\{t\in V:\psi(t)\subseteq Y\}$. If $u\neq v$, then according to \Cref{obs: 2-ve-to-2-ec}, there is no edge between $S\cup\{u\}$ and $T\cup\{v\}$ except for $\{u,v\}$. Then removing either $u$ or $v$ will disconnect the graph. Otherwise, $u=v$ and $x=u_0,y=u_1$, then there is no edge between $S$ and $T$. Note that in this case, $S$ and $T$ will be non-empty since we have partitioned $N(u)$ into two non-empty sets. Thus, removing $u$ will disconnect the graph. In both cases, we arrive at a contradiction to the fact that $G$ is $2$-vertex-connected. 
\end{proof}

\begin{claim}\label{claim: 2-conn-2}
    If $G$ has a vertex cut $\{v\}$, then there exists a partition of $N(v)$ such that $\{v_0,v_1\}$ is a bridge in $G'$, no matter how we partition the neighborhoods of other vertices.
\end{claim}
\begin{proof}
    Let $S,T\subseteq V$ be two vertex sets that are disconnected after removing $v$ from $G$. Let $N_0(v)=N(v)\cap S$ and $N_1(v)=N(v)\cap T$. Then $\{v_0,v_1\}$ is a bridge in $G'$.
\end{proof}

\begin{proof}[Proof of \Cref{thm: 2-vertex-conn}]
    Let $G=(V,E)$ be a graph of maximum degree $\Delta$. Then for each $v\in V$, there exist at most $2^{\deg(v)-1}-1\leq 2^{\Delta-1}-1$ ways of partitioning $N(v)$. Let $t(v)=2^{\deg(v)-1}-1$, and $t=2^{\Delta-1}-1$. Let the set of partitions be $\Gamma(v)=\{\Gamma^i(v)\}_{i=1}^{t}$, where $\Gamma^i=\{N_0^i(v),N_1^i(v)\}$, $\Gamma^i(v)\neq\Gamma^j(v)$ for every $1\leq i<j\leq t(v)$ and $\Gamma^i(v)=\Gamma^{t(v)}(v)$ for all $t(v)\leq i\leq t$.

    For each $i\in[t]$, we construct a graph $G_i$ using the partition $\Gamma^i(v)$ for every vertex $v\in G$. According to \Cref{claim: 2-conn-1,claim: 2-conn-2}, if $G$ is $2$-vertex-connected, all $\{G_i\}_{i=1}^t$ are $2$-edge-connected. Otherwise, there exists some $G_{i^*},i^*\in[t]$ such that $G_{i^*}$ has a bridge. Therefore, it suffices to simulate the certification of $2$-edge-connectivity simultaneously for each $G_i$. Our certification scheme is as follows:
    \begin{itemize}
        \item For each $v\in V$, assign the list of partitions $\Gamma(v)=\{\Gamma^i(v)\}_{i=1}^t$ to $v$. Each of the partitions can be stored in $O(1)$ bits by first doing a $2$-hop coloring on $V$, and then encoding the partition of $N(v)$ by a partition of the colors in $N(v)$. 
        \item For each $i\in[t]$, let $c_i$ be the certificate assignment for $2$-edge-connectivity when the underlying graph is $G_i$. For each $v\in V$, assign $v$ the list of certificates $\{(c_i(v_0),c_i(v_1))\}_{i=1}^t$.
        \item Each vertex $v\in V$ runs the following verification algorithm:
        \begin{itemize}
            \item First check that the $2$-hop coloring (for encoding the partition) is proper, this can be done by having each vertex check that no color appears twice in their neighborhood. Then check that the set of partitions $\Gamma(v)$ indeed contains all possible partitions of its neighborhood, which can be done with the knowledge of its neighborhood in the original graph.
            \item For each $i\in[t]$, each vertex $v\in V$ has the knowledge of the local graph topology of $G_i$ by looking at the partition of its neighbors and itself. Therefore, it can simulate the verification algorithm of $v_0$ and $v_1$ on $G_i$ with the certificates $\{(c_i(v_0),c_i(v_1))\}$. If the verification fails for some $i$, it outputs \reject. Otherwise, it outputs \accept.
        \end{itemize}
    \end{itemize}
    The correctness of this certification scheme follows from the correctness of certifying $2$-edge-connectivity on bounded-degree graphs. The size of the certificates blows up by a factor of $O(t)=O(2^{\Delta})$, which gives us the size bound of certificates.
\end{proof}

%\subsection{Discussion}
%We have shown in \Cref{sec: lower} that the lower-bound graph for distinguishing $2$-edge/vertex-connectivity and $k$-edge/vertex-connectivity is of bounded degree ($k$). However, in this section, we see that distinguishing $2$-edge/vertex-connectivity on bounded-degree graphs is easy (has a constant-bit certification scheme). Is it true that certifying $2$-connectivity can be done in $O(1)$ bits? Or is it the case that there exists a lower bound, and the hard instance is of unbounded degree?\yijun{move to intro or conclusion}



==> 2-conn_bdd-deg.tex <==
\section{Constant-bit certification for $2$-connectivity on bounded degree graphs}\label{sec: 2-conn-bdd-deg}
In this section, we show that certifying both $2$-edge-connectivity and $2$-vertex connectivity can be done in $O(1)$ bits on bounded degree graphs.

\subsection{$2$-edge-connectivity}
It is known that the edges of a bridgeless graph can be covered by $3$ Eulerian subgraphs.
\begin{lemma}\cite{AT85}\label{lem: Eulerian-cover}
    For any $2$-edge-connected graph $G$, there exists $3$ Eulerian subgraphs $C_1,C_2,C_3$ such that $E(G)=E(C_1)\cup E(C_2)\cup E(C_3)$.
    %\yijun{\cite{Cha09} is informal, and I could not find the claim in \cite{BJJ83}. Suggest cite~\cite[Lemma 4.1]{alon1985covering} }
\end{lemma}

Using this Eulerian subgraph covering, we have an $O(1)$-bit edge-certification for $2$-edge-connectivity: For each $i\in[3]$, color all the edges in $C_i$ with color $i$. Each vertex then checks that ($1.$) for each color $i\in[3]$, the number of incident edges that are colored $i$ is even, and ($2.$) every edge is colored by at least a color in $[3]$.

According to \Cref{lem: edge-cert-bdd-deg}, we can transform this $O(1)$-bit edge-certification scheme to an $O(1)$-bit (vertex-) certification scheme.\yijun{Turn the above into a proof right below the theorem statement in latex proof environment.} Therefore, we have the following Theorem.
\begin{theorem}\label{thm: 2-edge-conn}
    There exists an $O(1)$-bit local certification scheme for $2$-edge-connectivity on bounded-degree graphs.
\end{theorem}

\subsection{$2$-vertex-connectivity}
We show that $2$-vertex-connectivity can be certified with $O(1)$ bits on constant degree graphs via a reduction to $2$-edge-connectivity. 
\begin{theorem}\label{thm: 2-vertex-conn}
    There exists an $O(1)$-bit local certification scheme for $2$-vertex-connectivity on bounded-degree graphs.
\end{theorem}

The intuition is to transform the graph $G$ into a set of graphs by making the vertices of $G$ into edges and reconnect with its neighborhood in a way such that $G$ is $2$-vertex-connected if and only if all the transformed graphs are $2$-edge-connected.

\paragraph{Transforming a $2$-vertex-connected graph into a $2$-edge-connected graph}
Given a $2$-vertex-connected graph $G=(V,E)$, we construct a graph $G'=(V',E')$ by the following operation:
\begin{itemize}
    \item For each vertex $v\in G$, make it into a super vertex $\psi(v)=\{v_0,v_1\}$. Add the vertices $v_0,v_1$ to $V'$, and add an edge $\{v_0,v_1\}$ to $E'$.
    \item For each vertex $v\in G$, partition $N(v)$, the neighborhood of $v$, into two non-empty subsets $N_0(v),N_1(v)$.
    \item For each pair of vertices $\{u,v\}\in E$ and $i,j\in\{0,1\}$, add an edge $\{u_i,v_j\}$ to $E'$ if and only if $v\in N_i(u)$ and $u\in N_j(v)$.
\end{itemize}
We claim that if the original graph $G$ is $2$-vertex-connected, then the resulting graph $G'$ is $2$-edge-connected.
\begin{claim}\label{claim: 2-conn-1}
    If $G$ is $2$-vertex-connected, then $G'$ is $2$-edge-connected.
\end{claim}
\begin{proof}
    According to the rules of how we construct $G'$, we have the following observation:\yijun{do not put a formal observation/claim/lemma inside a proof.}
    \begin{observation}\label{obs: 2-ve-to-2-ec}
        For each pair of vertices $u,v\in G$, $\{u,v\}\in E$ if and only if there exists some edge $\{u_i,v_j\}\in E'$ between $\psi(u)$ and $\psi(v)$.
    \end{observation}
    Suppose that $G'$ is not $2$-edge-connected, then there exists a bridge $e=\{x,y\}\in E'$ that splits the graph into two connected components $X$ and $Y$ where $x\in X,y\in Y$. Suppose that $x\in \psi(u)$ and $y\in \psi(v)$ for some $u,v\in V$, then for each $w\in V$, $w\not\in\{u,v\}$, the two vertices in $\psi(w)\subseteq V'$ must belong to the same side of the cut $(X,Y)$. Let $S=\{s\in V:\psi(s)\subseteq X\}$ and $T=\{t\in V:\psi(t)\subseteq Y\}$. If $u\neq v$, then according to \Cref{obs: 2-ve-to-2-ec}, there is no edge between $S\cup\{u\}$ and $T\cup\{v\}$ except for $\{u,v\}$. Then removing either $u$ or $v$ will disconnect the graph. Otherwise, $u=v$ and $x=u_0,y=u_1$, then there is no edge between $S$ and $T$. Note that in this case, $S$ and $T$ will be non-empty since we have partitioned $N(u)$ into two non-empty sets. Thus, removing $u$ will disconnect the graph. In both cases, we arrive at a contradiction to the fact that $G$ is $2$-vertex-connected. 
\end{proof}

\begin{claim}\label{claim: 2-conn-2}
    If $G$ has a vertex cut $\{v\}$, then there exists a partition of $N(v)$ such that $\{v_0,v_1\}$ is a bridge in $G'$, no matter how we partition the neighborhoods of other vertices.
\end{claim}
\begin{proof}
    Let $S,T\subseteq V$ be two vertex sets that are disconnected after removing $v$ from $G$. Let $N_0(v)=N(v)\cap S$ and $N_1(v)=N(v)\cap T$. Then $\{v_0,v_1\}$ is a bridge in $G'$.
\end{proof}


\begin{proof}[Proof of \Cref{thm: 2-vertex-conn}] aaa
 \paragraph{Local certification scheme for $2$-vertex-connectivity}\yijun{turn the discussion below into a formal ``Proof of \Cref{thm: 2-vertex-conn}'' in the latex proof environment}
Let $G=(V,E)$ be a graph of maximum degree $\Delta$. Then for each $v\in V$, there exists at most $2^{\deg(v)-1}-1\leq 2^{\Delta-1}-1$ ways of partitioning $N(v)$. Let $t(v)=2^{\deg(v)-1}-1$, and $t=2^{\Delta-1}-1$. Let the set of partitions be $\Gamma(v)=\{\Gamma^i(v)\}_{i=1}^{t}$, where $\Gamma^i=\{N_0^i(v),N_1^i(v)\}$, $\Gamma^i(v)\neq\Gamma^j(v)$ for every $1\leq i<j\leq t(v)$ and $\Gamma^i(v)=\Gamma^{t(v)}(v)$ for all $t(v)\leq i\leq t$.

For each $i\in[t]$, we construct a graph $G_i$ using the partition $\Gamma^i(v)$ for every vertex $v\in G$. According to \Cref{claim: 2-conn-1} and \Cref{claim: 2-conn-2}, if $G$ is $2$-vertex-connected, all $\{G_i\}_{i=1}^t$ are $2$-edge-connected. Otherwise, there exists some $G_{i^*},i^*\in[t]$ such that $G_{i^*}$ has a bridge. Therefore, it suffices to simulate the certification of $2$-edge-connectivity simultaneously for each $G_i$. Our certification scheme is as follows:
\begin{itemize}
    \item For each $v\in V$, assign the list of partitions $\Gamma(v)=\{\Gamma^i(v)\}_{i=1}^t$ to $v$. This can be done in $O(1)$ bits by first doing a $2$-hop coloring on $V$, and then encode the partitions of $N(v)$ by a partitions of the colors in $N(v)$. 
    \item For each $i\in[t]$, let $c_i$ be the certificate assignment for $2$-edge-connectivity when the underlying graph is $G_i$. For each $v\in V$, assign $v$ the list of certificates $\{(c_i(v_0),c_i(v_1))\}_{i=1}^t$.
    \item Each vertex $v\in V$ runs the following verification algorithm:
    \begin{itemize}
        \item Check that the set of partitions $\Gamma(v)$ indeed contains all possible partitions of its neighborhood, which can be done with the knowledge of its neighborhood in the original graph.\yijun{+check if the 2-hop coloring is proper?}
        \item For each $i\in[t]$, each vertex $v\in  V$ has the knowledge of the local graph topology of $G_i$ by looking at the partition of its neighbors and itself. Therefore, it can simulate the verification algorithm of $v_0$ and $v_1$ on $G_i$ with the certificates $\{(c_i(v_0),c_i(v_1))\}$. If the verification fails for some $i$, it outputs \reject. Otherwise, it outputs \accept.
    \end{itemize}
\end{itemize}
The correctness of this certification scheme follows from the correctness of certifying $2$-edge-connectivity on bounded-degree graphs. The size of the certificates blows up by a factor of $O(t)$, which is still a constant since $t$ is a constant on bounded-degree graphs.\yijun{can write down the dependence on $\Delta$ in the theorem -- it will be a good open problem for future work to improve it.}
\end{proof}





\subsection{Discussion}
We have shown in \Cref{sec: lower} that the lower-bound graph for distinguishing $2$-edge/vertex-connectivity and $k$-edge/vertex-connectivity is of bounded degree ($k$). However, in this section, we see that distinguishing $2$-edge/vertex-connectivity on bounded-degree graphs is easy (has a constant-bit certification scheme). Is it true that certifying $2$-connectivity can be done in $O(1)$ bits? Or is it the case that there exists a lower bound, and the hard instance is of unbounded degree?

==> PODC-review <==
PODC 2026 Paper #316 Reviews and Comments
===========================================================================
Paper #316 Local Certification of Vertex and Edge Connectivity


Review #316A
===========================================================================

Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This work studies distributed certification of edge and vertex connectivity. The studied model is one of the two standard models in this field, the proof labelling schemes. The goal is to give a distributed proof of some graph property (like k-edge connectivity) that can be verified locally by each node of the graph. The prover assigns a proof label to each node. Each node looks at all the information in its neighbourhood (1 hop) and either accepts or reject based on another algorithm called the verifier. We want a scheme such that 1) for yes-instances there exists a proof that makes all nodes accept, and 2) for no-instances no proof makes all nodes accept. The complexity measure is the number of bits per node in the proof.

Connectivity has been studied in this context before, and it is known that certifying 2-edge connectivity, 2-vertex connectivity, and 3-vertex connectivity can be done with proofs of size O(log n). The main results of present work expand these results to general k-connectivity:
- For k >= 3, both k-edge connectivity and k-vertex connectivity require Omega((log n) / k )-bit proofs.
- For k >= 2, k-edge connectivity can be certified with proofs of size O(k log n) when k is even and of size O(81^(k^2) k log n) when k is odd.
- For k in {1,2,3,4} the k-vertex connectivity can be certified with proofs of size O(k^3 n^(1/2) log^2.5 n). Assuming a conjecture called Itai-Zehavi conjecture about a connection between k-vertex connectivity and the ability to span the graph with k independent spanning trees at any vertex, this result is extended to any k.
- Certain certification task related to independence of spanning trees requires Omega(n^(1/2)) bits of proof, indicating that the current approach is difficult to improve.

For restricted graph classes it is also shown that:
- 2-edge connectivity can be certified with O(Delta^2) bits in bounded-degree graphs.
- 2-vertex connectivity can be certified with O(Delta^2 2^Delta) bits by a reduction to the edge connectivity case.
- The complexity of certifying k-connectivity (both types) in planar graphs is Theta(log n).

These results extend previous work both in terms on new results and new techniques. The scheme for edge connectivity for even k is based on a classic result guaranteeing the existence of a strongly (k/2)-connected orientation iff the graph is k-connected. The odd case is based on another characterisation which gives the constant 81^(k^2) that apparently could be improved to 2^O(k). The lower bound is based on a standard counting argument used to glue together a no-instance where a proof is accepted.

The problem of k-connectivity is obviously a classic problem and present work extends the state of the art in distributed certification. Based on my understanding, the value of the results is based on the statements themselves and there is no particular hope that the techniques could be applied to anything else. Generally, the novelty of the paper seems modest. It is unfortunate that there is still such a gap between the upper and lower bounds for vertex connectivity. While the writeup is decent, I think the techniques used for the certification schemes should have been explained in more detail in the first 10 pages.

Comments for authors
--------------------
Generally I would suggest considering how to best highlight your results in the first 10 pages, as instructed by the call. Specifically, I don't think the lower bound starting on page 9 is the most exciting content you could have highlighted. Similarly on page 7 you have a very standard scheme to certify spanning trees, a definition out of context, and the definition of spanning tree independence. Instead of this content I would have wanted e.g. an extended Section 1.1.1.

[todo*?]


- p.6: You mention that your lower bounds work for LCPs before defining LCPs in the next paragraph.

[todo?]
[yx: I changed the order of two paragraphs]

- p.7: it is not clear here what the edge certification model is? Edges don't have identifiers.

[todo?]
[yx: added some explanation]
[mt: It may be good to point out only the differences between the proof-labeling scheme and the edge certification scheme. I have added a paragraph, highlighted in red around Lines 284--287.]

Review #316B
===========================================================================

Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
4. Expert

Paper summary
-------------
*Summary*

The paper is about local certification, a setting where a prover assigns 
(hopefully) small labels (=certificates) to the node a network to convince them 
that a property holds. The nodes can check these labels: they look at their 
neighborhoods, and output whether the certification looks convincing or not. 
All nodes should be convinced iff the property holds. 

There has been intense research in this area to establish what are the optimal 
certificate size for natural graph properties, such as planarity. 
Vertex and edge connectivity are natural properties that have not been well 
studied: only one paper proved O(log n) bounds for 2-(and 3)-vertex and 2-edge
connectivity, as a by-product of another result about forbidden minors. 

This paper establishes the following results:

* A Omega(log n/k) lower bound for k-vertex and k-edge connectivity (with an 
hidden dependency in k).

* A O(f(k)log n) upper bound for k-vertex connectivity

* A conditional O(sqrt(n)) for k-edge connectivity, and a lower bound showing 
that, for this technique, sqrt(n) is optimal

* A O(f(Delta)) upper bound for k-vertexoredge-connectivity in bounded degree 
graphs. 

* A tight Theta(log n) bound for both connectivity in planar graphs. 

The techniques are very varied, using all kind of tools from centralized computing
and combinatorics, and adapting them in non-trivial ways (especially for the 
planar result) to local certification. 

*Strength*

* The problem studied is very natural, and the paper fills a gap in the study 
of local certification. 

* The results are tight in n, or at least tight for the techniques used. 

* The paper brings many new tools in the area of local certification, and opens 
many interesting open directions, and we can certainly expect follow-ups. 

*Weaknesses*

* The introduction does not present a good overview of the techniques: the tools 
are only mentioned, the challenges are not discussed. I believe that using the 
10 first pages to give a deep sketch into the techniques would be much better. 

* The paper does not present properly how important this is. It sometimes make it
sound like "this was not known, so we study it", while I think it is a very 
interesting topic.

Comments for authors
--------------------
*General comments*

* I would suggest to use the format where the introduction is ~10 pages and
contains all the useful intuitions + the open questions. 

[todo*?]


* To follow up on weakness 1, you cannot assume that people are familiar with 
arc-strong-connectivity, branchings, independent spanning trees, heavy-light 
decomposition, bridgeless graphs, certification on edges, separating cycles, etc. 
You have space, just explain what these are, add figures. You do not even define 
connectivity! 

[todo*?]
[yx: Im not sure whether to keep the current paragraph, add some brief explanation, and give formal definition in prelim; or to add one background paragraph to define all these things before the technical overview.]

* To follow-up on weakness 2, you should sell the paper better. For example:
- explain why for the forbidden minors conjecture connectivity is key

[todo?]
[yx: I try to motivate this paper first by saying that connectivity is a fundamental problem, and say that it has been used in the minor-closed certification problem. Im not sure whether itis better or not.]

- explain why we are interested in the log n regime, and discuss how the line
of work on meta-theorems (does not) help with connectivity. 

[todo*?]

- discuss the dependency in Delta: this is a fairly new topic, few papers care 
about Delta as a parameter. 

[todo?]
[yx: I cite one prior work that considers \Delta as a parameter and add a paragraph at the beginning of Sec 1.2]

- Also the dependency in k is quite fascinating. 

[todo*?]

- Also justify that certifying things in planar graphs (instead of only caring 
about general graphs) is interesting (the series of papers about metatheorems, 
the STACS paper with its result on matching in planar graphs, the CONGEST/LOCAL
papers in this setting, etc.). 

[todo*?]


*Specific comments*

Page 1

* EL22 should also be cited for bounded genus/planar

[todo?]
[yx: edited]

Page 2

* "bounded neighborhood, then we consider Theta(n) such instances" not clear

[todo?]
[yx: edited, marked in red]

* "devise" > sketch? 

[todo*?]

* 1.1.1: introduce the subsection

[todo*?]

* As said earlier, the paragraph about branchings et al assumes too much knowledge
from the readers. 

[todo*?]

* Independent spanning trees: use a figure. Also, compare with edge-disjoint 
spanning trees. 

[todo?]
[yx: added a figure and explained in the caption. However not sure whether to also give a formal definition in sec2 and put this figure there]

* "We note that [...]" why? (Not clear at that point whether it is trivial or not)

[todo*?]
[yx: should we make it a lemma after conjecture 2.5? and refer to that lemma here.]

* 24 > why that number? 

[todo*?]
[yx: i guess is (4 choose 2)=6? or do you count all 4 roots?]

page 3

* heavy-light decomposition should be defined and illustrated. 

[todo?]
[yx: briefly explain what heavy-light decomp is when using it, marked in red. Added a figure and explained in the caption. However not sure whether to put it in prelim after giving formal definitions]

* Theorem 5: compare with BFP24

[todo?]
[yx: added to the paragraph before theorem 5, marked in red]

* I didn't get the paragraph after Theorem 5

[todo?]
[yx: edited]

Page 4

* The order of the theorems in 1.3 is strange: you discuss the upper bound and 
then have the theorem of the lower bound. 

[todo?]
[yx: not sure whether to state the planar graph lower bound also in theorem 1 and refer to it here?]

* "and _all_ deleting"

[todo*?]

* The discussion after Theorem 8 is too sketchy to be useful. 

[todo*?]

Page 5

* You mention CONGEST: consider explaining why CONGEST and local certification
are somehow related. 

[todo*?]

* [GNT]: no year? 
[yx: the bibtex exported from siam does not contain year so i added it]

[todo?]

* "It was known that treedepth [...]": better connect with your work. 

[todo*?]

Page 7

* Around Lemma 2.3: you use arboricity and degeneracy interchangeably and without 
definition. 

[todo?]
[yx: edited (marked in red). use degeneracy]
[yx: check if other places use arboricity]

Page 8

* Is the discussion after conjecture 2.5 known or new? Make it explicit. 

[todo*?]
[yx: should we make it a lemma after conjecture 2.5? and refer to that lemma here.]

* "[...] This contradicts [...]": strange flow

[todo?]
[yx: edited, marked in red]

* Heavy-light decomposition: if it is known, give a ref, if it is new, say it. 

[todo?]
[yx: edited citation]

* induce_d_

[todo?]
[yx: fixed]

* "For each leaf [...]" strange switch to an imperative style. 

[todo?]
[yx: edited, marked in red]

Page 9

* Move figure 1 at the start of section 3, and improve the caption

[todo?]
[yx: edited the paragraph before lemma 3.1 and put the figure there, im not sure about whether it would be better to put it at the very start of this section]
[yx: figure is changed and added explanation in the caption]

* You should say earlier why the crossing is enough for you (it makes the 
connectivity very low)

[todo?]
[yx: edited, stated around the beginning of sec3, marked in red]

* "accept" appears in two different fonts. 

[todo?]
[yx; fixed]

Page 10 

* "where they from"

[todo?]
[yx: edited]

Page 12

* "We assume the graph is connected" should be said earlier. 

[todo?]
[yx: I commented out this line and stated in the first page, after problem 1.2, marked in red.]

Page 13

* Somewhere it should be checked that an edge cannot be oriented in both directions..?

[todo*?]

Page 14

* Lemma 4.3 and proofs: why include this? 

[todo*?]

Page 15

* "provide v _with_ the lists"

[todo?]
[yx: fixed]

* rank is not defined

[todo?]
[yx: edited and made it red]

* address is not defined

[todo?]
[yx: I rewrote some part of the vertex-connectivity proof, marked in red. This is defined in the certificate assignment paragraph.]

* Add a picture for heavy-light decomposition

[todo?]
[yx: added in page 3, see the comment i left there.]

* u_i_j is the largest rank. Why don't you also store the smallest rank? 

[todo?]
[yx: I rewrote some part of the vertex-connectivity proof, marked in red. This is explained in plain text.]

* "where T_i(v)": define T_i separately, since it is also used elsewhere (= it is 
not a local variable of the definition of u)

[todo?]
[yx: removed and added a line (red) at the beginning of that section]

page 19

* improve the caption of Fig 3

[todo?]
[yx: edited. See p11.]


Review #316C
===========================================================================

Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This paper gives new proof labeling schemes for certifying edge and vertex connectivity. It achieves $O_k(\log n)$-bit certificates for $k$-edge-connectivity, which is optimal in its dependency in $n$. Regarding vertex-connectivity, it achieves $O_k(\sqrt{n})$-bit certificates for $k$-vertex-connectivity, and $O(\log n)$-bit certificates for planar graphs (note that planar graphs have bounded edge and vertex connectivity). The paper complements its $O_k(\sqrt{n})$ upper bound by a lower bound for their approach, showing that said approach was essentially pushed to its limits and that a scheme achieving better than $O_k(\sqrt{n})$ will need to rely on other combinatorial objects.


The edge-connectivity certification result is essentially two results in one, one for even $k$ and the other for odd $k$. The result significantly generalizes similar prior results by Bousquet, Feuilloley, and Pierron (ref BFP24 in the paper), who gave $O(\log n)$-bit proof labeling schemes for $2$-edge-connectivity, $2$-vertex connectivity, and $3$-vertex connectivity. The result for even $k$ makes use of some classic results on decomposing well connected graphs, not unlike how prior results in BFP24 used ear-decompositions. The result for odd $k$ relies on $k$-edge-connectivity reducing to the graph remaining $k-1$-connected when removing any edge. This is certified efficiently using a partition of the edges into $\exp(O(k^2))$ sets whose individual removal keeps the graph $k-1$-edge-connected, from ref DJS03 in the paper.


The $O_k(\sqrt{n})$-bit vertex connectivity certification is much more involved, and actually relies on the unproven Itai-Zehavi conjecture characterizing $k$-vertex-connectivity by the existence of $k$ independent spanning trees rooted at each node, which can be replaced by showing that $k$ nodes admit $k$ independent spanning trees rooted at them. Note that the unproven nature of the conjecture does not mean that the scheme presented in the paper could potentially fully break, rather it means that said scheme might not be able to certify all $k$-vertex-connected graphs. The paper is able to certify $k$-vertex-connectivity in all graphs that admit $k$ nodes that each have $k$ independent spanning trees rooted at them, and there might be partial results known about the Itai-Zehavi conjecture that show that the paper is thus able to certify $k$-vertex connectivity unconditionally for some natural classes of graphs. Certifying that two spanning trees are independent requires sharing a lot of information about them throughout the network, leading to the high $\sqrt{n}$ cost, which is only obtained after multiple optimizations limiting how much the information about the spanning trees is replicated accross the network, while keeping it duplicated enough for nodes to locally verify the independence of two spanning trees. The $\sqrt{n}$ is shown to be optimal using a connection with communication complexity.

The scheme for planar graphs exploits a characterization of vertex connectivity specific to planar graphs, together with useful properties like the bounded degeneracy of planar graphs, to obtain smaller certicates.


**Evaluation**

The paper makes important progress on the local certification of classic and important graph properties. On top of achieving tight results for edge-connectivity, it complements its more difficult scheme for vertex-connectivity with a lower bound showing the limitation of its approach, and shows how to obtain better results on an important class of graphs (planar graphs). It is also generally nice to read.

On the negative side, the edge connectivity results are obtained using essentially the first techniques one would probably try, and the more interesting vertex connectivity result might be very far from tight. I find interesting what the paper uncovered regarding the certification of independent spanning trees but it's very possible that the two problems (vertex connectivity and independent spanning trees) are very different in the end (as maybe evidenced by the fact that $k$-vertex connectivity admits $O(\log n)$ certificates for the very first values of $k$).

All in all, I find the paper interesting, and it could be accepted at PODC, but I find it below the average PODC paper (weak accept).

Comments for authors
--------------------
- page 7, lemma 2.2: isn't the simple scheme you mention for vertex certification only $O(\Delta (f(n) + \log \Delta))$ bits, since each node receives at most $\Delta$ edge-certicates and $O(\log \Delta)$ bits suffice to tag a certificate with the colors of its endpoints?

[todo?]
[yx: I think it's correct, only change the lemma statement]

- page 9, lemma 3.1, (ii): it might be clearer to formulate this property as "for any $G'$ built as follows, $G' \not \in \cal{P}$"

[todo?]
[yx: edited (red)]

- page 15: expansive -> expensive

[todo?]
[yx: edited]

- page 15: if I understand correctly, the information of $\eta_T(v)$ is already contained in $p_T(v)$. It might be worth pointing out, or introducing $\eta_T$ and $p_T$ differently.

[todo?]
[yx: I rewrote some part of the vertex-connectivity proof, marked in red. Now eta_T(v) is included in p_T(v).]

- page 16, proof of lemma 5.2: here and in other places you use the argument that if $u$ is an ancestor of $v$ in both $T_1$ and $T_2$, then that means that the paths from root to $v$ of both trees go through $u$, and thus are not internally vertex-disjoint. I think this proof would be clearer by stating this explicitly, and also addressing the fact that this only works for a non-root $u$.

[todo?]
[yx: I rewrote some part of the vertex-connectivity proof, marked in red. I added some explanation at the beginning of this section, which includes this observation. ]


- page 18, around 75% into the page: the port p_j -> the node p_j ? (or call these nodes "ports" elsewhere, explaining why you call them that)

[todo?]
[yx: change to "vertex"]
[yx: But think whether a high-level description of the construction should be stated at the beginning of sec5.2]

- page 18, near bottom: the two spanning trees [...] is -> are

[todo?]
[yx: edited]

- page 19, beginning of the proof of Lemma 5.3: DISJ(x,y)=TRUE should be DISJ(x,y)=FALSE

[todo?]
[yx: edited]

==> conclusion_PODCvers.tex <==
\section{Conclusion}

In this work, we present a systematic study of the local certification of $k$-edge/vertex-connectivity, establishing new upper and lower bounds. Our results sharpen our understanding of the landscape of what is achievable, but they also leave several intriguing questions open.

\paragraph{$2$-edge/vertex-connectivity.}
In~\Cref{sec: lower}, our lower-bound construction for $k$-edge/vertex-connectivity relies on indistinguishability from graphs whose edge/vertex-connectivity is at most $2$. Notably, the construction uses graphs of maximum degree $O(k)$, and hence bounded-degree graphs when $k$ is constant. 
In contrast, \Cref{sec: 2-conn-bdd-deg} shows that certifying $2$-edge/vertex-connectivity in bounded-degree graphs is particularly simple: both admit constant-bit certification schemes. This discrepancy suggests that certifying $2$-connectivity may be qualitatively different from certifying $k$-connectivity for $k \ge 3$.
A natural question is whether $2$-connectivity can be certified using $O(1)$ bits in general graphs, when the degree is unbounded. Alternatively, does a nontrivial lower bound exist, with intrinsically hard instances necessarily requiring unbounded degree?


\paragraph{$k$-edge-connectivity.}
For $k$-edge-connectivity, we establish a tight bound of $\Theta_k(\log n)$ with respect to $n$. However, the dependence on $k$ is still far from being understood. 
In~\Cref{sec:kec-upper}, we show that for $k \ge 3$, $k$-edge-connectivity can be certified using $O(k \log n)$ bits when $k$ is even and $O(81^{k^2} k\log n)$ bits when $k$ is odd. In~\cite{DeVosJS03}, DeVos, Johnson, and Seymour claimed (without proof) that the factor $81^{k^2}$ can be reduced to $2^{O(k)}$. For $k \le 5$, the factor $81^{k^2}$ can be replaced with $30$. Whether the dependence on $k$ can be made subexponential remains open. 
On the lower bound side, we only obtain $\Omega\!\left(\frac{\log n}{k}\right)$. Closing the gap between the current upper and lower bounds, in terms of their dependence on $k$, is an interesting direction for future work.

\paragraph{$k$-vertex-connectivity.}
In~\Cref{sec:kvc-upper}, we show that $k$-vertex-connectivity admits certificates of  $\Tilde{O}_k(\sqrt{n})$ bits under the Itai--Zehavi conjecture, while our lower bound remains $\Omega_k(\log n)$. Determining the correct complexity of certifying $k$-vertex-connectivity therefore remains a central open problem arising from this work.

A related observation further highlights the difficulty of the problem. In~\Cref{sec:lower-2indst}, we prove that certifying whether two prescribed spanning trees are independent requires $\Omega(\sqrt{n})$ bits. In contrast, $2$-vertex-connectivity and $3$-vertex-connectivity admit $O(\log n)$-bit certification schemes via variants of ear decompositions~\cite{BFP21}. This gap suggests that the independent spanning tree approach is unlikely to yield tight bounds for general $k$-vertex-connectivity. Progress may require new structural insights or a more careful way of selecting the spanning trees.


\paragraph{Approximate local certification schemes.}
Censor-Hillel~et~al.~\cite{CHPP20} introduced the notion of an \emph{approximation proof-labeling scheme}, which distinguishes graphs satisfying a property from graphs that are far from satisfying it. For example, they showed that certifying graph diameter $\le k$ requires $\Omega\!\left(\frac{n}{k}\right)$ bits, whereas a $2$-approximation requires only $O(\log n)$ bits.

Our results also have implications in this approximate setting. The lower bound constructions in~\Cref{sec: lower} can be adapted to obtain the same lower bound for distinguishing graphs with $(\ge k)$-edge/vertex-connectivity from those with $(\le k-2)$-edge/vertex-connectivity. On the upper bound side, if we allow an additive-one approximation, then $k$-edge-connectivity for every $k$ can be certified in $O(k\log n)$ bits, simply by applying the scheme for even values of $k$.

Similar to how edge-connectivity is characterized by edge-disjoint spanning trees, a natural analogue for vertex-connectivity is a \emph{connected dominating set partition} (CDS partition), introduced in~\cite{CHGK13}. The best known result~\cite{CHGG+17} shows that every $k$-vertex-connected graph admits a partition into $\Omega\!\left(\frac{k}{\log^2 n}\right)$ connected dominating sets (CDSs). Since each CDS can be certified using $O(\log n)$ bits, this implies that one can certify $\Omega\!\left(\frac{k}{\log^2 n}\right)$-vertex-connectivity using $O\!\left(\frac{k}{\log n}\right)$ bits, assuming the graph is $k$-connected. In other words, this yields an $O(\log^2 n)$-approximation for $k$-vertex-connectivity.

If any exact certification of $k$-vertex-connectivity turns out to require large certificates, is it possible to obtain significantly better approximation ratios using a small number of bits? Understanding this trade-off between accuracy and certificate size for vertex-connectivity remains an interesting direction for future work.
 



% \section{Conclusion}

% In this work, we give a comprehensive study of local certification of $k$-edge-connectivity and $k$-vertex-connectivity, obtaining various upper and lower bounds. However, many intriguing questions remain open.

% \paragraph{$2$-edge/vertex-connectivity}
% We have shown in~\Cref{sec: lower} that the lower-bound graph for distinguishing $2$-edge/vertex-connectivity and $k$-edge/vertex-connectivity is of bounded degree ($O(k)$). However, in~\Cref{sec: 2-conn-bdd-deg}, we see that certifying $2$-edge/vertex-connectivity on bounded-degree graphs is easy, which has a constant-bit certification scheme. It provides us with evidence that certifying $2$-connectivity could be fundamentally different from certifying $k$-connectivity for $k\geq 3$. Is it true that certifying $2$-connectivity can be done in $O(1)$ bits? Or is it the case that there exists a lower bound, and the hard instance is of unbounded degree?

% \paragraph{$k$-edge-connectivity.}
% In~\Cref{sec:kec-upper}, we show that for $k\geq 3$, certifying $k$-edge connectivity can be done in $O(k\log n)$ bits for even $k$ and $O(81^{k^2}\log n)$ bits for odd $k$. Whether the dependency on $k$ can be reduced is left as an open question. On the other hand, we only have a lower bound of $\Omega(\frac{\log n}{k})$. Is it possible to close the gap?

% \paragraph{$k$-vertex-connectivity}
% In~\Cref{sec:kvc-upper}, we show that certifying $k$-vertex-connectivity can be done in $\Tilde{O}_k(\sqrt{n})$ bits. While our lower bound for certifying $k$-vertex-connectivity is still $\Omega_k(\log n)$. What would be the correct complexity is the main open question left in this paper. 

% Notice that we also proved in~\Cref{sec:lower-2indst} that certifying two prescribed spanning trees are independent requires $\Omega(\sqrt{n})$ bits, while certifying $2$-vertex connectivity is known to be certified in $O(\log n)$ bits via open ear-decomposition~\cite{BFP21}. This suggests that the independent tree approach may not be the right way to get a tight bound. Either we need to apply other tools for $k$-connectivity, or we need to find a clever way to choose those $k$ spanning trees so that they become easy to certify.

% \paragraph{Approximate local certification scheme.}
% In~\cite{CHPP20}, they introduce the notion of \emph{approximation proof-labeling scheme}, which is a local certification scheme that distinguishes graphs with a certain property from graphs that are far from having that property. They prove that certifying graph diameter $\diam\leq k$ requires $\Omega(\frac{n}{k})$ bits while a $2$-approximation proof-labeling scheme requires only $O(\log n)$ bits.

% In our work, it is also worth mentioning the potential application and future work in approximate local certification schemes. The lower bound constructions shown in~\Cref{sec: lower} can, in fact, be modified to prove a lower bound for distinguishing $k$-connectivity and $(k-2)$-connectivity. On the upper bound side, if we allow an additive-one approximation, then approximate $k$-edge-connectivity can be certified in $O(k\log n)$ bits.

% The main tool that captures edge-connectivity is edge-disjoint spanning trees, and an analogous tool for vertex connectivity is \emph{connected dominating set partition (CDS partition)}, which is a partition of the vertex set into connected dominating sets, as defined by~\cite{CHGK13}. Using the current best result for CDS partition given in~\cite{CHGG+17}, if a graph is $k$-connected, then it can be partitioned into $\Omega(\frac{k}{\log^2n})$ CDSs. By certifying CDSs (which can be done in $\log n$ bits each), we can certify $\Omega(\frac{k}{\log^2n})$-connectivity with $O(\frac{k}{\log n})$ bits under the assumption that the graph is $k$-connected. This gives a $O(\log^2n)$-approximation. If certifying $k$-vertex connectivity turns out to be hard, is it possible to get a better approximation ratio for certifying $k$-vertex connectivity using a small number of bits?

==> draft-yx.tex <==
\section{Introduction}


We study local certification of high connectivity in distributed networks, modeled as $n$-vertex simple undirected graphs $G$. In a \emph{local certification scheme}~\cite{GS16,Feu21}\mtt{Do these two papers have the same model as ours?}, the vertices of $G$ are given pairwise distinct $O(\log n)$-bit  identifiers, and a prover assigns a short label to each vertex. Each vertex then runs a local deterministic verifier and outputs accept or reject after inspecting only its own identifier and label, together with the labels of its neighbors. \mtt{I consider this model $KT_0$. Please confirm.} The scheme must satisfy completeness and soundness: if $G$ satisfies the prescribed global property $\mathcal{P}$, then there exists a labeling under which all vertices accept; if $G$ does not satisfy $\mathcal{P}$, then for every possible labeling, at least one vertex rejects. The efficiency of a scheme is measured by its per-vertex label size, defined as the maximum, over all vertices, of the number of bits in the prover-assigned label. As is the norm in this model, we assume that the input network $G$ is connected. Under this assumption, we investigate the per-vertex label size required to certify that $G$ is \emph{$k$-edge-connected} (resp. \emph{$k$-vertex-connected}) for each integer $k\ge 2$; that is, every pair of vertices is connected by at least $k$ edge-disjoint paths (resp. at least $k$ internally vertex-disjoint paths). \mtt{Is the problem definition clear enough for an algorithmist whose expertise does not contain distributed computation.}







Certifying high edge or vertex connectivity is a natural preprocessing step for distributed algorithms that exploit high connectivity as an algorithmic resource. Such algorithms often use high connectivity in one of two ways: they either decompose the input graph into highly connected components and run the subsequent algorithm within each component, or they use the disjoint tree structures available in highly connected networks to disseminate information efficiently. \yijun{elaborate a bit to further motivate connectivity certification?} \mtt{We now have these two, detailed in the subsequent two paragraphs.}

The work of Bousquet, Feuilloley, and Pierron~\cite{BFP21,BFP24} is a representative example of the former approach. They show that $k$-vertex-connectivity, for $k\le 3$, can be certified with $O(\log n)$-bit labels per vertex. They then decompose the graph into $2$- or $3$-vertex-connected components and exploit the restricted structure of these components to certify several $H$-minor-free graph classes, for small excluded minors $H$, again with $O(\log n)$-bit labels per vertex. This line of work is motivated by the broader goal of certifying minor-closed graph classes~\cite{FFM+23, FFM+20, esperet2022local,CKM25},\mtt{Add more references?} a family that includes fundamental examples such as planar graphs and bounded-treewidth graphs. They also leave open the problem of designing efficient local certification schemes for higher vertex connectivity (Open Question~52 in~\cite{BFP21}),\mtt{BFP21 here is important because this makes the open problem aged.} motivated in part by the possibility of extending this decomposition-based approach to graph classes defined by larger excluded minors.

The work of Chandra, Chang, Dory, Ghaffari, and Leitersdorf~\cite{ChandraCD0L24} is a representative example of the latter approach. \mtt{Other similar works?} Their distributed algorithm exploits high edge connectivity to disseminate information efficiently: in a graph with edge connectivity $\lambda$, it solves $q$-message broadcast in $O(((n+q)/\lambda)\log n)$ rounds. Since the vertices do not know $\lambda$ in advance, the algorithm uses a guessing procedure to obtain a suitable estimate. A local certificate for $k$-edge-connectivity would provide a complementary way to verify a guaranteed lower bound on $\lambda$, allowing the network to run high-connectivity algorithms under a locally certified connectivity promise.
 \mtt{If their computation allows a helper (our local certification scheme) to tell their algorithm $\lambda$, then I believe that the overall rounds becomes smaller if $\delta > \lambda$. If yes, please add some concrete statement here.}

We begin with showing that certifying $k$-vertex-connectivity and $k$-edge-connectivity requires per-vertex label size $\Omega_k(\log n)$ for every $k \ge 3$ (\cref{thm: k-conn-lower}). This answers Question~51 of~\cite{BFP21} in the affirmative for all constant $k \ge 3$. Our proof applies even to \emph{bounded-degree graphs}, that is, graphs whose maximum degree $\Delta$ is upper bounded by a constant. This lower-bound argument does not extend to the case $k=2$: indeed, we prove in \cref{thm: 2-edge-conn} and \cref{thm: 2-vertex-conn} that, on bounded-degree graphs, both $2$-edge-connectivity and $2$-vertex-connectivity can be certified with $O_\Delta(1)$-bit labels per vertex.



\begin{restatable}{theorem}{thmKConnLower}\label{thm: k-conn-lower}
    For every integer $k \ge 3$, any local certification scheme for $k$-edge-connectivity or for $k$-vertex-connectivity requires per-vertex labels of size $\Omega((\log n)/k)$, even on bounded-degree graphs and even when each vertex has access to the identifiers of its neighbors.
\end{restatable}
\yx{Note that now we have three models, where each theorem works in different model (Omega(log n)-lower bound works in KT1, upper bounds for k-EC/k-VC in general graphs work in KT0, and additional results for 2-EC and 2-VC work in anonymous.) These would be added to the theorem statements (I haven't done yet) and be elaborated a bit in the model definition section, so may need to take this into account}


Our second result is a matching upper bound for $k$-edge-connectivity, stated in \cref{thm: k-ec}. Together, \cref{thm: k-conn-lower} and \cref{thm: k-ec} give tight bounds for certifying $k$-edge-connectivity for every constant $k \ge 3$. The certification scheme in \cref{thm: k-ec} uses a unified construction for all $k\ge 2$, based on applying Edmonds' branching theorem~\cite{Edmonds73} to the directed graph $\vec{G}$ obtained from $G$ by replacing each edge $\{u,v\}$ with the two antiparallel arcs $(u,v)$ and $(v,u)$. A key point is that this directed formulation substantially simplifies the extension from small values of $k$ to arbitrary $k$. In contrast, the best previous result applies only to $2$-edge-connectivity~\cite{BFP24}; its proof relies on a purely undirected graph-theoretic tool, namely an ear decomposition. It remains unclear how to generalize that proof to arbitrary $k$ using only purely undirected graph-theoretic tools.







\begin{restatable}{theorem}{thmkEC}\label{thm: k-ec}
    For every integer $k \ge 2$, there is a local certification scheme for $k$-edge-connectivity with per-vertex label size $O(k\log n)$ when $k$ is even, and $O(81^{k^2}k\log n)$ when $k$ is odd.
\end{restatable}
\mtt{This theorem will be updated after $k$-ec section is rewritten.}


Our third result is an upper bound for $k$-vertex-connectivity, stated in~\cref{thm: k-vc-cert}. For $k=4$, the upper bound is unconditional; for every $k\ge 5$, it is conditional on the Itai--Zehavi conjecture~\cite{ZI89}. This conjecture states that an undirected graph $G$ is $k$-vertex-connected if and only if, for every vertex $r\in V(G)$, there exist $k$ \emph{independent spanning trees} rooted at $r$. Here, independence means that, for every vertex $x\in V(G)\setminus {r}$, the paths from $r$ to $x$ in the $k$ trees are internally vertex-disjoint. In contrast, the best previous result applies only to $2$-vertex-connectivity and $3$-vertex-connectivity~\cite{BFP24}; its proof follows a different route, based on open ear decompositions and Mondshein sequences. The case $k\ge 4$ was left open as Question~52 in~\cite{BFP21}. \mtt{I use BFP21 when referring to open questions, and BFP24 when referring to their algorithmic results.}




\begin{restatable}{theorem}{thmKVC}\label{thm: k-vc-cert}
    For every integer $k\ge 4$ for which the Itai--Zehavi conjecture holds, $k$-vertex-connectivity admits a local certification scheme with per-vertex label size $O(k^3\sqrt{n}\log^{2.5} n)$. In particular, since the conjecture is known to hold for $k=4$, $4$-vertex-connectivity admits a local certification scheme with per-vertex label size $O(\sqrt{n}\log^{2.5} n)$.
\end{restatable}

%\begin{conjecture}[{Itai--Zehavi conjecture~\cite{ZI89}}]\label{conj: Itai--Zehavi}
%    A graph $G$ is $k$-vertex-connected if and only if for every vertex $r\in V(G)$, there exist $k$ independent spanning trees rooted at $r$.
%\end{conjecture}


\yx{add the 2-connectivity result below}
As mentioned after~\Cref{thm: k-conn-lower}, our lower bound only applies to k≥3. This raises a natural question: what is the complexity of certifying 2-edge-connectivity and 2-vertex-connectivity? Can one obtain sublogarithmic upper bounds or superconstant lower bounds? We partially answer this question by showing that both 2-edge-connectivity and 2-vertex-connectivity admit local certification schemes with constant per-vertex label size on bounded-degree graphs. In fact, our certificates work even in the anonymous setting, where vertices have no identifiers.

\begin{restatable}{theorem}{thmTwoEC}\label{thm: 2-edge-conn}
    There exists a local certification scheme for $2$-edge-connectivity on bounded-degree graphs with per-vertex label size $O(\Delta\log\Delta)$, even when the vertices are anonymous.
\end{restatable}

\begin{restatable}{theorem}{thmTwoVC}\label{thm: 2-vertex-conn}
    There exists a local certification scheme for $2$-vertex-connectivity on bounded-degree graphs with per-vertex label size $O(2^{\Delta}\cdot\Delta\log\Delta)$, even when the vertices are anonymous.
\end{restatable}

\yx{say that 2-conn is fundamentally different from k ge 3}
This result improves upon~\cite{BFP21} when restricted to bounded-degree graphs. Their scheme essentially certifies an ear decomposition of the graph. Simulating the order in which ears are added may require may require $O(\log n)$ bits, even when the graph has constant degree; see Lemma 20 and Corollary 21 of~\cite{BFP21} for details.

Moreover, we show that for $2$-edge-connectivity, the certification scheme can be extended to bounded-expansion graphs, a broad family that includes bounded degree graphs, planar graphs, and more generally, minor-closed graphs.

\begin{restatable}{theorem}{thmTwoECnew}\label{thm: 2-ec-bdd-expansion}
    Let $\Fcal$ be a bounded-expansion graph class. Given the promise that the input graph belongs to $\Fcal$, there exists a local certification scheme for $2$-edge-connectivity with $O(1)$ per-vertex label size, where the constant only depends on the graph class $\Fcal$.
\end{restatable}

In contrast, we prove a superconstant lower bound for certifying $2$-vertex-connectivity in the anonymous setting. Our construction is a slight modification of the lower bound for parity certification in~\cite{BFVZ26}. This lower bound inherently exploits the absence of identifiers and therefore does not extend to the setting where vertices have unique identifiers.

\begin{restatable}{theorem}{thmTwoVCLB}\label{thm: 2-vc-lb}
    Any local certification scheme for $2$-vertex-connectivity requires per-vertex labels of size $\Omega(\log(\log^*n))$ when the vertices are anonymous.
\end{restatable}

We note that~\Cref{thm: 2-ec-bdd-expansion} and~\Cref{thm: 2-vc-lb} are incomparable. The lower-bound construction in~\Cref{thm: 2-vc-lb} does not have bounded degeneracy, whereas~\Cref{thm: 2-ec-bdd-expansion} only concerns bounded-expansion graphs.\yx{consider removing it}




We summarize the known and new upper and lower bounds on the optimal per-vertex label size for certifying $k$-edge-connectivity and $k$-vertex-connectivity in \cref{tab: results}.




\subsection{Technique Overview}

\paragraph{Lower-bound technique.}
Our lower bound follows the cut-and-plug framework of Göös and Suomela~\cite{GS16}. The graph-theoretic task is to find, for each property $\mathcal{P}$, a witness graph $G\in\mathcal{P}$ with a small local interface whose rewiring destroys the property. In our setting, this interface is an edge $\{u,v\}$ whose endpoints have only $O(k)$ neighbors. Consider two copies $G_1$ and $G_2$ of $G$, with corresponding edges $\{u_1,v_1\}$ and $\{u_2,v_2\}$. Both $G_1$ and $G_2$ satisfy $\mathcal{P}$, so there are labelings under which all vertices accept. The cut-and-plug operation starts from the vertex-disjoint union $G_1 \uplus G_2$, deletes the two edges $\{u_1,v_1\}$ and $\{u_2,v_2\}$, and adds the cross edges $\{u_1,v_2\}$ and $\{u_2,v_1\}$. For our witness graphs, this edge-swapped union no longer satisfies $\mathcal{P}$: in fact, its edge connectivity and vertex connectivity are both at most $2$. However, if the labels are too short, the two copies can be chosen so that, after this edge swap, every vertex still sees exactly the same local view as it saw in some accepting copy. Hence all vertices still accept the edge-swapped union, contradicting soundness.

The rewiring itself uses only two copies, but the proof must first force two copies to be locally indistinguishable to the verifier. To do this, we consider polynomially many copies of the same witness graph, with different assignments of identifiers to the vertices. If the labels have size $o(\log n)$, then there are too few possible labeled local views around the small interface to distinguish all these copies. Hence two copies can be chosen so that, after the rewiring, every vertex still sees a local view that it would accept in some valid copy. The verifier is therefore forced to accept the rewired graph, even though it is not $k$-edge-connected or $k$-vertex-connected for any $k\ge 3$, contradicting soundness.

This also explains why the strategy is tight with respect to $k=2$: the obstruction produced by the rewiring has connectivity at most $2$, which is not enough to refute $2$-connectivity. Indeed, on bounded-degree graphs, both $2$-edge-connectivity and $2$-vertex-connectivity admit $O_\Delta(1)$-bit certificates.

\paragraph{Upper-bound technique for edge connectivity.}
For the upper bound for $k$-edge-connectivity, we move from the undirected graph $G$ to the directed graph $\vec{G}$ obtained by replacing each undirected edge $\{u,v\}$ with the two antiparallel arcs $(u,v)$ and $(v,u)$. The key observation is that $G$ is $k$-edge-connected if and only if $\vec{G}$ is $k$-arc-strongly connected. This directed formulation lets us use Edmonds' branching theorem~\cite{Edmonds73}: high arc-connectivity can be witnessed by collections of arc-disjoint spanning branchings rooted at a common vertex. The prover certifies these branching structures, and each vertex locally checks their consistency.

This directed viewpoint is the reason the construction extends cleanly to arbitrary $k$. Previous local certificates for $2$-edge-connectivity relied on undirected tools such as ear decompositions, whose generalization to larger $k$ is not immediate. By contrast, Edmonds' theorem gives a uniform certificate for all $k$: increasing $k$ simply means certifying more branching structures. Thus the directed setting turns the problem of certifying high undirected edge connectivity into a direct and modular certification of directed branching witnesses.

\paragraph{Upper-bound technique for vertex connectivity.}
For the upper bound for $k$-vertex-connectivity, we use the Itai--Zehavi characterization in terms of independent spanning trees. Assuming this characterization for the given value of $k$, it suffices to certify suitable collections of rooted spanning trees such that, for every vertex $x$, the root-to-$x$ paths in the trees are internally vertex-disjoint. Thus the main building block is to certify that two prescribed spanning trees $T_1$ and $T_2$, rooted at the same vertex, are independent.

A naive certificate would give each vertex its full list of ancestors in both trees, but this can require linear space. We reduce the cost using heavy-light decompositions. In each tree, every root-to-vertex path intersects only $O(\log n)$ heavy-light segments, so the prover can encode such a path by a short list of segment-rank pairs. These encodings allow vertices to locally test ancestor relations. The remaining challenge is to ensure that, if independence fails, then some vertex can detect a common internal ancestor on its two root paths. To achieve this, the certificates propagate compact path addresses through the two trees, using a long/short segment threshold to balance the amount of information stored at each vertex: there are few long segments globally, while only few short-segment vertices appear along any root-to-vertex path. This yields an $\widetilde{O}(\sqrt{n})$-bit certificate for independence of two rooted spanning trees.

We also show that this building block is essentially optimal. Namely, there are $n$-vertex graphs with two prescribed spanning trees $T_1$ and $T_2$ rooted at the same vertex $r$ such that any local certification scheme for verifying that $T_1$ and $T_2$ are independent requires per-vertex label size $\Omega(\sqrt{n})$.


\begin{restatable}{proposition}{thmIndepST}\label{lem: indep-st-lower}
There are $n$-vertex graphs $G$ with two spanning trees $T_1$ and $T_2$ rooted at the same vertex $r$, given as part of the input, such that any local certification scheme for verifying that $T_1$ and $T_2$ are independent requires per-vertex label size $\Omega(\sqrt{n})$.
\end{restatable}



This independent-tree formulation makes the extension to larger $k$ direct. Once we can certify independence of two rooted spanning trees, we certify pairwise independence among the $k$ trees required for each root. The only additional cost is the number of tree pairs and roots, leading to the stated $O(k^3\sqrt{n}\log^{2.5} n)$ per-vertex label size.


\yx{mentioned 2-connectivity upper bound below}
\paragraph{Constant upper bound for $2$-connectivity.}
\yx{title to be changed}
Our main building block for certifying $2$-edge-connectivity is a decomposition theorem stating that every $2$-edge-connected graph can be covered by a constant number of (possibly disconnected) Eulerian subgraphs.

This decomposition immediately suggests a certification strategy. Suppose that the prover is allowed to place labels not only on vertices but also on edges, where the label of an edge can be read by both of its endpoints. The prover can then assign a distinct label to each Eulerian subgraph and let every edge inherit the label of the subgraphs containing it. Each vertex then checks that, for every label, the number of incident edges carrying that label is even. On bounded-degree graphs, it is known that labels on edges can be transformed into labels on vertices with only an $\Tilde{O}(\Delta)$ overhead~\cite{BFVZ26}.

%Suppose that the prover is allowed to put labels not only to the vertices but also to the edges that can be accessed by each incident vertex, then the prover can assign distinct label on the edges of each Eulerian subgraph, this can be verified by requiring each vertex to check that its degree is even in each Eulerian subgraph. On bounded degree graphs, it is known that the labels on edges can be transformed into labels on vertices with an $\Tilde{O}(\Delta)$ overhead.~\cite{BFVZ26}.



%On bounded degree graphs, the edge certification scheme can be transformed into a vertex certification scheme with an {\color{red}$\Tilde{O}(\Delta)$} overhead
%\footnote{In this paper, we will write explicitly the dependency on $\Delta$ in the Theorems whenever possible. In distributed graph algorithms, it is natural to consider graph classes with bounded degree. For local certification schemes, the first non-trivial bound with dependency in the max-degree $\Delta$ was given in~\cite{BFZ25}.}. 


\yx{mention that this can be extended to bounded expansion}
%with the recently developed constant-size certification scheme for pseudoforests~\cite{BFVZ26} as a building block.

For $2$-vertex-connectivity, we show that constant-size label suffices for bounded degree graphs by a reduction to $2$-edge-connectivity. Intuitively, we replace each vertex with an edge and split its neighbors into two nonempty sets, each connecting to a different endpoint of the edge. Observe that if the original graph is $2$-vertex-connected, then the modified graph is $2$-edge-connected regardless of how we partition the neighborhood. Conversely, we prove that if all such graphs are $2$-edge-connected, then the original graph is $2$-vertex-connected. We note that the converse direction works only for $2$-vertex connectivity, and thus the reduction cannot be generalized to certify higher connectivity.




\paragraph{Super-constant lower bound for $2$-vertex connectivity.}
Our lower bound for $2$-vertex-connectivity is a slight modification of the parity lower bound in~\cite{BFVZ26}. In~\cite{BFVZ26}, the task was to certify that a graph has an even number of nodes. Their approach is to construct the  ``powerset graph'' and then glue two such graphs of even size together by identifying two nodes, one from each graph. The powerset graphs $G=(V,E)$ are bipartite graphs constructed as follows. Let $V=V_1\cup V_2$ where $V_1=[m]$ is the ground set of $m$ elements. For each subset $S\subseteq [m]$, itnroduce a vertex $v_S$ to $V_2$, and connect $v_S$ to every vertex $i\in S\subseteq V_1$. According to the finite unions theorem, they prove that if the number of labels is $o(\log^*n)$ where $n=|V|$, then there exist two subsets $S_1$ and $S_2$ such that $v_{S_1}$, $v_{S_2}$, and $v_{S_1\cup S_2}$ are colored the same. Since we are in the anonymous model, they simply take two copies of $G$, denoted by $G_1$ and $G_2$, and then identify $v_{S_1}$ in $G_1$ and $v_{S_2}$ in $G_2$ to obtain a graph $G'$ with an odd number of vertices. Notice that the identified vertex has the same view as $v_{S_1\cup S_2}$, and therefore all vertices still output \accept in $G'$. Our lower bound for $2$-vertex-connectivity follows from the observation that the construction of $G$ can be made $2$-vertex-connected, and that the combined graph $G'$ has a cut vertex (which is the identified one).





\paragraph{Paper organization.}
The rest of the paper is organized as follows. In \cref{sec:prelim}, we introduce the graph-theoretic tools used throughout the paper. In \cref{sec:lower}, we prove our lower bounds for certifying $k$-edge-connectivity and $k$-vertex-connectivity. We then present our upper bound for $k$-edge-connectivity in \cref{sec:kec-upper}, based on Edmonds' branching theorem. Finally, in \cref{sec:kvc-upper}, we give our upper bound for $k$-vertex-connectivity via independent spanning trees.

\clearpage

\yx{Some notes about the intended change for intro:
- Define the model anonymous/ PLS/ LCP as anonymous/ KT0/ KT1, define them formally here\\
- arrangement: general upper bound (edge, vertex) -> lower bound for k>2 -> additional 2-conn results, write as a story\\
- for k-vc, define IST and the conjecture here formally before the theorem
- Ill be editing the intro for the next few days so it may look a bit messy
}

\iffalse
Certifying graph connectivity has also been motivated in the prior work~\cite{BFP21} that tried to answer the problem of whether every minor-closed graph property admits an $O(\log n)$ local certification scheme~\cite{Feu21}. Certifying minor-closed properties are important open question in this field that has received great attention. Several natural graph classes are captured by minor-closed properties, including planar graphs, bounded genus graphs, and bounded tree-width graphs. Working towards this goal, it has been shown that planar graphs and bounded genus graphs can be certified in $O(\log n)$ bits~\cite{FFM+23, FFM+20, esperet2022local}. There are also meta-theorems showing that a broad class of properties can be certified efficiently in certain minor-closed graph classes~\cite{CKM25}.\yx{cite other meta-theorem papers} However, certifying general minor-closed properties remained wide open. 
\fi

%High edge and vertex connectivity are fundamental algorithmic resources in distributed networks.
%They underlie sparse connectivity certificates and distributed min-cut algorithms, where the value of the edge connectivity $\lambda$ guides sampling and sparsification~\cite{Thu95,GK13,DHNS19}.
%They also enable communication structures: highly edge-connected graphs support many spanning-tree-based backbones, while highly vertex-connected graphs support analogous connected-dominating-set structures, with applications to high-throughput information dissemination and oblivious routing~\cite{CGK14}.
%Recent algorithms further use high connectivity to build efficient communication backbones for tasks such as minimum spanning tree and multi-message broadcast~\cite{CPT20,CCDGHL24}.
%In these applications, a certified lower bound on the connectivity lets the algorithm choose its parameters, build the required number of backbones, and rely on the promised level of fault tolerance without first estimating the connectivity.
%This motivates the verification question studied here: can a connected distributed network locally certify, using short labels, that it is $k$-edge-connected or $k$-vertex-connected for a prescribed value of $k$?




\iffalse
Local certification provides us with a framework to achieve error detection. It was first proposed as a building block of a self-stabilizing algorithm to certify the solution under transient faults~\cite{KKP05}. In particular, space complexity is an important measurement of a self-stabilizing algorithm, and there has been work that makes black-box use of compact local certification schemes to design compact self-stabilizing algorithms~\cite{BFP14}. However, certifying the structure of a network itself is also important, as running distributed algorithms and certifying their solutions may be simpler in certain graph classes.
\fi

%{\color{red}In this paper, we study \emph{graph connectivity} in the local certification scheme. The \emph{edge (resp. vertex) connectivity} of an undirected graph is the size of the minimum edge (resp. vertex) cut, which is defined to be the minimum number of edges (resp. vertices) whose removal disconnects the graph. Connectivity captures the robustness of a network. Finding the connectivity of a graph is a fundamental problem that has been extensively studied in graph algorithms.\yx{cite some papers here} Our goal is to certify that a network has edge or vertex connectivity at least $k$ for some fixed value $k$.}
%\yx{I try to motivate this paper first by saying that connectivity is a fundamental problem, and say that it has been used in the minor-closed certification problem. Im not sure whether itis better or not.}
%\yx{Given the first paragraph, this one could be removed?}

sults toward the following questions: 

%\begin{problem}[{\cite[Question 57]{BFP21}}]\label{ques1}
%    Does the certification for $k$-vertex-connectivity require $\Omega(\log n)$ bits for any $k\geq 2$?
%\end{problem}
%\begin{problem}[{\cite[Question 58]{BFP21}}]\label{ques2}
%    Can $k$-vertex-connectivity be certified with $O(\log n)$ bits for any $k\geq 4$?
%\end{problem}

\iffalse
{\color{blue}
In this paper, we established several new results and tools towards certifying $k$-edge/vertex-connectivity for any fixed value of $k$. In~\Cref{sec: model-def}, we first give a brief background on different models of local certification schemes. In~\Cref{sec: resuls}, we give an overview of our contributions and the main ideas. A summary of our results can be found in~\Cref{tab: results}.
}
\fi

\iffalse

\subsection{Models of local certification}\label{sec: model-def}


{\color{blue}
Consider a family $\Fcal$ of (possibly labeled) input graphs. A local certification scheme allows vertices to verify some property $\Pcal$ for the graphs in $\Fcal$ using only their local views. In this paper, we consider $\Fcal$ to be a subset of all connected graphs. Local certification schemes can be described as an external \emph{prover} and a \emph{verifier}. Given a graph $G$ from $\Fcal$, the prover assigns some certificates to each vertex, and the verifier, which is a distributed algorithm, decides whether to accept based on the local view of a vertex.

More formally, a \emph{certificate assignment} of $G$ of length $s$ is a mapping from $V(G)$ to the set of $s$-bit strings. The \emph{view} of a vertex consists of some information in its neighborhood that is accessible to the verifier. Different models of local certification schemes have been proposed based on different levels of information contained in the view of a vertex. In the following, we define three extensively studied models. For readers who are familiar with the notion of local certification schemes, they correspond to the \emph{anonymous model}~\cite{KKP05, BFZ25}, the \emph{id-based proof-labeling schemes}~\cite{KKP05, Feu21}, and the \emph{locally checkable proofs} with local horizon $1$~\cite{GS16, Feu21}. To avoid confusion, in this paper we refer to them as the \emph{anonymous model}, the \emph{$KT_0$ model}, and the \emph{$KT_1$ model}, inspired by standard notions in distributed algorithms.\yx{cite papers.}

\begin{description}
    \item[The anonymous model] The vertices are not equipped with identifiers. The verifier has access only to the certificate assignments in its neighborhood.
    \item[The $KT_0$ model] The vertices are equipped with unique $O(\log n)$-bit identifiers. The verifier has access to its own ID and input, and the certificate assigned to all its neighbors, but not their identifiers.
    \item[The $KT_1$ model] The vertices are equipped with unique $O(\log n)$-bit identifiers. The verifier has access to the certificate assignments, IDs, and inputs of all its neighbors and itself.
\end{description}


The property $\Pcal$ that we want to certify should be independent of IDs. We say that $\Pcal$ admits a \emph{certification scheme} of size $s$ if there exists a verifier that satisfies \emph{completeness} and \emph{soundness}:

\begin{itemize}
    \item Completeness: For any $n$-vertex graph $G\in\Pcal$, and any ID assignment of $G$, there exists a certificate assignment of size $s(n)$ such that all vertices output accept.
    \item Soundness: For every $G\not\in\Pcal$, for every ID assignment of $G$, for any certificate assignment of any size, there exists at least one vertex that outputs reject.
\end{itemize}

There is another notion called \emph{edge certification scheme}~\cite{BFP21, FFM+23}. The setting is the same as in the standard local certification scheme, except that a certificate assignment of length $s$ for a graph $G$ is a mapping from $V(G) \cup E(G)$, rather than only $V(G)$, to the set of $s$-bit strings. Accordingly, the view of each vertex is enlarged to include the certificates assigned to its incident edges in each variation of the model. To distinguish edge-certification schemes from the standard local certification schemes, where we only assign certificates on vertices, we sometimes call the standard local certification schemes the \emph{vertex-certification schemes}. We will adapt some results from the edge certification scheme to the vertex-certification schemes and use them as building blocks for our main algorithms.

}

{\color{red}Notice that every local certification scheme that works in the anonymous model also works in the $KT_0$ model; and every local certification scheme that works in the $KT_0$ model also works in the $KT_1$ model. Therefore, proving an upper bound in the anonymous model is stronger than proving the same bound in the $KT_0$ model, which in turn is stronger than in the $KT_1$ model. From the perspective of lower bounds, the implications are reversed. In the region where the certificate assignment is of size $\Omega(\log n)$, the $KT_0$ model and the $KT_1$ model are asymptotically equivalent, as in the $KT_0$ model, the prover can always write the ID of a vertex in its own certificate and let the vertex verify the consistency. In contrast, there is a sharp separation between the anonymous model and the $KT_0$ model, as several tasks, including certifying leader election and spanning tree, are impossible in the anonymous model, while every computable function admits a certification scheme in the $KT_0$ model by assigning the description of the whole network to every vertex. See~\cite{KKP05} for more details.


In this paper, we will take $KT_0$ as our main focus. All our results at least hold for the $KT_0$ model except for the $2$-vertex-connectivity lower bound, which only works in the anonymous model.
%unless stated otherwise.
}

\yx{maybe can consider shortening this section here and moving the complete definition back to the prelim?}
\fi




\subsection{Results and technical overview}\label{sec: resuls}

\subsubsection{A lower bound for $k$-edge-connectivity and $k$-vertex-connectivity for $k\ge 3$.}

We answer \Cref{ques1} affirmatively by proving \cref{thm: k-conn-lower} using the so-called cut-and-plug technique introduced in~\cite{GS16}. The intuition is that we consider a $k$-edge/vertex-connected graph that has a special edge, {\color{red}where both endpoints have a bounded number of neighbors, and consider $\Theta(n)$ copies of such a graph} on different identifier sets. If the proof size is $o(\log n)$, then there must exist a constant number of copies receiving identical label assignments in the neighborhood of the special edges. We pick two such copies and glue them together to create a new accepting graph with low connectivity by removing the special edges and reconnecting each endpoint to the copy of its neighbor (originally incident to the special edge) in the other copy of the graph. This results in a graph with connectivity $2$ (both edge and vertex), but all vertices still accept due to identical labels in their neighborhoods.
%We answer \Cref{ques1} affirmatively by proving \cref{thm: k-conn-lower} using the crossing technique introduced in~\cite{GS16}. The intuition is that if a $k$-edge/vertex-connected graph has an edge with a bounded neighborhood, then we consider $\Theta(n)$ such instances. If the proof size is $o(\log n)$, then there must exist a constant number of instances receiving identical labels in the neighborhood of that edge, and we can pick two of them, cut the edges, and glue them together, which results in a graph with connectivity $2$ (both edge and vertex) but all vertices still accept due to identical labels in their neighborhoods.




We then devise an optimal local certification scheme for $k$-edge-connectivity for any constant $k \ge 3$ in \cref{sec:optimal}. Next, in \cref{sec:bottlenecktight}, we devise a bottleneck-tight local certification scheme for $k$-vertex-connectivity for $k=4$ (and, more generally, for any constant $k \ge 5$ assuming the Zehavi--Itai conjecture), thereby partially answering \Cref{ques2}.

%, we first construct a local certification scheme for a sparse subgraph that preserves $k$-vertex-connectivity (called a \emph{sparse certificate}). %It has been shown that iteratively finding $k$ BFS forest results in a sparse certificate for both $k$-edge- and $k$-vertex-connectivity~\Cref{lem: sparse-cert-iff}. Therefore, the local certification can be done by iteratively certifying BFS spanning forests.
%\begin{restatable}{lemma}{lemSparseCert}\label{lem: cert-sparse-cert}
%    There exists an $O(k\log n)$-bit local certification scheme for a sparse certificate of both $k$-edge-connectivity and $k$-vertex-connectivity.
%\end{restatable}
%Given the sparse certificate, any edge-certification scheme can be transformed into a vertex-certification scheme efficiently~\cref{lem:EdgeCert-degeneracy}. 

%In~\cite{BFP21}, they give a local certification scheme for $3$-vertex-connectivity using $O(\log n)$ bits on vertices and $O(1)$ bits on edges. As a corollary of \Cref{lem: cert-sparse-cert}, we can restrict ourselves to bounded arboricity graphs, and thus improve the complexity to $O(\log n)$ bits on vertices only.
%\begin{restatable}{corollary}{corThreeVC}\label{cor: 3-vc}
%    The complexity of certifying $3$-vertex-connectivity is $\Theta(\log n)$.
%\end{restatable}


\subsubsection{An optimal local certification scheme for $k$-edge-connectivity}\label{sec:optimal}

In~\cite{BFP21}, the authors certify $2$-edge-connectivity via a constructive characterization known as an \emph{ear decomposition}. We take a different route to certify $k$-edge-connectivity for all $k \ge 2$.

For even $k \ge 2$, we use the classical equivalence: an undirected simple graph $G$ is $k$-edge-connected if and only if $G$ admits an orientation $\vec{G}$ that is $(k/2)$-arc-strongly connected~\cite{Robbins39,NashWilliams60}. We then apply Edmonds' branching theorem~\cite{Edmonds73} to reduce the task to certifying $k/2$ pairwise arc-disjoint out-branchings and $k/2$ pairwise arc-disjoint in-branchings rooted at a common vertex, which can be done using $O(k\log n)$ bits.

For odd $k \ge 3$, we use another equivalence: $G$ is $k$-edge-connected if and only if there exists a partition of $E(G)$ into sets $E_1,E_2,\ldots,E_{\ell_k}$ such that $G\setminus E_i$ is $(k-1)$-edge-connected for every $i \in [\ell_k]$. In~\cite{DeVosJS03}, DeVos, Johnson, and Seymour showed that one may take $\ell_k \le 81^{k^2}$, and they further claimed (without proof) that this bound can be reduced to $\ell_k = 2^{O(k)}$. For small values of $k$, it is known that $\ell_3 \le 9$ and $\ell_5 \le 30$.

%Goedgebeur, M{\'{a}}cajov{\'{a}}, and Renders show that $\ell_3 \le 4$


%{\color{red}(To be aligned with corresponding sections)}



Given \cref{thm: k-conn-lower}, we know that \cref{thm: k-ec} is optimal for every constant $k \ge 3$.

%\mtt{The dependence on $k$ may be as large as $81^{k^2}$. Did we remove this dependence?}\yijun{I suggest that we keep the dependence on $k$ (and also max deg $\Delta$) whenever possible.}

\subsubsection{A bottleneck-tight local certification scheme for $k$-vertex-connectivity}\label{sec:bottlenecktight}
{\color{blue}
In~\cite{BFP21}, the authors certify $k$-vertex-connectivity for $k \in \{2,3\}$ using constructive characterizations based on \emph{open ear decompositions} and \emph{Mondshein sequences}. We again take a different route to certify $k$-vertex-connectivity for all $k \ge 2$. Our certification scheme relies on a conjecture by Zehavi and Itai~\cite{ZI89} on the equivalence between vertex-connectivity and independent spanning trees, which we now explain.

Given a graph $G$, two spanning trees $T$ and $T'$ rooted at the same vertex $r$ are said to be \emph{independent} if for any vertex $v$, the $v$--$r$ path in $T$ and the $v$--$r$ path in $T'$ are internally vertex-disjoint. We say that $G$ admits $k$ independent spanning trees rooted at $r$ if there exist $k$ spanning trees of $G$ rooted at $r$ that are pairwise independent. Zehavi and Itai conjectured that for every fixed integer $k \ge 1$, an undirected simple graph $G$ is $k$-vertex-connected if and only if, for every vertex $r \in V(G)$, $G$ contains $k$ \emph{independent spanning trees} rooted at $r$.


Zehavi--Itai conjecture had been known to hold for every $k \in \{1, 2, 3\}$~\cite{ItaiR88,CheriyanM88,ZI89}, and was later proven to hold also for $k=4$~\cite{CLY06}.
%\begin{lemma}[\cite{CLY06}]
    %Let $G$ be a $4$-vertex-connected graph, and let $r\in V(G)$. Then there exist four independent spanning trees of $G$ rooted at $r$.
%\end{lemma}

We note that, by a simple observation, the Itai--Zehavi conjecture implies that a graph $G$ is $k$-vertex-connected if and only if there exist $k$ distinct vertices $r_1,\ldots,r_k \in V(G)$ (rather than all vertices) such that, for each $i \in [k]$, $G$ contains $k$ independent spanning trees rooted at $r_i$. Suppose that $G$ contains such roots but is not $k$-vertex-connected, then there exists a vertex cut $C$ with $|C|<k$ such that $G-C$ is disconnected. Since $C$ has size less than $k$, it cannot contain all of $r_1,\ldots,r_k$, so some root $r^*$ remains in $G-C$. Since $G-C$ is disconnected, there exists a vertex $x$ that belongs to a component of $G-C$ different from the one containing $r^*$. 
%Let $x$ be a vertex in a component of $G-C$ different from the one containing $r^*$. 
This contradicts the existence of $k$ independent spanning trees in $G$ rooted at $r^*$, which implies that there are $k$ internally vertex-disjoint paths between $r^*$ and $x$, and hence no vertex cut of size less than $k$ can separate them.


%In~\cite{BFP21}, the authors certify $k$-vertex-connectivity for $k \in \{2,3\}$ using constructive characterizations based on \emph{open ear decompositions} and \emph{Mondshein sequences}. We again take a different route to certify $k$-vertex-connectivity for all $k \ge 2$.

%For $k$-vertex-connectivity, we rely on the equivalence conjectured by Zehavi and Itai~\cite{ZI89}: for every fixed integer $k \ge 1$, an undirected simple graph $G$ is $k$-vertex-connected if and only if, for every vertex $r \in V(G)$, $G$ contains $k$ \emph{independent spanning trees} rooted at $r$, meaning that for each vertex $s \in V(G)\setminus\{r\}$, the $k$ paths from $s$ to $r$ (one in each tree) are pairwise internally vertex-disjoint.

%Zehavi--Itai conjecture is known to hold for every $k \in \{1, 2, 3, 4\}$~\cite{ItaiR88,CheriyanM88,ZI89,CLY06}.
%We note that, to certify that $G$ is $k$-vertex-connected, it suffices to choose $k$ distinct roots $r_1,\ldots,r_k \in V(G)$ (rather than all vertices) such that, for each $i \in [k]$, the graph contains $k$ independent spanning trees rooted at $r_i$.
Given the above equivalence, certifying $4$-vertex-connectivity reduces to certifying that $24$ pairs of spanning trees rooted at a common vertex are independent. More generally, assuming~\Cref{conj: Itai--Zehavi}, the same reduction applies to certifying $k$-vertex-connectivity for every $k \ge 5$. In~\Cref{sec:kvc-upper}, we prove that $\Tilde{O}_k(\sqrt{n})$ bits suffice to certify two independent spanning trees rooted at the same vertex, which leads to the following theorem.



For $k=4$, our certification scheme works unconditionally, and there is no previously known non-trivial local certification scheme.

%\subsection{Graph connectivity}
%Let $G$ be a graph and $r$ be a vertex of $G$. Two spanning trees $T$ and $T'$ of $G$ are said to be \emph{independent} if for any vertex $v$ in $G$, the $v$--$r$ path in $T$ and the $v$--$r$ path in $T'$ are internally vertex-disjoint. We say that $G$ admits $k$ independent spanning trees rooted at $r$ if there exist $k$ spanning trees of $G$ rooted at $r$, say $T_1,\ldots,T_k$, that are pairwise independent.

%For $k=4$, it is known that $4$-vertex-connectivity is equivalent to having $4$ independent spanning trees rooted at every vertex.
%\begin{lemma}[\cite{CLY06}]
    %Let $G$ be a $4$-vertex-connected graph, and let $r\in V(G)$. Then there exist four independent spanning trees of $G$ rooted at $r$.
%\end{lemma}

%Itai and Zehavi~\cite{ZI89} conjectured that the equivalence also holds for $k\geq 5$.
%\begin{conjecture}[{Itai--Zehavi conjecture~\cite{ZI89}}]\label{conj: Itai--Zehavi}
    %A graph $G$ is $k$-vertex-connected if and only if for every vertex $r\in V(G)$, there exist $k$ independent spanning trees rooted at $r$.
%\end{conjecture}

%{\color{red}We note that, by a simple observation, the }
%Itai--Zehavi conjecture implies that a graph $G$ is $k$-vertex-connected if and only if there exist $k$ distinct vertices $r_1,\ldots,r_k \in V(G)$ (rather than all vertices) such that, for each $i \in [k]$, $G$ contains $k$ independent spanning trees rooted at $r_i$. Suppose that $G$ contains such roots but is not $k$-vertex-connected, then there exists a vertex cut $C$ with $|C|<k$ such that $G-C$ is disconnected. Since $C$ has size less than $k$, it cannot contain all of $r_1,\ldots,r_k$, so some root $r^*$ remains in $G-C$. {\color{red}Since $G-C$ is disconnected, there exists a vertex $x$ that belongs to a component of $G-C$ different from the one containing $r^*$ }
%This contradicts the existence of $k$ independent spanning trees in $G$ rooted at $r^*$, which implies that there are $k$ internally vertex-disjoint paths between $r^*$ and $x$, and hence no vertex cut of size less than $k$ can separate them.

%Itai--Zehavi conjecture implies that a graph $G$ is $k$-vertex connected if and only if there exist $k$ different vertices $r_1,\ldots,r_k$ in $G$ such that for each $i\in [k]$, there exist $k$ independent spanning trees rooted at $r_i$. Indeed, if we can remove fewer than $k$ vertices to disconnect the graph, this cut separates at least one of the vertices in $\{r_i : i \in [k]\}$ from some vertex $x \notin \{r_i : i \in [k]\}$. This yields a contradiction since $x$ and $r$ are connected by $k$ internally disjoint paths.

%For $k=4$, it is known that $k$-vertex-connectivity is equivalent to having $4$ independent spanning trees for $4$ different vertices. Zehavi--Itai conjectured that this holds for any larger $k$. 


Let us sketch the idea to certify that two spanning trees rooted at a common vertex are independent. The naive approach is that, for each vertex $u$, we send the information of $u$ to all its descendants in both trees; that is, we record all the information along the root-to-$v$ path. By doing so, the vertex can tell if there are any other vertices in the intersection of the two root-to-$v$ paths. It is only efficient when the tree has low depth.

To reduce complexity, we apply \emph{heavy-light decomposition}~\cite{SLEATOR1983362_heavy-light}, which partitions a tree into paths (called segments) such that each vertex belongs to the same segment as the child with the largest subtree. Heavy-light decomposition has been known as a general technique that yields efficient query algorithms on trees. In our application, heavy-light decomposition allows us to compress the tree into $O(\log n)$ layers, encode each path with at most $O(\log n)$ segments, and store the root-to-$v$ path encoding for each tree compactly. For each segment $S$ in the root-to-$v$ path, we want to bound the amount of information that $S$ should send to $v$.} \yx{not sure about the intuition or whether to add more details}

%We apply heavy-light decomposition to compress the tree into $O(\log n)$ layers and encode each path by a set of at most $O(\log n)$ segments, and we can store the root-to-$v$ path-encoding for each tree compactly. For each segment $S$ in the root-to-$v$ path, we want to bound the amount of information that $S$ should send to $v$. \yx{not sure about the intuition or whether to add more details}

A key observation is that for each vertex $u$ that belongs to segment $S_1$ in $T_1$ and segment $S_2$ in $T_2$, it suffices that one of the segments $S_i$ for $i \in \{1, 2\}$ takes the responsibility to send the information of $u$ to all its descendants in $T_i$. If a segment is short, then we can afford to let it take the responsibility, as the number of ancestors in a short segment is small. On the other hand, if a long segment takes the responsibility, then it must send the information of $u$ that also belongs to a long segment in the other tree. Intuitively, the amount of such information can be bounded, as we cannot have many long segments in each tree. Finally, we trade off the length of short segments and the number of long segments to obtain the desired bound.

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures-IST_cropped 1.pdf}
        \caption{Two spanning trees that are vertex-independent.}
        \label{fig: IST}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures-IST_cropped 2.pdf}
        \caption{Two spanning trees that are not vertex-independent}
        \label{fig: non-IST}
    \end{subfigure}
    \caption{Illustration of independent spanning trees. Both figures demonstrate two spanning trees in a ring rooted at the same vertex $r$, one in black and the other in dotted lines, oriented from the leaves to the root. In~\Cref{fig: IST}, both spanning trees are paths; the dotted one has $v_6$ as the leaf, and the other has $v_1$ as the leaf. The two trees are vertex-independent. In~\Cref{fig: non-IST}, the two trees are not vertex-independent (but still edge-independent) since the paths from $v_4$ (and also $v_5$) pass through $v_3$ in both trees.}
    \label{fig: IST-illustration}
\end{figure}

\begin{figure}[ht]
    \centering
    %\includegraphics[width=0.3\linewidth]{figures-heavy-light_cropped.pdf}
    \input{hldecomp}
    \caption{An illustration of the heavy-light decomposition. The segments are marked in black. For example, vertex $v$ has two children $v_1$ and $v_2$, and $v_1$ has more vertices in its subtree, and therefore belongs to the same segment as $v$. If a leaf does not belong to the same segment as its parent, it is itself considered a segment, see $v_3$.}
    \label{fig:heavy-light}
\end{figure}
\mtt{I use chatgpt to re-plot the previous figure. Please keep it only if it looks better.}

%\begin{restatable}{theorem}{thmKVC}\label{thm: k-vc-cert}
    %There exists an $O(k^3\sqrt{n}\log^{2.5}n)$-bit local certification scheme for $4$-vertex-connectivity. 
    %Moreover, assuming the Itai--Zehavi conjecture (\Cref{conj: Itai--Zehavi}), the same bound holds for every $k \ge 5$.
    %This holds also for any $k\geq 5$ assuming the Itai--Zehavi conjecture (\Cref{conj: Itai--Zehavi}).
%\end{restatable}

Since the upper bound for $k$-vertex-connectivity is $\Tilde{O}_k(\sqrt{n})$, while the lower bound we get is $\Omega_k(\log n)$, a natural question to ask is whether we can do better using the independent tree approach. We prove that given a labeled graph where each vertex receives two IDs that point to its parents in $T_1$ and $T_2$, certifying that $T_1$ and $T_2$ are independent spanning trees rooted at the same vertex in $G$ requires $\Omega(\sqrt{n})$ bits.

\begin{restatable}{theorem}{thmIndepST}\label{thm: indep-st-lower}
    Given a graph $G$ and two spanning trees $T_1$ and $T_2$ rooted at the same vertex $r$, certifying $T_1$ and $T_2$ are independent requires $\Omega(\sqrt{n})$ bits.
\end{restatable}

In view of \cref{thm: indep-st-lower}, the analysis of \cref{thm: k-vc-cert} is bottleneck-tight for every constant $k \ge 4$.



\subsubsection{Additional results for $2$-edge-connectivity and $2$-vertex-connectivity in the anonymous model}
\yx{the title may be changed.}
\yx{motivation need to be revised.}
{\color{blue}
Recall that our lower bound in~\Cref{thm: k-conn-lower} only works for $k\ge 3$. It is natural to ask whether $O(\log n)$ is the right complexity for certifying $2$-edge-connectivity (or $2$-vertex-connectivity). Can we get a sub-logarithmic upper bound on the restricted graph class? Or can we get a super-constant lower bound? In~\Cref{sec: 2-conn-bdd-deg}, we partially answer this question. On the upper bound side, we provide a constant-bit certification scheme for certifying $2$-edge-connecitivity and $2$-vertex-connectivity on bounded-degree graphs. Moreover, we show that for $2$-edge-connectivity, the certification scheme can be extended to bounded-expansion graphs (which includes planar graphs, and more generally, minor-free graph classes) using a very recent result in~\cite{BFVZ26}. On the other hand, we proved a super-constant lower bound for certifying $2$-vertex-connectivity via a slight modification of the lower bound for parity certification in~\cite{BFVZ26}.

\paragraph{Breaking the logarithmic barrier in restricted graph classes.}
Given a graph $G$, we say that an edge $e$ is a \emph{bridge} of $G$ if removing $e$ increases the number of connected components in $G$. A graph is \emph{bridgeless} if it does not contain a bridge. Our first observation is that $2$-edge-connectivity admits a constant-bit edge-certification scheme via a simple application of the fact that any bridgeless graph can be covered by a constant number of (possibly disconnected) Eulerian subgraphs.

\begin{restatable}{lemma}{lemTwoECedge}\label{lem: 2-ec-EdgeCert}
    There exists an $O(1)$-bit edge-certification scheme for $2$-edge connectivity.
\end{restatable}

On bounded degree graphs, the edge certification scheme can be transformed into a vertex certification scheme with an {\color{red}$\Tilde{O}(\Delta)$} overhead\footnote{In this paper, we will write explicitly the dependency on $\Delta$ in the Theorems whenever possible. In distributed graph algorithms, it is natural to consider graph classes with bounded degree. For local certification schemes, the first non-trivial bound with dependency in the max-degree $\Delta$ was given in~\cite{BFZ25}.}. 

\begin{restatable}{theorem}{thmTwoEC}\label{thm: 2-edge-conn}
    There exists an {\color{red}$O(\Delta\log\Delta)$}-bit local certification scheme for $2$-edge-connectivity on bounded-degree graphs.
\end{restatable}

This result improves upon~\cite{BFP21} when restricted to bounded-degree graphs. Their $O(\log n)$-bit local certification scheme for $2$-edge-connectivity essentially ``describes'' an ear decomposition of the graph, and simulating the ordering of the added ear may require $O(\log n)$ bits, even when the graph has constant degree. For more details, see Lemma 20 and Corollary 21 of~\cite{BFP21}.

\yx{say that 2-conn is fundamentally different from k ge 3}
}


%can be certified with complexity that depends only on $\Delta$, where $\Delta$ is the maximum degree of the input graph. 

%{\color{red}In distributed graph algorithms, it is natural to consider graph classes with bounded degree.\yx{cite papers??} For local certification schemes, the first non-trivial bound with dependency in the max-degree $\Delta$ was given in~\cite{BFZ25}. We show that $2$-edge-connectivity and $2$-vertex-connectivity can both be certified with complexity that depends only on $\Delta$.}

%For $2$-edge-connectivity, it is known that any bridgeless graph can be covered by a constant number of (possibly disconnected) Eulerian subgraphs (see \cref{lem: Eulerian-cover}), which leads to a constant-bit local certification scheme on edges. 

%On bounded degree graphs, the edge certification scheme can be transformed into a vertex certification scheme with an {\color{red}$\Tilde{O}(\Delta)$} overhead. {\color{red}For bounded degree graph, this result improves upon~\cite{BFP21}, which introduced an $O(\log n)$-bit local certification scheme for $2$-edge-connectivity. As their certification scheme essentially ``describes'' an ear decomposition of the graph, simulating the ordering of the added ear may require $O(\log n)$ bits, even when the graph has constant degree. For more details, see Lemma 20 and Corollary 21 of~\cite{BFP21}.}

For $2$-vertex-connectivity, we also obtain a constant-bit local certification scheme for bounded degree graphs by a reduction to $2$-edge-connectivity. Intuitively, we replace each vertex with an edge and split its neighbors into two nonempty sets, each connecting to a different endpoint of the edge. Observe that if the original graph is $2$-vertex-connected, then the modified graph is $2$-edge-connected regardless of how we partition the neighborhood. Conversely, we prove that if all such graphs are $2$-edge-connected, then the original graph is $2$-vertex-connected. We note that the converse direction works only for $2$-vertex connectivity, and thus the reduction cannot be generalized to certify higher connectivity.\yx{not sure whether to discuss this}
%For $2$-vertex-connectivity, we also obtain a constant-bit local certification scheme for bounded degree graphs by a reduction to $2$-edge-connectivity. Intuitively, we consider a vertex cut in the graph. If we can correctly guess how the neighbors are separated into two parts, then making those vertices into edges that connect the two parts will result in a graph that transforms vertex-connectivity to edge-connectivity. The problem is how we can simultaneously guess the neighborhood partition for all potential vertex cuts, and it can be done when we only need to tell whether the graph admits a cut vertex or not.
\begin{restatable}{theorem}{thmTwoVC}\label{thm: 2-vertex-conn}
    There exists an {\color{red}$O(2^{\Delta}\cdot\Delta\log\Delta)$}-bit local certification scheme for $2$-vertex-connectivity on bounded-degree graphs.
\end{restatable}

{\color{blue}
The main obstacle to extending~\Cref {thm: 2-edge-conn} to general graphs was that transforming edge-certification schemes to vertex-certification schemes requires vertices to distinguish certificates from different incident edges. In the previous work~\cite{FFM+23}, they showed that when the graph admits an edge-partition into a constant number of pseudoforests\footnote{In their paper, they use degeneracy as the parameter, which is equivalent to pseudoarboricity (the minimum number of pseudoforests into which its edges can be partitioned) within a factor of $2$.} and the certificates are of size $\Omega(\log n)$, an edge-certification scheme can be transformed into a vertex-certification scheme with only a constant blowup. However, in the case where the certificate size is $o(\log n)$, an additive $O(\log n)$ term is required.

A \emph{pseudoforest} is a graph where each connected component has at most one cycle, and a \emph{pseudoforest decomposition} of a graph is a partition of the edges such that each component of the partition induces a pseudoforest. We note that, in~\cite{FFM+23}, the additive $O(\log n)$ overhead comes from the cost of encoding the parent-children relationship in a pseudoforest decomposition by writing the parents' IDs on each vertex.


We show that for bounded expansion graphs, this obstacle can be overcome, and in particular, we have a constant-bit local certification scheme for $2$-edge-connectivity in the anonymous model. Bounded expansion graphs contain a broad range of well-studied graph classes, such as bounded degree graphs, planar graphs, and more generally, minor-closed graphs. The formal definition will be given in~\Cref{sec: 2-conn-bdd-deg}. We sketch the main idea as follows.

We first observe that, as long as a partition of edges into a constant number of pseudoforests is given as input to the vertices (in the sense that each vertex has at most one parent in each pseudoforest, and they have the knowledge of their own parent and children in each pseudoforest), transforming edge-certification to vertex-certification incurs only a constant overhead by letting the children take the responsibility of simulating the edge connected to the parent.

In~\cite{BFVZ26}, they show that for bounded expansion graphs, there exists a way of encoding the parent-children relationship in a certain pseudoforest using only constant bits via conflict-free coloring. Our main idea is to apply their pseudoforest certification scheme to simultaneously encode a \emph{sparse certificate} for $2$-edge-connectivity (which is a sparse subgraph that is $2$-edge-connected if and only if the original graph is) and a pseudoforest decomposition on top of it. Then we apply the edge-certification scheme in~\Cref{lem: 2-ec-EdgeCert} to the sparse certificate and then transform it into a constant-bit vertex-certification scheme.

\begin{restatable}{theorem}{thmTwoECnew}\label{thm: 2-ec-bdd-expansion}
    Let $\Fcal$ be a bounded-expansion graph class. Given the promise that the input graph belongs to $\Fcal$, there exists an $O_\Fcal(1)$-bit local certification scheme for $2$-edge-connectivity, where the constant only depends on the graph class $\Fcal$.
\end{restatable}

\begin{remark}\label{rmk: 2VC-to-2EC}
    Recall that in~\Cref{thm: 2-vertex-conn}, our reduction relies on enumerating all possible partitions of each vertex's neighborhood. Therefore, it cannot be directly generalized to bounded expansion graphs.
\end{remark}


\paragraph{A super-constant lower bound for $2$-vertex connectivity in the anonymous model.}
Our lower bound for $2$-vertex-connectivity is a slight modification of the parity lower bound in~\cite{BFVZ26}. In~\cite{BFVZ26}, the task was to certify that a graph has an even number of nodes. Their approach is to construct the  ``powerset graph'' and then glue two such graphs of even size together by identifying two nodes, one from each graph. The powerset graphs $G=(V,E)$ are bipartite graphs constructed as follows. Let $V=V_1\cup V_2$ where $V_1=[m]$ is the ground set of $m$ elements. For each subset $S\subseteq [m]$, itnroduce a vertex $v_S$ to $V_2$, and connect $v_S$ to every vertex $i\in S\subseteq V_1$. According to the finite unions theorem, they prove that if the number of labels is $o(\log^*n)$ where $n=|V|$, then there exist two subsets $S_1$ and $S_2$ such that $v_{S_1}$, $v_{S_2}$, and $v_{S_1\cup S_2}$ are colored the same. Since we are in the anonymous model, they simply take two copies of $G$, denoted by $G_1$ and $G_2$, and then identify $v_{S_1}$ in $G_1$ and $v_{S_2}$ in $G_2$ to obtain a graph $G'$ with an odd number of vertices. Notice that the identified vertex has the same view as $v_{S_1\cup S_2}$, and therefore all vertices still output \accept in $G'$. Our lower bound for $2$-vertex-connectivity follows from the observation that the construction of $G$ can be made $2$-vertex-connected, and that the combined graph $G'$ has a cut vertex (which is the identified one).

\begin{restatable}{theorem}{thmTwoVCLB}\label{thm: 2-vc-lb}
    Certifying $2$-vertex-connectivity requires $\Omega(\log(\log^*n))$ bits in the anonymous model.
\end{restatable}

We note that, since our lower bound graph for $2$-vertex-connectivity is not of bounded degeneracy,~\Cref{thm: 2-ec-bdd-expansion} and~\Cref{thm: 2-vc-lb} are incomparable.

}
 





==> intro-PODC_vers.tex <==
\section{Introduction}

High edge and vertex connectivity are fundamental algorithmic resources in distributed networks.
They underlie sparse connectivity certificates and distributed min-cut algorithms, where the value of the edge connectivity $\lambda$ guides sampling and sparsification~\cite{Thu95,GK13,DHNS19}.
They also enable communication structures: highly edge-connected graphs support many spanning-tree-based backbones, while highly vertex-connected graphs support analogous connected-dominating-set structures, with applications to high-throughput information dissemination and oblivious routing~\cite{CGK14}.
Recent algorithms further use high connectivity to build efficient communication backbones for tasks such as minimum spanning tree and multi-message broadcast~\cite{CPT20,CCDGHL24}.
In these applications, a certified lower bound on the connectivity lets the algorithm choose its parameters, build the required number of backbones, and rely on the promised level of fault tolerance without first estimating the connectivity.
This motivates the verification question studied here: can a connected distributed network locally certify, using short labels, that it is $k$-edge-connected or $k$-vertex-connected for a prescribed value of $k$?


\yx{Some notes about the intended change for intro:
- Define the model anonymous/ PLS/ LCP as anonymous/ KT0/ KT1, define them formally here\\
- arrangement: general upper bound (edge, vertex) -> lower bound for k>2 -> additional 2-conn results, write as a story\\
- for k-vc, define IST and the conjecture here formally before the theorem
}

Local certification is a mechanism that enables a network to verify a global property $\mathcal{P}$ using only local information. Informally, a local certification scheme consists of a prover, which assigns labels to the vertices, and a distributed verification algorithm, which examines the local view of each vertex and decides whether to accept or reject. If a network configuration satisfies $\mathcal{P}$, then there must exist a labeling under which every vertex accepts. Conversely, if the configuration does not satisfy $\mathcal{P}$, then for every possible labeling, at least one vertex must reject. The goal is to design compact local certification schemes for a given property, with label size as small as possible.
\mtt{This paragraph does not look like a beginning paragraph.}

%Local certification is a mechanism that allows a network to verify certain global properties $\Pcal$ using only local information. Informally, a local certification scheme can be described as a prover that assigns labels to the vertices, and a distributed verification algorithm that takes as input the local view of a vertex and decides whether to accept or reject. Whenever a network configuration satisfies $\Pcal$, there should be a labeling such that the verification passes on every vertex in the network, whereas if the network configuration does not satisfy $\mathcal{P}$, then no matter how the prover labels the vertices, the verification will fail on some vertices. The goal is to design a compact local certification for some given property with a small label size.
%\mtt{How about replacing ``is correct'' with ``satisfies $\mathcal{P}$''} 

Local certification provides us with a framework to achieve error detection. It was first proposed as a building block of a self-stabilizing algorithm to certify the solution under transient faults~\cite{KKP05}. In particular, space complexity is an important measurement of a self-stabilizing algorithm, and there has been work that makes black-box use of compact local certification schemes to design compact self-stabilizing algorithms~\cite{BFP14}. However, certifying the structure of a network itself is also important, as running distributed algorithms and certifying their solutions may be simpler in certain graph classes.

{\color{red}In this paper, we study \emph{graph connectivity} in the local certification scheme. The \emph{edge (resp. vertex) connectivity} of an undirected graph is the size of the minimum edge (resp. vertex) cut, which is defined to be the minimum number of edges (resp. vertices) whose removal disconnects the graph. Connectivity captures the robustness of a network. Finding the connectivity of a graph is a fundamental problem that has been extensively studied in graph algorithms.\yx{cite some papers here} Our goal is to certify that a network has edge or vertex connectivity at least $k$ for some fixed value $k$.}
\yx{I try to motivate this paper first by saying that connectivity is a fundamental problem, and say that it has been used in the minor-closed certification problem. Im not sure whether itis better or not.}

{\color{red}Certifying graph connectivity has also been motivated in the prior work~\cite{BFP21} that tried to answer the problem of whether every minor-closed graph property admits an $O(\log n)$ local certification scheme~\cite{Feu21}. Certifying minor-closed properties are important open question in this field that has received great attention. Several natural graph classes are captured by minor-closed properties, including planar graphs, bounded genus graphs, and bounded tree-width graphs. Working towards this goal, it has been shown that planar graphs and bounded genus graphs can be certified in $O(\log n)$ bits~\cite{FFM+23, FFM+20, esperet2022local}. There are also meta-theorems showing that a broad class of properties can be certified efficiently in certain minor-closed graph classes~\cite{CKM25}.\yx{cite other meta-theorem papers} However, certifying general minor-closed properties remained wide open. In~\cite{BFP21}, graph connectivity has been used as a building block to show that minor-free graphs with some small-sized forbidden minors admit $O(\log n)$-bit certification schemes. They first showed that certifying $2$-edge connectivity, $2$-vertex connectivity, and $3$-vertex connectivity can be done in $O(\log n)$ bits. They then decomposed the graphs into $2$-vertex-connected (or $3$-vertex-connected) components and showed that small-sized minor-free graph classes have restricted structures in those connected components that admit efficient certification schemes. With the hope that the local certification schemes for graph connectivity may be useful in certifying more complicated minor-closed graph classes,~\cite{BFP21} posed the following questions:}
\yijun{elaborate a bit to further motivate connectivity certification?}
%One important open problem in this field is whether every minor-closed graph property admits an $O(\log n)$ local certification scheme~\cite{Feu21}. Minor-closed properties capture several natural graph classes, including planar graphs, bounded genus graphs, and bounded tree-width graphs, and many problems admit more efficient distributed algorithms and certification schemes in certain minor-closed graph classes~\cite{HLZ22, cha23, CKM25}. Working towards this goal, it has been shown that planar graphs and bounded genus graphs can be certified in $O(\log n)$ bits~\cite{FFM+23, FFM+20, esperet2022local}. Minor-free graphs with some small-sized minors are also proven to have $O(\log n)$-bit certification schemes~\cite{BFP21}. 

%It was left as an open question in~\cite{BFP21} to understand the complexity of certifying $k$-vertex-connectivity. As stated in~\cite{BFP21}, the importance of certifying $k$-vertex-connectivity is twofold. First, they show that certifying both $2$-edge-connectivity and $2$-vertex-connectivity can be done in $O(\log n)$ bits, and also certifying $3$-vertex-connectivity can be done in $O(\log n)$ bits. % on vertices. % and $O(1)$ bits on edges. 
%Certifying $2$-vertex-connected components and $3$-vertex-connected components are then used as building blocks\yijun{elaborate a bit to further motivate connectivity certification?} to certify minor-free graph classes; therefore, certifying $k$-vertex-connected components may be a useful tool to certify other, more complicated graph classes. Second, since robustness is a nice property of a network and can be captured by connectivity, certifying $k$-vertex-connectivity is of independent interest as well. In particular, we establish some tools and results toward the following questions: 
\begin{problem}[{\cite[Question 57]{BFP21}}]\label{ques1}
    Does the certification for $k$-vertex-connectivity require $\Omega(\log n)$ bits for any $k\geq 2$?
\end{problem}
\begin{problem}[{\cite[Question 58]{BFP21}}]\label{ques2}
    Can $k$-vertex-connectivity be certified with $O(\log n)$ bits for any $k\geq 4$?
\end{problem}


%In this paper, we work towards the goal of certifying $k$-edge/vertex-connectivity for any value of $k$. {\color{red}The input graphs are assumed to be connected.} A summary of our results can be found in~\Cref{tab: results}.
In this paper, we established several new results and tools towards certifying $k$-edge/vertex-connectivity for any fixed value of $k$. {\color{red}The input graphs are assumed to be connected.}\mtt{Consider to mention that this is a norm in the field.} A summary of our results can be found in~\Cref{tab: results}.

\subsection{General Graphs}

We answer \Cref{ques1} affirmatively by proving \cref{thm: k-conn-lower} using the crossing technique introduced in~\cite{GS16}. The intuition is that we consider a $k$-edge/vertex-connected graph that has a special edge, {\color{red}where both endpoints have a bounded number of neighbors, and consider $\Theta(n)$ copies of such a graph} on different identifier sets. If the proof size is $o(\log n)$, then there must exist a constant number of copies receiving identical label assignments in the neighborhood of the special edges. We pick two such copies and glue them together to create a new accepting graph with low connectivity by removing the special edges and reconnect each endpoint to the copy of its neighbor (originally incident to the special edge) in the other copy of graph. This results in a graph with connectivity $2$ (both edge and vertex) but all vertices still accept due to identical labels in their neighborhoods.
%We answer \Cref{ques1} affirmatively by proving \cref{thm: k-conn-lower} using the crossing technique introduced in~\cite{GS16}. The intuition is that if a $k$-edge/vertex-connected graph has an edge with a bounded neighborhood, then we consider $\Theta(n)$ such instances. If the proof size is $o(\log n)$, then there must exist a constant number of instances receiving identical labels in the neighborhood of that edge, and we can pick two of them, cut the edges, and glue them together, which results in a graph with connectivity $2$ (both edge and vertex) but all vertices still accept due to identical labels in their neighborhoods.

\begin{restatable}{theorem}{thmKConnLower}\label{thm: k-conn-lower}
    For any integer $k\geq 3$, certifying $k$-edge-connectivity and $k$-vertex-connectivity both require $\Omega((\log n)/k)$ bits.
\end{restatable}


We then devise an optimal local certification scheme for $k$-edge-connectivity for any constant $k \ge 3$ in \cref{sec:optimal}. Next, in \cref{sec:bottlenecktight}, we devise a bottleneck-tight local certification scheme for $k$-vertex-connectivity for $k=4$ (and, more generally, for any constant $k \ge 5$ assuming the Zehavi--Itai conjecture), thereby partially answering \Cref{ques2}.

%, we first construct a local certification scheme for a sparse subgraph that preserves $k$-vertex-connectivity (called a \emph{sparse certificate}). %It has been shown that iteratively finding $k$ BFS forest results in a sparse certificate for both $k$-edge- and $k$-vertex-connectivity~\Cref{lem: sparse-cert-iff}. Therefore, the local certification can be done by iteratively certifying BFS spanning forests.
%\begin{restatable}{lemma}{lemSparseCert}\label{lem: cert-sparse-cert}
%    There exists an $O(k\log n)$-bit local certification scheme for a sparse certificate of both $k$-edge-connectivity and $k$-vertex-connectivity.
%\end{restatable}
%Given the sparse certificate, any edge-certification scheme can be transformed into a vertex-certification scheme efficiently~\cref{lem:EdgeCert-degeneracy}. 

%In~\cite{BFP21}, they give a local certification scheme for $3$-vertex-connectivity using $O(\log n)$ bits on vertices and $O(1)$ bits on edges. As a corollary of \Cref{lem: cert-sparse-cert}, we can restrict ourselves to bounded arboricity graphs, and thus improve the complexity to $O(\log n)$ bits on vertices only.
%\begin{restatable}{corollary}{corThreeVC}\label{cor: 3-vc}
%    The complexity of certifying $3$-vertex-connectivity is $\Theta(\log n)$.
%\end{restatable}

\subsubsection{An optimal local certification scheme for $k$-edge-connectivity}\label{sec:optimal}

In~\cite{BFP21}, the authors certify $2$-edge-connectivity via a constructive characterization known as an \emph{ear decomposition}. We take a different route to certify $k$-edge-connectivity for all $k \ge 2$.

For even $k \ge 2$, we use the classical equivalence: an undirected simple graph $G$ is $k$-edge-connected if and only if $G$ admits an orientation $\vec{G}$ that is $(k/2)$-arc-strongly connected~\cite{Robbins39,NashWilliams60}. We then apply Edmonds' branching theorem~\cite{Edmonds73} to reduce the task to certifying $k/2$ pairwise arc-disjoint out-branchings and $k/2$ pairwise arc-disjoint in-branchings rooted at a common vertex, which can be done using $O(k\log n)$ bits.

For odd $k \ge 3$, we use another equivalence: $G$ is $k$-edge-connected if and only if there exists a partition of $E(G)$ into sets $E_1,E_2,\ldots,E_{\ell_k}$ such that $G\setminus E_i$ is $(k-1)$-edge-connected for every $i \in [\ell_k]$. In~\cite{DeVosJS03}, DeVos, Johnson, and Seymour showed that one may take $\ell_k \le 81^{k^2}$, and they further claimed (without proof) that this bound can be reduced to $\ell_k = 2^{O(k)}$. For small values of $k$, it is known that $\ell_3 \le 9$ and $\ell_5 \le 30$.

%Goedgebeur, M{\'{a}}cajov{\'{a}}, and Renders show that $\ell_3 \le 4$


%{\color{red}(To be aligned with corresponding sections)}

\begin{restatable}{theorem}{thmkEC}\label{thm: k-ec}
    For any integer $k \ge 2$, there exists an $O(k \log n)$-bit local certification scheme for $k$-edge-connectivity when $k$ is even, and an $O(81^{k^2}k\log n)$-bit local certification scheme when $k$ is odd.
\end{restatable}

Given \cref{thm: k-conn-lower}, we know that \cref{thm: k-ec} is optimal for every constant $k \ge 3$.

%\mtt{The dependence on $k$ may be as large as $81^{k^2}$. Did we remove this dependence?}\yijun{I suggest that we keep the dependence on $k$ (and also max deg $\Delta$) whenever possible.}

\subsubsection{A bottleneck-tight local certification scheme for $k$-vertex-connectivity}\label{sec:bottlenecktight}

In~\cite{BFP21}, the authors certify $k$-vertex-connectivity for $k \in \{2,3\}$ using constructive characterizations based on \emph{open ear decompositions} and \emph{Mondshein sequences}. We again take a different route to certify $k$-vertex-connectivity for all $k \ge 2$.

For $k$-vertex-connectivity, we rely on the equivalence conjectured by Zehavi and Itai~\cite{ZI89}: for every fixed integer $k \ge 1$, an undirected simple graph $G$ is $k$-vertex-connected if and only if, for every vertex $r \in V(G)$, $G$ contains $k$ \emph{independent spanning trees} rooted at $r$, meaning that for each vertex $s \in V(G)\setminus\{r\}$, the $k$ paths from $s$ to $r$ (one in each tree) are pairwise internally vertex-disjoint.
Zehavi--Itai conjecture is known to hold for every $k \in \{1, 2, 3, 4\}$~\cite{ItaiR88,CheriyanM88,ZI89,CLY06}.
We note that, to certify that $G$ is $k$-vertex-connected, it suffices to choose $k$ distinct roots $r_1,\ldots,r_k \in V(G)$ (rather than all vertices) such that, for each $i \in [k]$, the graph contains $k$ independent spanning trees rooted at $r_i$.
Given the above equivalence, certifying $4$-vertex-connectivity reduces to certifying that $24$ pairs of spanning trees rooted at a common vertex are independent. More generally, assuming the conjecture, the same reduction applies to certifying $k$-vertex-connectivity for every $k \ge 5$.

%the idea of certifying $k$ independent spanning trees for $k$ different vertices. 


%For $k=4$, it is known that $k$-vertex-connectivity is equivalent to having $4$ independent spanning trees for $4$ different vertices. Zehavi--Itai conjectured that this holds for any larger $k$. 

%We use a heavy-light decomposition to further reduce the size of certificates to $\Tilde{O}_k(\sqrt{n})$.

To certify that two spanning trees rooted at a common vertex are independent, the naive approach is that, for each vertex $u$, we send the information of $u$ to all its descendants in both trees; that is, we record all the information along the root-to-$v$ path. By doing so, the vertex can tell if there are any other vertices in the intersection of the two root-to-$v$ paths. It is only efficient when the tree has low depth.

{\color{red}To reduce complexity, we apply \emph{heavy-light decomposition}~\cite{SLEATOR1983362_heavy-light}, which partitions a tree into paths (called segments) such that each vertex belongs to the same segment as the child with the largest subtree. Heavy-light decomposition has been known as a general technique that yields efficient query algorithms on trees. In our application, heavy-light decomposition allows us to compress the tree into $O(\log n)$ layers, encode each path with at most $O(\log n)$ segments, and store the root-to-$v$ path encoding for each tree compactly. For each segment $S$ in the root-to-$v$ path, we want to bound the amount of information that $S$ should send to $v$.} \yx{not sure about the intuition or whether to add more details}

%We apply heavy-light decomposition to compress the tree into $O(\log n)$ layers and encode each path by a set of at most $O(\log n)$ segments, and we can store the root-to-$v$ path-encoding for each tree compactly. For each segment $S$ in the root-to-$v$ path, we want to bound the amount of information that $S$ should send to $v$. \yx{not sure about the intuition or whether to add more details}

A key observation is that for each vertex $u$ that belongs to segment $S_1$ in $T_1$ and segment $S_2$ in $T_2$, it suffices that one of the segments $S_i$ for $i \in \{1, 2\}$ takes the responsibility to send the information of $u$ to all its descendants in $T_i$. If a segment is short, then we can afford to let it take the responsibility, as the number of ancestors in a short segment is small. On the other hand, if a long segment takes the responsibility, then it must send the information of $u$ that also belongs to a long segment in the other tree. Intuitively, the amount of such information can be bounded, as we cannot have many long segments in each tree. Finally, we trade off the length of short segments and the number of long segments to obtain the desired bound.

\yx{I add a figure for IST here but not sure whether to move it to prelim.}
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures-IST_cropped 1.pdf}
        \caption{Two spanning trees that are vertex-independent.}
        \label{fig: IST}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures-IST_cropped 2.pdf}
        \caption{Two spanning trees that are not vertex-independent}
        \label{fig: non-IST}
    \end{subfigure}
    \caption{Illustration of independent spanning trees. Both figures demonstrate two spanning trees in a ring rooted at the same vertex $r$, one in black and the other in dotted lines, oriented from the leaves to the root. In~\Cref{fig: IST}, both spanning trees are paths; the dotted one has $v_6$ as the leaf, and the other has $v_1$ as the leaf. The two trees are vertex-independent. In~\Cref{fig: non-IST}, the two trees are not vertex-independent (but still edge-independent) since the paths from $v_4$ (and also $v_5$) pass through $v_3$ in both trees.}
    \label{fig: IST-illustration}
\end{figure}

\yx{I add a figure for hevay-light decomp here but not sure whether to move it to prelim.}

\begin{figure}[ht]
    \centering
    %\includegraphics[width=0.3\linewidth]{figures-heavy-light_cropped.pdf}
    \input{hldecomp}
    \caption{An illustration of the heavy-light decomposition. The segments are marked in black. For example, vertex $v$ has two children $v_1$ and $v_2$, and $v_1$ has more vertices in its subtree, and therefore belongs to the same segment as $v$. If a leaf does not belong to the same segment as its parent, it is itself considered a segment, see $v_3$.}
    \label{fig:heavy-light}
\end{figure}
\mtt{I use chatgpt to re-plot the previous figure. Please keep it only if it looks better.}

\begin{restatable}{theorem}{thmKVC}\label{thm: k-vc-cert}
    There exists an $O(k^3\sqrt{n}\log^{2.5}n)$-bit local certification scheme for $4$-vertex-connectivity. 
    Moreover, assuming the Itai--Zehavi conjecture (\Cref{conj: Itai--Zehavi}), the same bound holds for every $k \ge 5$.
    %This holds also for any $k\geq 5$ assuming the Itai--Zehavi conjecture (\Cref{conj: Itai--Zehavi}).
\end{restatable}

Since the upper bound for $k$-vertex-connectivity is $\Tilde{O}_k(\sqrt{n})$, while the lower bound we get is $\Omega_k(\log n)$, a natural question to ask is whether we can do better using the independent tree approach. We prove that given a labeled graph where each vertex receives two IDs that point to its parents in $T_1$ and $T_2$, certifying that $T_1$ and $T_2$ are independent spanning trees rooted at the same vertex in $G$ requires $\Omega(\sqrt{n})$ bits.

\begin{restatable}{theorem}{thmIndepST}\label{thm: indep-st-lower}
    Given a graph $G$ and two spanning trees $T_1$ and $T_2$ rooted at the same vertex $r$, certifying $T_1$ and $T_2$ are independent requires $\Omega(\sqrt{n})$ bits.
\end{restatable}

In view of \cref{thm: indep-st-lower}, the analysis of \cref{thm: k-vc-cert} is bottleneck-tight for every constant $k \ge 4$.

\subsection{Bounded-Degree Graphs}
{\color{red}In distributed graph algorithms, it is natural to consider graph classes with bounded degree.\yx{cite papers??} For local certification schemes, the first non-trivial bound with dependency in the max-degree $\Delta$ was given in~\cite{BFZ25}. We show that $2$-edge-connectivity and $2$-vertex-connectivity can both be certified with complexity that depends only on $\Delta$.}

For $2$-edge-connectivity, it is known that any bridgeless graph can be covered by a constant number of (possibly disconnected) Eulerian subgraphs (\cref{lem: Eulerian-cover}), which leads to a constant-bit local certification scheme on edges. On bounded degree graphs, the edge certification scheme can be transformed into a vertex certification scheme with an {\color{red}$\Tilde{O}(\Delta)$} overhead. {\color{red}For bounded degree graph, this result improves upon~\cite{BFP21}, which introduced an $O(\log n)$-bit local certification scheme for $2$-edge-connectivity. As their certification scheme essentially ``describes'' an ear decomposition of the graph, simulating the ordering of the added ear may require $O(\log n)$ bits, even when the graph has constant degree. For more details, see Lemma 20 and Corollary 21 of~\cite{BFP21}.}
\begin{restatable}{theorem}{thmTwoEC}\label{thm: 2-edge-conn}
    There exists an {\color{red}$O(\Delta\log\Delta)$}-bit local certification scheme for $2$-edge-connectivity on bounded-degree graphs.
\end{restatable}


For $2$-vertex-connectivity, we also obtain a constant-bit local certification scheme for bounded degree graphs by a reduction to $2$-edge-connectivity. Intuitively, we replace each vertex with an edge and split its neighbors into two nonempty sets, each connecting to a different endpoint of the edge. Observe that if the original graph is $2$-vertex-connected, then the modified graph is $2$-edge-connected regardless of how we partition the neighborhood. Conversely, we prove that if all such graphs are $2$-edge-connected, then the original graph is $2$-vertex-connected. We note that the converse direction works only for $2$-vertex connectivity, and thus the reduction cannot be generalized to certify higher connectivity.\yx{not sure whether to discuss this}
%For $2$-vertex-connectivity, we also obtain a constant-bit local certification scheme for bounded degree graphs by a reduction to $2$-edge-connectivity. Intuitively, we consider a vertex cut in the graph. If we can correctly guess how the neighbors are separated into two parts, then making those vertices into edges that connect the two parts will result in a graph that transforms vertex-connectivity to edge-connectivity. The problem is how we can simultaneously guess the neighborhood partition for all potential vertex cuts, and it can be done when we only need to tell whether the graph admits a cut vertex or not.
\begin{restatable}{theorem}{thmTwoVC}\label{thm: 2-vertex-conn}
    There exists an {\color{red}$O(2^{\Delta}\cdot\Delta\log\Delta)$}-bit local certification scheme for $2$-vertex-connectivity on bounded-degree graphs.
\end{restatable}

 

\begin{table}
    \centering
    \begin{tabular}{m{17em}m{12em}m{10em}}

        Task & Complexity & Reference\\ 
        \midrule
        \midrule
        
        \multirow{2}{16em}{$2$-edge-connectivity}
         & $O(\log n)$ & \cite{BFP21} \\ 
         & {\color{red}$O(\Delta\log\Delta)$} & \Cref{thm: 2-edge-conn} \\ 
        \addlinespace[8pt]
        \multirow{3}{16em}{$k$-edge-connectivity, $k\geq 3$}
         & $\Omega((\log n)/k)$ & \Cref{thm: k-conn-lower}\\
         & $O(k\log n)$, $k$ even & \Cref{thm: k-ec}  \\
         & $O(81^{k^2} k \log n)$, $k$ odd & \Cref{thm: k-ec} \\
        %\addlinespace[8pt]
        \midrule
        
        \multirow{2}{16em}{$2$-vertex-connectivity}
         & $O(\log n)$ & \cite{BFP21} \\
         & {\color{red}$O(2^\Delta\cdot\Delta\log\Delta)$} & \Cref{thm: 2-vertex-conn} \\
        \addlinespace[8pt]

        $3$-vertex-connectivity & $O(\log n)$  & \cite{BFP21} \\
        %$3$-vertex-connectivity & $O(\log n)$ on vertices and $O(1)$ on edges & \cite{BFP21} \\
        % & $O(\log n)$ & \Cref{cor: 3-vc}\\
        \addlinespace[8pt]
        $4$-vertex-connectivity & $O(k^3\sqrt{n}\log^{2.5}n)$ & \Cref{thm: k-vc-cert} \\
        \addlinespace[8pt]
        $k$-vertex-connectivity, $k\geq 5$ & $O(k^3\sqrt{n}\log^{2.5}n)$ assuming Itai--Zehavi conjecture & \Cref{thm: k-vc-cert} \\
        \addlinespace[8pt]
        $k$-vertex-connectivity, $k \ge 3$ & $\Omega((\log n)/k)$ & \Cref{thm: k-conn-lower} \\
        \addlinespace[8pt]
        Two independent spanning trees & $\Omega(\sqrt{n})$ & \Cref{thm: indep-st-lower}\\
        \bottomrule
    \end{tabular}
    \caption{Our main results.}
    \label{tab: results}
\end{table}


\subsection{Related works}
Local certification schemes for different graph classes have been intensively studied. In~\cite{GS16}, they introduce common complexity classes in local certification and prove tight bounds for several graph properties. For example, $s$--$t$ reachability can be certified in $O(1)$ bits, and to certify that $s$--$t$ connectivity equal to $k$, it suffices to use $O(\log k)$ bits; a crossing technique is developed to prove $\Omega(\log n)$ lower bound for many properties such as parity of the graph size and spanning trees, together with the existing upper bound, the complexity of these problems are $\Theta(\log n)$. There are also graph properties with certification complexity $\poly(n)$, such as symmetricity and non-$3$-colorability, where the lower bounds are reduced from communication complexity. 

%\yijun{Is it possible to add back the logarithmic lower bound for VC for any $k \geq 3$ in the table?}



%In~\cite{BFP21}, they make use of the constructive characterizations for $2$-vertex-connected graphs to certify $2$-vertex-connectivity, and certify minor-freeness for small forbidden minors by decomposing graphs into $2$-vertex-connected components. 


There is a long line of work that studies the connectivity problem in the \textsf{CONGEST} model. Computing the min-cut in a network requires $\Tilde{\Omega}(\sqrt{n}+\diam)$ rounds~\cite{SHK+11, GK13}, where the lower bound also holds for any constant-approximation. In~\cite{GK13}, they proposed a $(2+\epsilon)$-approximation algorithm that almost matches the lower bound; the approximation ratio was later improved to $(1+\epsilon)$ by~\cite{NS14}. For exact min-cut,~\cite{GNT20} improved the complexity of~\cite{DHNS19} and provided the first sublinear algorithm; the worst-case optimal round complexity $\Tilde{O}(\sqrt{n}+\diam)$ was achieved in~\cite{DEM+21}, matching the lower bound. Later on, a universal optimal algorithm for exact min-cut was proposed by~\cite{GZ22}. The min-cut problem is also studied in other related models, such as congested clique~\cite{GN18} and massively parallel computation~\cite{GN20}.



It was known that the treedepth decomposition over a bounded treedepth graph \cite{feuilloley2022can} can be certified with $O(\log n)$ bits, and moreover this leads to $O(\log n)$-bit certification of any monadic second order graph property on bounded treedepth graphs. This result was later extended to $O(1)$-round algorithms in the $\CONGEST$ model~\cite{fomin2026distributed}. Low-treedepth coloring has also been applied to show compact local certification and efficient distributed algorithms for deciding first-order properties in graphs of bounded expansion~\cite{fomin2025brief,nevsetvril2016distributed}.
 




==> intro-backup.tex <==
\section{Introduction}

Local certification is a mechanism that allows a network to verify certain global properties $\Pcal$ using only local information. Informally, a local certification scheme can be described as a prover that assigns labels to the vertices, and a distributed verification algorithm that takes as input the local view of a vertex and decides whether to accept or reject. Whenever a network configuration satisfies $\Pcal$, there should be a labeling such that the verification passes on every vertex in the network, whereas if the network configuration does not satisfy $\mathcal{P}$, then no matter how the prover labels the vertices, the verification will fail on some vertices. The goal is to design a compact local certification for some given property with a small label size.
%\mtt{How about replacing ``is correct'' with ``satisfies $\mathcal{P}$''} 

Local certification provides us with a framework to achieve error detection. It was first proposed as a building block of a self-stabilizing algorithm to certify the solution under transient faults~\cite{KKP05}. In particular, space complexity is an important measurement of a self-stabilizing algorithm, and there has been work that makes black-box use of compact local certification schemes to design compact self-stabilizing algorithms~\cite{BFP14}. However, certifying the structure of a network itself is also important, as running distributed algorithms and certifying their solutions may be simpler in certain graph classes.

One important open problem in this field is whether every minor-closed graph property admits an $O(\log n)$ local certification scheme~\cite{Feu21}. Minor-closed properties capture several natural graph classes, including planar graphs, bounded genus graphs, and bounded tree-width graphs, and many problems admit more efficient distributed algorithms and certification schemes in certain minor-closed graph classes~\cite{HLZ22, cha23, CKM25}. Working towards this goal, it has been shown that planar graphs and bounded genus graphs can be certified in $O(\log n)$ bits~\cite{FFM+23, FFM+20}. Minor-free graphs with some small-sized minors are also proven to have $O(\log n)$-bit certification schemes~\cite{BFP21}. 

It was left as an open question in~\cite{BFP21} to understand the complexity of certifying $k$-vertex-connectivity. As stated in~\cite{BFP21}, the importance of certifying $k$-vertex-connectivity is twofold. First, they show that certifying both $2$-edge-connectivity and $2$-vertex-connectivity can be done in $O(\log n)$ bits, and certifying $3$-vertex-connectivity can be done in $O(\log n)$ bits on vertices and $O(1)$ bits on edges. Certifying $2$-vertex-connected components and $3$-vertex-connected components are then used as building blocks to certify minor-free graph classes; therefore, certifying $k$-vertex-connected components may be a useful tool to certify other, more complicated graph classes. Second, since robustness is a nice property of a network and can be captured by connectivity, certifying $k$-vertex-connectivity is of independent interest as well. In particular, we establish some tools and results toward the following questions:\yijun{say that \cite{BFP21} did for connectivity certification: 2-vc/ec with $O(\log n)$ bits, and 3-vc with $O(\log n)$ bits but labels are put on edges only (which suffice for their purpose, as they deal with bounded degeneracy graphs), so that the following questions become natural to ask.}
\begin{problem}[{\cite[Question 57]{BFP21}}]\label{ques1}
    Does the certification for $k$-vertex-connectivity require $\Omega(\log n)$ bits for any $k\geq 2$?
\end{problem}
\begin{problem}[{\cite[Question 58]{BFP21}}]\label{ques2}
    Can $k$-vertex-connectivity be certified with $O(\log n)$ bits for any $k\geq 4$?
\end{problem}


\subsection{Our results}
In this paper, we work towards the goal of certifying $k$-edge/vertex-connectivity for any value of $k$. A summary of our results can be found in~\Cref{tab: results}.

Using the crossing technique introduced in~\cite{GS16}, we answer \Cref{ques1} affirmatively:\yijun{todo: add brief technical overview surrounding the theorems to highlight all the innovative/interesting proof ideas -- the reviewer is only obligated to read the first 10 pages} 
%\yijun{todo: add a table summarizing new and old results.}\yijun{do theorem-restate consistently for all theorems}
\begin{restatable}{theorem}{thmKConnLower}\label{thm: k-conn-lower}
    For any integer $k\geq 3$, certifying $k$-edge-connectivity and $k$-vertex-connectivity both require $\Omega(\frac{\log n}{k})$ bits.
\end{restatable}
The intuition is that if a $k$-edge/vertex-connected graph has an edge with a bounded neighborhood, then we consider $\Theta(n)$ such instances. If the proof size is $o(\log n)$, then there must exist a constant number of instances receiving identical labels in the neighborhood of that edge, and we can pick two of them, cut the edges, and glue them together, which results in a graph with connectivity $2$\mtt{vertex and edge? needs to come back to fix} but all vertices still accept due to identical labels in their neighborhoods.

The lower bound works for planar graphs as well.
\begin{restatable}{theorem}{thmKConnPlanarLower}\label{thm: k-conn-lower-planar}
    For any integer $3\leq k\leq 5$, certifying $k$-edge-connectivity and $k$-vertex-connectivity for planar graphs both require $\Omega(\log n)$ bits.
\end{restatable}

To answer \Cref{ques2}, we first construct a local certification scheme for a sparse subgraph that preserves $k$-vertex-connectivity (called a \emph{sparse certificate}). It has been shown that iteratively finding $k$ BFS forest results in a sparse certificate for both $k$-edge- and $k$-vertex-connectivity~\Cref{lem: sparse-cert-iff}. Therefore, the local certification can be done by iteratively certifying BFS spanning forests.
\begin{restatable}{lemma}{lemSparseCert}\label{lem: cert-sparse-cert}
    There exists an $O(k\log n)$-bit local certification scheme for a sparse certificate of both $k$-edge-connectivity and $k$-vertex-connectivity.
\end{restatable}
Given the sparse certificate, any edge-certification scheme can be transformed into a vertex-certification scheme efficiently~\cref{lem:EdgeCert-degeneracy}.

In~\cite{BFP21}, they give a local certification scheme for $3$-vertex-connectivity using $O(\log n)$ bits on vertices and $O(1)$ bits on edges. As a corollary of \Cref{lem: cert-sparse-cert}, we can restrict ourselves to bounded arboricity graphs, and thus improve the complexity to $O(\log n)$ bits on vertices only.
\begin{restatable}{corollary}{corThreeVC}\label{cor: 3-vc}
    The complexity of certifying $3$-vertex-connectivity is $\Theta(\log n)$.
\end{restatable}

In~\cite{BFP21}, they certify $2$-edge-connectivity using a constructive characterization called \emph{ear-decomposition}. We use a different approach to certify $k$-edge-connectivity for any $k\geq 2$. For $k\equiv 0\mod 2$, we use the known equivalence between $k$-edge-connectivity in undirected graphs and $\frac{k}{2}$-arc-connectivity orientation in directed graphs~\cite{Robbins39,NashWilliams60}, then applying Edmonds' branching theorem~\cite{Edmonds73} to reduce the problem to certifying $k$ arc-disjoint out-branchings, which can be done in $O(k\log n)$ bits. For $k\equiv 1\mod 2$, certifying $k$-edge-connectivity can be reduced to certifying $(k-1)$-edge-connectivity via an edge-covering.
%\mtt{The case of $k=1$ may look strange.}

{\color{red}(To be aligned with corresponding sections)}
\begin{restatable}{theorem}{thmkEC}\label{thm: k-ec}
    For any integer $k \ge 3$, there exists an $O(k \log n)$-bit local certification scheme for $k$-edge-connectivity when $k$ is even, and an $O(81^{k^2}k\log n)$-bit local certification scheme when $k$ is odd.
\end{restatable}

%\mtt{The dependence on $k$ may be as large as $81^{k^2}$. Did we remove this dependence?}\yijun{I suggest that we keep the dependence on $k$ (and also max deg $\Delta$) whenever possible.}

For $k$-vertex-connectivity, we use the idea of certifying $k$ independent spanning trees for $k$ different vertices. For $k=4$, it is known that $k$-vertex-connectivity is equivalent to having $4$ independent spanning trees for $4$ different vertices. Zehavi--Itai conjectured that this holds for any larger $k$. Assuming the conjecture, the task can be reduced to certifying that two trees rooted at the same vertex are independent. 
%We use a heavy-light decomposition to further reduce the size of certificates to $\Tilde{O}_k(\sqrt{n})$.

{\color{red}think i didn't write this part well}
The naive approach is that for each vertex $u$, we send the information of $u$ to all its descendants in both trees, that is, we record all the information along the root-to-$v$ path. By doing so, the vertex can tell if there are any other vertices in the intersection of the two root-to-$v$ paths. It is only efficient when the tree has low depth. We apply heavy-light decomposition to compress the tree into $O(\log n)$ layers and encode each path by a set of at most $O(\log n)$ segments, and we can store the root-to-$v$ path-encoding for each tree compactly. For each segment $S$ in the root-to-$v$ path, we want to bound the amount of information that $S$ should send to $v$.

A key observation is that for each vertex $u$ that belongs to segment $S_1$ in $T_1$ and segment $S_2$ in $T_2$, it suffices that one of the segments $S_i$ takes the responsibility to send the information of $u$ to all its descendants in $T_i$. If a segment is short, then we can afford to let it take the responsibility, as the number of ancestors in a short segment is small. On the other hand, if a long segment takes the responsibility, then it must send the information of $u$ that also belongs to a long segment in the other tree. Intuitively, the amount of such information can be bounded, as we cannot have many long segments in each tree. Finally, we trade off the length of short segments and the number of long segments to obtain the desired bound.

\begin{restatable}{theorem}{thmKVC}\label{thm: k-vc-cert}
    There exists an $O(k^3\sqrt{n}\log^{1.5}n)$-bit local certification scheme for $4$-vertex-connectivity. 
    Moreover, assuming the Itai--Zehavi conjecture (\Cref{conj: Itai--Zehavi}), the same bound holds for every $k \ge 5$.
    %This holds also for any $k\geq 5$ assuming the Itai--Zehavi conjecture (\Cref{conj: Itai--Zehavi}).
\end{restatable}

Since the upper bound for $k$-vertex-connectivity is $\Tilde{O}_k(\sqrt{n})$, while the lower bound we get is $\Omega_k(\log n)$, a natural question to ask is whether we can do better using the independent tree approach. We prove that given a labeled graph where each vertex receives two IDs that point to its parents in $T_1$ and $T_2$, certifying that $T_1$ and $T_2$ are independent spanning trees rooted at the same vertex in $G$ requires $\Omega(\sqrt{n})$ bits.

\begin{restatable}{theorem}{thmIndepST}\label{thm: indep-st-lower}
    Given a graph $G$ and two spanning trees $T_1$ and $T_2$ rooted at the same vertex $r$, certifying $T_1$ and $T_2$ are independent requires $\Omega(\sqrt{n})$ bits.
\end{restatable}



For $2$-edge-connectivity, it is known that any bridgeless graph can be covered by a constant number of Eulerian subgraphs~\Cref{lem: Eulerian-cover}, which leads to a constant-bit local certification scheme on edges. On bounded degree graphs, the edge certification scheme can be transformed into a vertex certification scheme with an $O(\Delta^2)$ overhead.
\begin{restatable}{theorem}{thmTwoEC}\label{thm: 2-edge-conn}
    There exists an $O(\Delta^2)$-bit local certification scheme for $2$-edge-connectivity on bounded-degree graphs.
\end{restatable}

For $2$-vertex-connectivity, we also obtain a constant-bit local certification scheme for bounded degree graphs by a reduction to $2$-edge-connectivity. Intuitively, we consider a vertex cut in the graph. If we can correctly guess how the neighbors are separated into two parts, then making those vertices into edges that connect the two parts will result in a graph that transforms vertex-connectivity to edge-connectivity. The problem is how we can simultaneously guess the neighborhood partition for all potential vertex cuts, and it can be done when we only need to tell whether the graph admits a cut vertex or not.
\begin{restatable}{theorem}{thmTwoVC}\label{thm: 2-vertex-conn}
    There exists an $O(\Delta^2\cdot 2^{\Delta})$-bit local certification scheme for $2$-vertex-connectivity on bounded-degree graphs.
\end{restatable}

We show that the upper bound in \Cref{thm: k-vc-cert} can be improved to $O(\log n)$ for planar graphs.
Since our $\Omega(\log n)$ lower bound also applies to planar graphs for all $k \geq 3$, and the vertex connectivity of any planar graph is at most $5$, it follows that $\Theta(\log n)$ is the tight bound for $k$-vertex connectivity on planar graphs for all $k \geq 3$.


\begin{restatable}{theorem}{thmPlanarVC}\label{thm:planar-vc}
 For any $k$, there exists an $O(\log n)$-bit local certification scheme for $k$-vertex-connectivity on planar graphs.
\end{restatable}

The proof of \Cref{thm:planar-vc} starts from an elegant observation~\cite{Eppstein1999SubgraphJGAA}: in a planar graph, vertex connectivity equals half the length of the shortest separating cycle in its radialization. The radialization transforms the graph by introducing a vertex for each face, connecting it to all vertices on the boundary of the face, and all deleting the original edges. This viewpoint is promising, as detecting cycles of constant length in planar graphs can be done with $O(\log n)$-bit labels using a known approach~\cite{fomin2025brief,nevsetvril2016distributed}: first reduce the graph to bounded treedepth via a low-treedepth coloring, and then perform dynamic programming over the  treedepth decomposition.

The central difficulty is that this machinery does not directly capture the topological requirement that the cycle must be separating. Our key insight is that, in 3-vertex-connected planar graphs, the separating condition admits a purely combinatorial reformulation: we show that it suffices to look for cycles that are both non-facial and chordless.

We then demonstrate that both conditions can be handled within dynamic programming over a treedepth decomposition. At each vertex $v$, the table stores collections of paths that may form parts of the target shortest cycle $C$. When merging solutions from distinct child subtrees of $v$, no new chords can arise, since treedepth decompositions forbid edges between internal vertices of different child subtrees. This naturally enforces the chordless property.

The non-facial condition is more challenging. Determining whether a cycle is $G$-facial may, in general, require global knowledge of the entire cycle, making it unclear what information must be stored when working with partial path solutions. To resolve this, we establish a structural lemma showing that for any fixed path $P$, avoiding extensions that yield a facial cycle requires excluding only a bounded number of specific continuations. Consequently, it suffices to store a bounded number of partial solutions for each subproblem.

\begin{table}
    \centering
    \begin{tabular}{m{16em}m{12em}m{10em}}

        Task & Complexity & Reference\\ 
        \midrule
        \midrule
        
        \multirow{2}{16em}{$2$-edge-connectivity}
         & $O(\log n)$ & \cite{BFP21} \\ 
         & $O(\Delta^2)$ & \Cref{thm: 2-edge-conn} \\ 
        \addlinespace[8pt]
        \multirow{2}{16em}{$2$-vertex-connectivity}
         & $O(\log n)$ & \cite{BFP21} \\
         & $O(\Delta^2\cdot 2^\Delta)$ & \Cref{thm: 2-vertex-conn} \\
        \addlinespace[8pt]
        \multirow{3}{16em}{$k$-edge-connectivity, $k\geq 3$}
         & $\Omega(\frac{\log n}{k})$ & \Cref{thm: k-conn-lower,thm: k-conn-lower-planar}\\
         & $O(k\log n)$, $k$ even & \Cref{thm: k-ec}  \\
         & $O(81^{k^2}\log n)$, $k$ odd & \Cref{thm: k-vc-cert} \\
        \addlinespace[8pt]
        $3$-vertex-connectivity & $O(\log n)$ on vertices and $O(1)$ on edges & \cite{BFP21} \\
         & $O(\log n)$ & \Cref{cor: 3-vc}\\
        \addlinespace[8pt]
        $4$-vertex-connectivity & $O(k^3\sqrt{n}\log^{1.5}n)$ & \Cref{thm: k-vc-cert} \\
        \addlinespace[8pt]
        $k$-vertex-connectivity, $k\geq 5$ & $O(k^3\sqrt{n}\log^{1.5}n)$ assuming Itai--Zehavi conjecture & \Cref{thm: k-vc-cert} \\
        \addlinespace[8pt]
        two independent spanning trees & $\Omega(\sqrt{n})$ & \Cref{thm: indep-st-lower}\\
        \addlinespace[8pt]
        $k$-vertex-connectivity, planar graphs & $O(\log n)$ & \Cref{thm:planar-vc} \\
        \bottomrule
    \end{tabular}
    \caption{Our main results.}
    \label{tab: results}
\end{table}


\subsection{Related works}
Local certification schemes for different graph classes have been intensively studied. In~\cite{GS16}, they introduce common complexity classes in local certification and prove tight bounds for several graph properties. For example, $s$--$t$ reachability can be certified in $O(1)$ bits, and to certify that $s$--$t$ connectivity equal to $k$, it suffices to use $O(\log k)$ bits; A crossing technique is developed to prove $\Omega(\log n)$ lower bound for many properties such as parity of the graph size and spanning trees, together with the existing upper bound, the complexity of these problems are $\Theta(\log n)$; There are also graph properties with certification complexity $\poly(n)$, such as symmetricity and non-$3$-colorability, where the lower bounds are reduced from communication complexity. 

As stated in the introduction, some minor-closed graph classes, such as bounded genus graphs and planar graphs, can be certified using $O(\log n)$ bits. It was first solved in the model of interactive distributed proof~\cite{NPY20} that verifies a graph is planar using three rounds of communication with $O(\log n)$-bit proof size. In~\cite{FFM+20}, they construct a local certification scheme (which can be viewed as one round of communication from prover to the verifier) for planarity in $O(\log n)$ bits, which is extended by~\cite{FFM+23} to bounded genus graphs. In~\cite{BFP21}, they make use of the constructive characterizations for $2$-vertex-connected graphs to certify $2$-vertex-connectivity, and certify minor-freeness for small forbidden minors by decomposing graphs into $2$-vertex-connected components. 


There is a long line of work that studies the connectivity problem in the \textsf{CONGEST} model. Computing the min-cut in a network requires $\Tilde{\Omega}(\sqrt{n}+\diam)$ rounds~\cite{SHK+11, GK13}, where the lower bound also holds for any constant-approximation. In~\cite{GK13}, they proposed a $(2+\epsilon)$-approximation algorithm that almost matches the lower bound; the approximation ratio was later improved to $(1+\epsilon)$ by~\cite{NS14}. For exact min-cut,~\cite{GNT20} improved the complexity of~\cite{DHNS19} and provided the first sublinear algorithm; the worst-case optimal round complexity $\Tilde{O}(\sqrt{n}+\diam)$ was achieved in~\cite{DEM+21}, matching the lower bound. Later on, a universal optimal algorithm for exact min-cut was proposed by~\cite{GZ22}. The min-cut problem is also studied in other related models, such as congested clique~\cite{GN18} and massively parallel computation~\cite{GN20}.



It was known that the treedepth decomposition over a bounded treedepth graph \cite{feuilloley2022can} can be certified with $O(\log n)$ bits, and moreover this leads to $O(\log n)$-bit certification of any monadic second order graph property on bounded treedepth graphs. This result was later extended to $O(1)$-round algorithms in the $\CONGEST$ model~\cite{fomin2026distributed}. Low-treedepth coloring has also been applied to show compact local certification and efficient distributed algorithms for deciding first-order properties in graphs of bounded expansion~\cite{fomin2025brief,nevsetvril2016distributed}.
\yijun{can discuss: the study of planar graphs in local certification and/or distributed proofs}




==> intro_backup_v2.tex <==
\subsection{Models of local certification}\label{sec: model-def}
%We mainly follow the definitions of the local certification scheme in \cite{BFZ25, Feu21}.

{\color{blue}
Consider a family $\Fcal$ of (possibly labeled) input graphs. A local certification scheme allows vertices to verify some property $\Pcal$ for the graphs in $\Fcal$ using only their local views. In this paper, we consider $\Fcal$ to be a subset of all connected graphs. Local certification schemes can be described as an external \emph{prover} and a \emph{verifier}. Given a graph $G$ from $\Fcal$, the prover assigns some certificates to each vertex, and the verifier, which is a distributed algorithm, decides whether to accept based on the local view of a vertex.

More formally, a \emph{certificate assignment} of $G$ of length $s$ is a mapping from $V(G)$ to the set of $s$-bit strings. The \emph{view} of a vertex consists of some information in its neighborhood that is accessible to the verifier. Different models of local certification schemes have been proposed based on different levels of information contained in the view of a vertex. In the following, we define three extensively studied models. For readers who are familiar with the notion of local certification schemes, they correspond to the \emph{anonymous model}~\cite{KKP05, BFZ25}, the \emph{id-based proof-labeling schemes}~\cite{KKP05, Feu21}, and the \emph{locally checkable proofs} with local horizon $1$~\cite{GS16, Feu21}. To avoid confusion, in this paper we refer to them as the \emph{anonymous model}, the \emph{$KT_0$ model}, and the \emph{$KT_1$ model}, inspired by standard notions in distributed algorithms.\yx{cite papers.}

\begin{description}
    \item[The anonymous model] The vertices are not equipped with identifiers. The verifier has access only to the certificate assignments in its neighborhood.
    \item[The $KT_0$ model] The vertices are equipped with unique $O(\log n)$-bit identifiers. The verifier has access to its own ID and input, and the certificate assigned to all its neighbors, but not their identifiers.
    \item[The $KT_1$ model] The vertices are equipped with unique $O(\log n)$-bit identifiers. The verifier has access to the certificate assignments, IDs, and inputs of all its neighbors and itself.
\end{description}

%The \emph{view} of a vertex consists of all information accessible to the verifier in its neighborhood. The verifier takes as input the view of a vertex and outputs accept or reject.


%Consider a family $\Fcal$ of (possibly labeled) graphs. In this paper, we consider $\Fcal$ to be a subset of all connected graphs. A local certification scheme allows vertices to verify some property $\Pcal$ using only their local views. It can be described as an external prover and a verifier. The prover puts some certificates on each vertex, and the verifier, which is a distributed algorithm, decides whether to accept locally.
%There are several models of local certification. In this paper, we consider the \emph{proof labeling scheme}. Each vertex in the graph is associated with a unique identifier (ID) of length $O(\log n)$. A \emph{certificate assignment} of $G$ of length $s$ is a mapping from $V(G)$ to the set of $s$-bit strings. The \emph{view} of a vertex consists of all information in its neighborhood (including itself), including the induced graph topology and certificate assignments of these vertices, as well as the inputs and ID of itself. The \emph{verifier} takes as input the view of a vertex and outputs accept or reject.


%There are several models of local certification. In this paper, we consider the \emph{locally checkable proofs}. Each node in the graph is associated with a unique identifier (ID) of length $O(\log n)$. A \emph{certificate assignment} of $G$ of length $s$ is a mapping from $V(G)$ to the set of $s$-bit strings. The \emph{view} of a vertex at distance $r$ consists of all information about its $r$-hop neighborhood (including itself), including the induced graph topology, certificate assignments, and the inputs and IDs of these vertices. The \emph{verifier} takes as input the view at distance $r$ of a vertex and outputs accept or reject. Here $r$ is said to be the \emph{local horizon} of the verifier. In this paper, we only consider verifiers of local horizon $1$.


The property $\Pcal$ that we want to certify should be independent of IDs. We say that $\Pcal$ admits a \emph{certification scheme} of size $s$ if there exists a verifier that satisfies \emph{completeness} and \emph{soundness}:

\begin{itemize}
    \item Completeness: For any $n$-vertex graph $G\in\Pcal$, and any ID assignment of $G$, there exists a certificate assignment of size $s(n)$ such that all vertices output accept.
    \item Soundness: For every $G\not\in\Pcal$, for every ID assignment of $G$, for any certificate assignment of any size, there exists at least one vertex that outputs reject.
\end{itemize}

There is another notion called \emph{edge certification scheme}~\cite{BFP21, FFM+23}. The setting is the same as in the standard local certification scheme, except that a certificate assignment of length $s$ for a graph $G$ is a mapping from $V(G) \cup E(G)$, rather than only $V(G)$, to the set of $s$-bit strings. Accordingly, the view of each vertex is enlarged to include the certificates assigned to its incident edges in each variation of the model. To distinguish edge-certification schemes from the standard local certification schemes, where we only assign certificates on vertices, we sometimes call the standard local certification schemes the \emph{vertex-certification schemes}. We will adapt some results from the edge certification scheme to the vertex-certification schemes and use them as building blocks for our main algorithms.

%In the \emph{edge certification scheme}~\cite{BFP21, FFM+23}, the setting is the same as in the standard local certification scheme, except that a certificate assignment of length $s$ for a graph $G$ is a mapping from $V(G) \cup E(G)$, rather than only $V(G)$, to the set of $s$-bit strings. Accordingly, the view of each vertex is enlarged to include the certificates assigned to its incident edges in each variation of the model. We will adapt some results from the edge certification scheme to the proof-labeling scheme and use them as building blocks for our main algorithms.
}

{\color{red}Notice that every local certification scheme that works in the anonymous model also works in the $KT_0$ model; and every local certification scheme that works in the $KT_0$ model also works in the $KT_1$ model. Therefore, proving an upper bound in the anonymous model is stronger than proving the same bound in the $KT_0$ model, which in turn is stronger than in the $KT_1$ model. From the perspective of lower bounds, the implications are reversed. In the region where the certificate assignment is of size $\Omega(\log n)$, the $KT_0$ model and the $KT_1$ model are asymptotically equivalent, as in the $KT_0$ model, the prover can always write the ID of a vertex in its own certificate and let the vertex verify the consistency. In contrast, there is a sharp separation between the anonymous model and the $KT_0$ model, as several tasks, including certifying leader election and spanning tree, are impossible in the anonymous model, while every computable function admits a certification scheme in the $KT_0$ model by assigning the description of the whole network to every vertex. See~\cite{KKP05} for more details.
%when we talk about a local certification scheme of size $\Omega(\log n)$ in the $KT_0$ model, we can assume for simplicity that the view of each vertex contains the IDs of its neighbors, as otherwise the prover can always write the ID of a vertex in its own certificate and let the vertex verify the consistency.

In this paper, we will take $KT_0$ as our main focus. All our results at least hold for the $KT_0$ model except for the $2$-vertex-connectivity lower bound, which only works in the anonymous model.
%unless stated otherwise.
}
%\yx{explain the relation between different models}
%\yx{in the theorems, result, and technical overview, specify which model we are referring to}
\yx{maybe can consider shortening this section here and moving the complete definition back to the prelim?}
\fi

%In the literature, there is another form of local certification called \emph{locally checkable proofs}. Locally checkable proof is similar to the proof-labeling scheme described above, except that the view of a vertex may consist of all information about its $r$-hop neighborhood (including itself), including the induced graph topology, certificate assignments, and the inputs and IDs of these vertices. The verifier takes as input the view at distance $r$ of a vertex and outputs accept or reject. Here $r$ is said to be the \emph{local horizon} of the verifier.

%Although we focus on proof labeling schemes in this paper, our lower bounds also work in the locally checkable proofs with local horizon $r=1$. \mtt{Is the proof labeling scheme exactly locally checkable proofs with $r=1$? I am not sure why we need this paragraph.}\yx{also in the locally checkable proof, each vertex sees the id of its neighbors (in the proof-labeling scheme only labels)}
%Also, when we talk about a proof labeling scheme of size $\Omega(\log n)$, we can assume for simplicity that the view of each vertex contains the IDs of its neighbors, as otherwise the prover can always write the ID of a vertex in its own certificate and let the vertex verify the consistency.



%{\color{orange} There are other related models of local certification, such as non-deterministic local decision, where the certificates should not depend on the identifier assignments, and the anonymous model, where the vertices are not equipped with identifiers. See~\cite{Feu21, BFZ25} and the references therein for more discussion on these models.} \mtt{This paragraph looks redudant to me.}\yx{now we have lower bound for 1-vc in the anonymous model, so need to think hos to give the background here.}


\subsection{Results and technical overview}\label{sec: resuls}

\subsubsection{A lower bound for $k$-edge-connectivity and $k$-vertex-connectivity for $k\ge 3$.}

We answer \Cref{ques1} affirmatively by proving \cref{thm: k-conn-lower} using the so-called cut-and-plug technique introduced in~\cite{GS16}. The intuition is that we consider a $k$-edge/vertex-connected graph that has a special edge, {\color{red}where both endpoints have a bounded number of neighbors, and consider $\Theta(n)$ copies of such a graph} on different identifier sets. If the proof size is $o(\log n)$, then there must exist a constant number of copies receiving identical label assignments in the neighborhood of the special edges. We pick two such copies and glue them together to create a new accepting graph with low connectivity by removing the special edges and reconnecting each endpoint to the copy of its neighbor (originally incident to the special edge) in the other copy of the graph. This results in a graph with connectivity $2$ (both edge and vertex), but all vertices still accept due to identical labels in their neighborhoods.
%We answer \Cref{ques1} affirmatively by proving \cref{thm: k-conn-lower} using the crossing technique introduced in~\cite{GS16}. The intuition is that if a $k$-edge/vertex-connected graph has an edge with a bounded neighborhood, then we consider $\Theta(n)$ such instances. If the proof size is $o(\log n)$, then there must exist a constant number of instances receiving identical labels in the neighborhood of that edge, and we can pick two of them, cut the edges, and glue them together, which results in a graph with connectivity $2$ (both edge and vertex) but all vertices still accept due to identical labels in their neighborhoods.




We then devise an optimal local certification scheme for $k$-edge-connectivity for any constant $k \ge 3$ in \cref{sec:optimal}. Next, in \cref{sec:bottlenecktight}, we devise a bottleneck-tight local certification scheme for $k$-vertex-connectivity for $k=4$ (and, more generally, for any constant $k \ge 5$ assuming the Zehavi--Itai conjecture), thereby partially answering \Cref{ques2}.

%, we first construct a local certification scheme for a sparse subgraph that preserves $k$-vertex-connectivity (called a \emph{sparse certificate}). %It has been shown that iteratively finding $k$ BFS forest results in a sparse certificate for both $k$-edge- and $k$-vertex-connectivity~\Cref{lem: sparse-cert-iff}. Therefore, the local certification can be done by iteratively certifying BFS spanning forests.
%\begin{restatable}{lemma}{lemSparseCert}\label{lem: cert-sparse-cert}
%    There exists an $O(k\log n)$-bit local certification scheme for a sparse certificate of both $k$-edge-connectivity and $k$-vertex-connectivity.
%\end{restatable}
%Given the sparse certificate, any edge-certification scheme can be transformed into a vertex-certification scheme efficiently~\cref{lem:EdgeCert-degeneracy}. 

%In~\cite{BFP21}, they give a local certification scheme for $3$-vertex-connectivity using $O(\log n)$ bits on vertices and $O(1)$ bits on edges. As a corollary of \Cref{lem: cert-sparse-cert}, we can restrict ourselves to bounded arboricity graphs, and thus improve the complexity to $O(\log n)$ bits on vertices only.
%\begin{restatable}{corollary}{corThreeVC}\label{cor: 3-vc}
%    The complexity of certifying $3$-vertex-connectivity is $\Theta(\log n)$.
%\end{restatable}


\subsubsection{An optimal local certification scheme for $k$-edge-connectivity}\label{sec:optimal}

In~\cite{BFP21}, the authors certify $2$-edge-connectivity via a constructive characterization known as an \emph{ear decomposition}. We take a different route to certify $k$-edge-connectivity for all $k \ge 2$.

For even $k \ge 2$, we use the classical equivalence: an undirected simple graph $G$ is $k$-edge-connected if and only if $G$ admits an orientation $\vec{G}$ that is $(k/2)$-arc-strongly connected~\cite{Robbins39,NashWilliams60}. We then apply Edmonds' branching theorem~\cite{Edmonds73} to reduce the task to certifying $k/2$ pairwise arc-disjoint out-branchings and $k/2$ pairwise arc-disjoint in-branchings rooted at a common vertex, which can be done using $O(k\log n)$ bits.

For odd $k \ge 3$, we use another equivalence: $G$ is $k$-edge-connected if and only if there exists a partition of $E(G)$ into sets $E_1,E_2,\ldots,E_{\ell_k}$ such that $G\setminus E_i$ is $(k-1)$-edge-connected for every $i \in [\ell_k]$. In~\cite{DeVosJS03}, DeVos, Johnson, and Seymour showed that one may take $\ell_k \le 81^{k^2}$, and they further claimed (without proof) that this bound can be reduced to $\ell_k = 2^{O(k)}$. For small values of $k$, it is known that $\ell_3 \le 9$ and $\ell_5 \le 30$.

%Goedgebeur, M{\'{a}}cajov{\'{a}}, and Renders show that $\ell_3 \le 4$


%{\color{red}(To be aligned with corresponding sections)}



Given \cref{thm: k-conn-lower}, we know that \cref{thm: k-ec} is optimal for every constant $k \ge 3$.

%\mtt{The dependence on $k$ may be as large as $81^{k^2}$. Did we remove this dependence?}\yijun{I suggest that we keep the dependence on $k$ (and also max deg $\Delta$) whenever possible.}

\subsubsection{A bottleneck-tight local certification scheme for $k$-vertex-connectivity}\label{sec:bottlenecktight}
{\color{blue}
In~\cite{BFP21}, the authors certify $k$-vertex-connectivity for $k \in \{2,3\}$ using constructive characterizations based on \emph{open ear decompositions} and \emph{Mondshein sequences}. We again take a different route to certify $k$-vertex-connectivity for all $k \ge 2$. Our certification scheme relies on a conjecture by Zehavi and Itai~\cite{ZI89} on the equivalence between vertex-connectivity and independent spanning trees, which we now explain.

Given a graph $G$, two spanning trees $T$ and $T'$ rooted at the same vertex $r$ are said to be \emph{independent} if for any vertex $v$, the $v$--$r$ path in $T$ and the $v$--$r$ path in $T'$ are internally vertex-disjoint. We say that $G$ admits $k$ independent spanning trees rooted at $r$ if there exist $k$ spanning trees of $G$ rooted at $r$ that are pairwise independent. Zehavi and Itai conjectured that for every fixed integer $k \ge 1$, an undirected simple graph $G$ is $k$-vertex-connected if and only if, for every vertex $r \in V(G)$, $G$ contains $k$ \emph{independent spanning trees} rooted at $r$.


Zehavi--Itai conjecture had been known to hold for every $k \in \{1, 2, 3\}$~\cite{ItaiR88,CheriyanM88,ZI89}, and was later proven to hold also for $k=4$~\cite{CLY06}.
%\begin{lemma}[\cite{CLY06}]
    %Let $G$ be a $4$-vertex-connected graph, and let $r\in V(G)$. Then there exist four independent spanning trees of $G$ rooted at $r$.
%\end{lemma}

We note that, by a simple observation, the Itai--Zehavi conjecture implies that a graph $G$ is $k$-vertex-connected if and only if there exist $k$ distinct vertices $r_1,\ldots,r_k \in V(G)$ (rather than all vertices) such that, for each $i \in [k]$, $G$ contains $k$ independent spanning trees rooted at $r_i$. Suppose that $G$ contains such roots but is not $k$-vertex-connected, then there exists a vertex cut $C$ with $|C|<k$ such that $G-C$ is disconnected. Since $C$ has size less than $k$, it cannot contain all of $r_1,\ldots,r_k$, so some root $r^*$ remains in $G-C$. Since $G-C$ is disconnected, there exists a vertex $x$ that belongs to a component of $G-C$ different from the one containing $r^*$. 
%Let $x$ be a vertex in a component of $G-C$ different from the one containing $r^*$. 
This contradicts the existence of $k$ independent spanning trees in $G$ rooted at $r^*$, which implies that there are $k$ internally vertex-disjoint paths between $r^*$ and $x$, and hence no vertex cut of size less than $k$ can separate them.


%In~\cite{BFP21}, the authors certify $k$-vertex-connectivity for $k \in \{2,3\}$ using constructive characterizations based on \emph{open ear decompositions} and \emph{Mondshein sequences}. We again take a different route to certify $k$-vertex-connectivity for all $k \ge 2$.

%For $k$-vertex-connectivity, we rely on the equivalence conjectured by Zehavi and Itai~\cite{ZI89}: for every fixed integer $k \ge 1$, an undirected simple graph $G$ is $k$-vertex-connected if and only if, for every vertex $r \in V(G)$, $G$ contains $k$ \emph{independent spanning trees} rooted at $r$, meaning that for each vertex $s \in V(G)\setminus\{r\}$, the $k$ paths from $s$ to $r$ (one in each tree) are pairwise internally vertex-disjoint.

%Zehavi--Itai conjecture is known to hold for every $k \in \{1, 2, 3, 4\}$~\cite{ItaiR88,CheriyanM88,ZI89,CLY06}.
%We note that, to certify that $G$ is $k$-vertex-connected, it suffices to choose $k$ distinct roots $r_1,\ldots,r_k \in V(G)$ (rather than all vertices) such that, for each $i \in [k]$, the graph contains $k$ independent spanning trees rooted at $r_i$.
Given the above equivalence, certifying $4$-vertex-connectivity reduces to certifying that $24$ pairs of spanning trees rooted at a common vertex are independent. More generally, assuming~\Cref{conj: Itai--Zehavi}, the same reduction applies to certifying $k$-vertex-connectivity for every $k \ge 5$. In~\Cref{sec:kvc-upper}, we prove that $\Tilde{O}_k(\sqrt{n})$ bits suffice to certify two independent spanning trees rooted at the same vertex, which leads to the following theorem.



For $k=4$, our certification scheme works unconditionally, and there is no previously known non-trivial local certification scheme.

%Itai and Zehavi~\cite{ZI89} conjectured that the equivalence also holds for $k\geq 5$.
%\begin{conjecture}[{Itai--Zehavi conjecture~\cite{ZI89}}]\label{conj: Itai--Zehavi}
    %A graph $G$ is $k$-vertex-connected if and only if for every vertex $r\in V(G)$, there exist $k$ independent spanning trees rooted at $r$.
%\end{conjecture}



Let us sketch the idea to certify that two spanning trees rooted at a common vertex are independent. The naive approach is that, for each vertex $u$, we send the information of $u$ to all its descendants in both trees; that is, we record all the information along the root-to-$v$ path. By doing so, the vertex can tell if there are any other vertices in the intersection of the two root-to-$v$ paths. It is only efficient when the tree has low depth.

To reduce complexity, we apply \emph{heavy-light decomposition}~\cite{SLEATOR1983362_heavy-light}, which partitions a tree into paths (called segments) such that each vertex belongs to the same segment as the child with the largest subtree. Heavy-light decomposition has been known as a general technique that yields efficient query algorithms on trees. In our application, heavy-light decomposition allows us to compress the tree into $O(\log n)$ layers, encode each path with at most $O(\log n)$ segments, and store the root-to-$v$ path encoding for each tree compactly. For each segment $S$ in the root-to-$v$ path, we want to bound the amount of information that $S$ should send to $v$.} \yx{not sure about the intuition or whether to add more details}

%We apply heavy-light decomposition to compress the tree into $O(\log n)$ layers and encode each path by a set of at most $O(\log n)$ segments, and we can store the root-to-$v$ path-encoding for each tree compactly. For each segment $S$ in the root-to-$v$ path, we want to bound the amount of information that $S$ should send to $v$. \yx{not sure about the intuition or whether to add more details}

A key observation is that for each vertex $u$ that belongs to segment $S_1$ in $T_1$ and segment $S_2$ in $T_2$, it suffices that one of the segments $S_i$ for $i \in \{1, 2\}$ takes the responsibility to send the information of $u$ to all its descendants in $T_i$. If a segment is short, then we can afford to let it take the responsibility, as the number of ancestors in a short segment is small. On the other hand, if a long segment takes the responsibility, then it must send the information of $u$ that also belongs to a long segment in the other tree. Intuitively, the amount of such information can be bounded, as we cannot have many long segments in each tree. Finally, we trade off the length of short segments and the number of long segments to obtain the desired bound.

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures-IST_cropped 1.pdf}
        \caption{Two spanning trees that are vertex-independent.}
        \label{fig: IST}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures-IST_cropped 2.pdf}
        \caption{Two spanning trees that are not vertex-independent}
        \label{fig: non-IST}
    \end{subfigure}
    \caption{Illustration of independent spanning trees. Both figures demonstrate two spanning trees in a ring rooted at the same vertex $r$, one in black and the other in dotted lines, oriented from the leaves to the root. In~\Cref{fig: IST}, both spanning trees are paths; the dotted one has $v_6$ as the leaf, and the other has $v_1$ as the leaf. The two trees are vertex-independent. In~\Cref{fig: non-IST}, the two trees are not vertex-independent (but still edge-independent) since the paths from $v_4$ (and also $v_5$) pass through $v_3$ in both trees.}
    \label{fig: IST-illustration}
\end{figure}

\begin{figure}[ht]
    \centering
    %\includegraphics[width=0.3\linewidth]{figures-heavy-light_cropped.pdf}
    \input{hldecomp}
    \caption{An illustration of the heavy-light decomposition. The segments are marked in black. For example, vertex $v$ has two children $v_1$ and $v_2$, and $v_1$ has more vertices in its subtree, and therefore belongs to the same segment as $v$. If a leaf does not belong to the same segment as its parent, it is itself considered a segment, see $v_3$.}
    \label{fig:heavy-light}
\end{figure}
\mtt{I use chatgpt to re-plot the previous figure. Please keep it only if it looks better.}

%\begin{restatable}{theorem}{thmKVC}\label{thm: k-vc-cert}
    %There exists an $O(k^3\sqrt{n}\log^{2.5}n)$-bit local certification scheme for $4$-vertex-connectivity. 
    %Moreover, assuming the Itai--Zehavi conjecture (\Cref{conj: Itai--Zehavi}), the same bound holds for every $k \ge 5$.
    %This holds also for any $k\geq 5$ assuming the Itai--Zehavi conjecture (\Cref{conj: Itai--Zehavi}).
%\end{restatable}

Since the upper bound for $k$-vertex-connectivity is $\Tilde{O}_k(\sqrt{n})$, while the lower bound we get is $\Omega_k(\log n)$, a natural question to ask is whether we can do better using the independent tree approach. We prove that given a labeled graph where each vertex receives two IDs that point to its parents in $T_1$ and $T_2$, certifying that $T_1$ and $T_2$ are independent spanning trees rooted at the same vertex in $G$ requires $\Omega(\sqrt{n})$ bits.

\begin{restatable}{theorem}{thmIndepST}\label{thm: indep-st-lower}
    Given a graph $G$ and two spanning trees $T_1$ and $T_2$ rooted at the same vertex $r$, certifying $T_1$ and $T_2$ are independent requires $\Omega(\sqrt{n})$ bits.
\end{restatable}

In view of \cref{thm: indep-st-lower}, the analysis of \cref{thm: k-vc-cert} is bottleneck-tight for every constant $k \ge 4$.



\subsubsection{Additional results for $2$-edge-connectivity and $2$-vertex-connectivity in the anonymous model}
\yx{the title may be changed.}
\yx{motivation need to be revised.}
{\color{blue}
Recall that our lower bound in~\Cref{thm: k-conn-lower} only works for $k\ge 3$. It is natural to ask whether $O(\log n)$ is the right complexity for certifying $2$-edge-connectivity (or $2$-vertex-connectivity). Can we get a sub-logarithmic upper bound on the restricted graph class? Or can we get a super-constant lower bound? In~\Cref{sec: 2-conn-bdd-deg}, we partially answer this question. On the upper bound side, we provide a constant-bit certification scheme for certifying $2$-edge-connecitivity and $2$-vertex-connectivity on bounded-degree graphs. Moreover, we show that for $2$-edge-connectivity, the certification scheme can be extended to bounded-expansion graphs (which includes planar graphs, and more generally, minor-free graph classes) using a very recent result in~\cite{BFVZ26}. On the other hand, we proved a super-constant lower bound for certifying $2$-vertex-connectivity via a slight modification of the lower bound for parity certification in~\cite{BFVZ26}.

\paragraph{Breaking the logarithmic barrier in restricted graph classes.}
Given a graph $G$, we say that an edge $e$ is a \emph{bridge} of $G$ if removing $e$ increases the number of connected components in $G$. A graph is \emph{bridgeless} if it does not contain a bridge. Our first observation is that $2$-edge-connectivity admits a constant-bit edge-certification scheme via a simple application of the fact that any bridgeless graph can be covered by a constant number of (possibly disconnected) Eulerian subgraphs.

\begin{restatable}{lemma}{lemTwoECedge}\label{lem: 2-ec-EdgeCert}
    There exists an $O(1)$-bit edge-certification scheme for $2$-edge connectivity.
\end{restatable}

On bounded degree graphs, the edge certification scheme can be transformed into a vertex certification scheme with an {\color{red}$\Tilde{O}(\Delta)$} overhead\footnote{In this paper, we will write explicitly the dependency on $\Delta$ in the Theorems whenever possible. In distributed graph algorithms, it is natural to consider graph classes with bounded degree. For local certification schemes, the first non-trivial bound with dependency in the max-degree $\Delta$ was given in~\cite{BFZ25}.}. 

\begin{restatable}{theorem}{thmTwoEC}\label{thm: 2-edge-conn}
    There exists an {\color{red}$O(\Delta\log\Delta)$}-bit local certification scheme for $2$-edge-connectivity on bounded-degree graphs.
\end{restatable}

This result improves upon~\cite{BFP21} when restricted to bounded-degree graphs. Their $O(\log n)$-bit local certification scheme for $2$-edge-connectivity essentially ``describes'' an ear decomposition of the graph, and simulating the ordering of the added ear may require $O(\log n)$ bits, even when the graph has constant degree. For more details, see Lemma 20 and Corollary 21 of~\cite{BFP21}.

\yx{say that 2-conn is fundamentally different from k ge 3}
}


%can be certified with complexity that depends only on $\Delta$, where $\Delta$ is the maximum degree of the input graph. 

%{\color{red}In distributed graph algorithms, it is natural to consider graph classes with bounded degree.\yx{cite papers??} For local certification schemes, the first non-trivial bound with dependency in the max-degree $\Delta$ was given in~\cite{BFZ25}. We show that $2$-edge-connectivity and $2$-vertex-connectivity can both be certified with complexity that depends only on $\Delta$.}

%For $2$-edge-connectivity, it is known that any bridgeless graph can be covered by a constant number of (possibly disconnected) Eulerian subgraphs (see \cref{lem: Eulerian-cover}), which leads to a constant-bit local certification scheme on edges. 

%On bounded degree graphs, the edge certification scheme can be transformed into a vertex certification scheme with an {\color{red}$\Tilde{O}(\Delta)$} overhead. {\color{red}For bounded degree graph, this result improves upon~\cite{BFP21}, which introduced an $O(\log n)$-bit local certification scheme for $2$-edge-connectivity. As their certification scheme essentially ``describes'' an ear decomposition of the graph, simulating the ordering of the added ear may require $O(\log n)$ bits, even when the graph has constant degree. For more details, see Lemma 20 and Corollary 21 of~\cite{BFP21}.}

For $2$-vertex-connectivity, we also obtain a constant-bit local certification scheme for bounded degree graphs by a reduction to $2$-edge-connectivity. Intuitively, we replace each vertex with an edge and split its neighbors into two nonempty sets, each connecting to a different endpoint of the edge. Observe that if the original graph is $2$-vertex-connected, then the modified graph is $2$-edge-connected regardless of how we partition the neighborhood. Conversely, we prove that if all such graphs are $2$-edge-connected, then the original graph is $2$-vertex-connected. We note that the converse direction works only for $2$-vertex connectivity, and thus the reduction cannot be generalized to certify higher connectivity.\yx{not sure whether to discuss this}
%For $2$-vertex-connectivity, we also obtain a constant-bit local certification scheme for bounded degree graphs by a reduction to $2$-edge-connectivity. Intuitively, we consider a vertex cut in the graph. If we can correctly guess how the neighbors are separated into two parts, then making those vertices into edges that connect the two parts will result in a graph that transforms vertex-connectivity to edge-connectivity. The problem is how we can simultaneously guess the neighborhood partition for all potential vertex cuts, and it can be done when we only need to tell whether the graph admits a cut vertex or not.
\begin{restatable}{theorem}{thmTwoVC}\label{thm: 2-vertex-conn}
    There exists an {\color{red}$O(2^{\Delta}\cdot\Delta\log\Delta)$}-bit local certification scheme for $2$-vertex-connectivity on bounded-degree graphs.
\end{restatable}

{\color{blue}
The main obstacle to extending~\Cref {thm: 2-edge-conn} to general graphs was that transforming edge-certification schemes to vertex-certification schemes requires vertices to distinguish certificates from different incident edges. In the previous work~\cite{FFM+23}, they showed that when the graph admits an edge-partition into a constant number of pseudoforests\footnote{In their paper, they use degeneracy as the parameter, which is equivalent to pseudoarboricity (the minimum number of pseudoforests into which its edges can be partitioned) within a factor of $2$.} and the certificates are of size $\Omega(\log n)$, an edge-certification scheme can be transformed into a vertex-certification scheme with only a constant blowup. However, in the case where the certificate size is $o(\log n)$, an additive $O(\log n)$ term is required.

A \emph{pseudoforest} is a graph where each connected component has at most one cycle, and a \emph{pseudoforest decomposition} of a graph is a partition of the edges such that each component of the partition induces a pseudoforest. We note that, in~\cite{FFM+23}, the additive $O(\log n)$ overhead comes from the cost of encoding the parent-children relationship in a pseudoforest decomposition by writing the parents' IDs on each vertex.


We show that for bounded expansion graphs, this obstacle can be overcome, and in particular, we have a constant-bit local certification scheme for $2$-edge-connectivity in the anonymous model. Bounded expansion graphs contain a broad range of well-studied graph classes, such as bounded degree graphs, planar graphs, and more generally, minor-closed graphs. The formal definition will be given in~\Cref{sec: 2-conn-bdd-deg}. We sketch the main idea as follows.

We first observe that, as long as a partition of edges into a constant number of pseudoforests is given as input to the vertices (in the sense that each vertex has at most one parent in each pseudoforest, and they have the knowledge of their own parent and children in each pseudoforest), transforming edge-certification to vertex-certification incurs only a constant overhead by letting the children take the responsibility of simulating the edge connected to the parent.

In~\cite{BFVZ26}, they show that for bounded expansion graphs, there exists a way of encoding the parent-children relationship in a certain pseudoforest using only constant bits via conflict-free coloring. Our main idea is to apply their pseudoforest certification scheme to simultaneously encode a \emph{sparse certificate} for $2$-edge-connectivity (which is a sparse subgraph that is $2$-edge-connected if and only if the original graph is) and a pseudoforest decomposition on top of it. Then we apply the edge-certification scheme in~\Cref{lem: 2-ec-EdgeCert} to the sparse certificate and then transform it into a constant-bit vertex-certification scheme.

\begin{restatable}{theorem}{thmTwoECnew}\label{thm: 2-ec-bdd-expansion}
    Let $\Fcal$ be a bounded-expansion graph class. Given the promise that the input graph belongs to $\Fcal$, there exists an $O_\Fcal(1)$-bit local certification scheme for $2$-edge-connectivity, where the constant only depends on the graph class $\Fcal$.
\end{restatable}

\begin{remark}\label{rmk: 2VC-to-2EC}
    Recall that in~\Cref{thm: 2-vertex-conn}, our reduction relies on enumerating all possible partitions of each vertex's neighborhood. Therefore, it cannot be directly generalized to bounded expansion graphs.
\end{remark}


\paragraph{A super-constant lower bound for $2$-vertex connectivity in the anonymous model.}
Our lower bound for $2$-vertex-connectivity is a slight modification of the parity lower bound in~\cite{BFVZ26}. In~\cite{BFVZ26}, the task was to certify that a graph has an even number of nodes. Their approach is to construct the  ``powerset graph'' and then glue two such graphs of even size together by identifying two nodes, one from each graph. The powerset graphs $G=(V,E)$ are bipartite graphs constructed as follows. Let $V=V_1\cup V_2$ where $V_1=[m]$ is the ground set of $m$ elements. For each subset $S\subseteq [m]$, itnroduce a vertex $v_S$ to $V_2$, and connect $v_S$ to every vertex $i\in S\subseteq V_1$. According to the finite unions theorem, they prove that if the number of labels is $o(\log^*n)$ where $n=|V|$, then there exist two subsets $S_1$ and $S_2$ such that $v_{S_1}$, $v_{S_2}$, and $v_{S_1\cup S_2}$ are colored the same. Since we are in the anonymous model, they simply take two copies of $G$, denoted by $G_1$ and $G_2$, and then identify $v_{S_1}$ in $G_1$ and $v_{S_2}$ in $G_2$ to obtain a graph $G'$ with an odd number of vertices. Notice that the identified vertex has the same view as $v_{S_1\cup S_2}$, and therefore all vertices still output \accept in $G'$. Our lower bound for $2$-vertex-connectivity follows from the observation that the construction of $G$ can be made $2$-vertex-connected, and that the combined graph $G'$ has a cut vertex (which is the identified one).

\begin{restatable}{theorem}{thmTwoVCLB}\label{thm: 2-vc-lb}
    Certifying $2$-vertex-connectivity requires $\Omega(\log(\log^*n))$ bits in the anonymous model.
\end{restatable}

We note that, since our lower bound graph for $2$-vertex-connectivity is not of bounded degeneracy,~\Cref{thm: 2-ec-bdd-expansion} and~\Cref{thm: 2-vc-lb} are incomparable.

}
 



==> k-vc-upper_backup.tex <==
\section{Certifying $k$-vertex-connectivity in $\Tilde{O}_k(\sqrt{n})$ bits}\label{sec:kvc-upper}

In this section, we show that $k$-vertex-connectivity admits a $\tilde{O}_k(\sqrt{n})$-bit local certification scheme based on the heavy--light decomposition.


\thmKVC*
%\begin{theorem}\label{thm: k-vc-cert}
    %There exists an $O(k^3\sqrt{n}\log^{1.5}n)$-bit local certification scheme for $4$-vertex-connectivity. This holds for any $k\geq 5$ assuming the Itai--Zehavi conjecture (\Cref{conj: Itai--Zehavi}).
%\end{theorem}

Given the discussion following \cref{conj: Itai--Zehavi}, it suffices to certify that there exist $k$ distinct vertices $r_1,\ldots,r_k \in V(G)$ (rather than all vertices) such that, for each $i \in [k]$, $G$ contains $k$ independent spanning trees rooted at $r_i$. We reduce this task to the following building block: fix a root $r^*$ and certify that every pair among the $k$ spanning trees rooted at $r^*$ is independent.


%The Itai--Zehavi conjecture implies that a graph $G$ is $k$-vertex-connected if and only if there exist $k$ distinct vertices $r_1,\ldots,r_k \in V(G)$ (rather than all vertices) such that, for each $i \in [k]$, $G$ contains $k$ independent spanning trees rooted at $r_i$.
\begin{lemma}\label{lem: 2-indep-tree-certification}
    Given a graph $G$, a vertex $r\in G$, and two spanning trees $T_1$ and $T_2$ on $G$ rooted at $r$ (the spanning tree inputs are of the form of the certification scheme described in \Cref{lem: BFS-cert}), there exists an $O(\sqrt{n}\log^{2.5}n)$-bit local certification scheme for certifying that $T_1$ and $T_2$ are independent.
\end{lemma}
We will describe a local certification scheme for certifying two independent spanning trees and prove \Cref{lem: 2-indep-tree-certification} in \Cref{sec: 2-indep-spt-cert}. Given this lemma, \Cref{thm: k-vc-cert} follows directly.
\begin{proof}[Proof of \Cref{thm: k-vc-cert}]
    Pick arbitrary $k$ vertices $r_1,\ldots,r_k$ in $G$. For each $i\in[k]$, we certify $k$ independent spanning trees rooted at $r_i$ by applying \Cref{lem: 2-indep-tree-certification} for $\binom{k}{2}$ pairs of spanning trees rooted at $r_i$. Therefore, the complexity increases by a factor of $O(k^3)$.%\yijun{add an explanation why doing this for $k$ vertices suffice}\mtt{It is now explained right before \cref{thm: k-vc-cert}.}
\end{proof}


\subsection{Proof of \Cref{lem: 2-indep-tree-certification}}\label{sec: 2-indep-spt-cert}
The intuition is that, given two spanning trees $T_1,T_2$ rooted at $r$, in order for a vertex $v$ to verify that the root-to-$v$ path in $T_1$ and the root-to-$v$ path in $T_2$ are internally vertex-disjoint, we need to provide $v$ with the lists of its ancestors in two trees; this could require $n\log n$ bits, which is expensive. We use heavy-light decomposition to reduce the complexity to $\Tilde{O}(\sqrt{n})$. {\color{red}For the rest of this section, when $T$ is a rooted tree, we denote by $T(v)$ to be the subtree of $T$ rooted at $v$.}

In \Cref{sec: 2-indep-spt-cert-comp}, we will describe the certificate assignment and its complexity; in \Cref{sec: 2-indep-spt-vrfy-pf}, we will describe the verification algorithm and the correctness of the entire certification scheme. Then \Cref{lem: 2-indep-tree-certification} follows.


\subsubsection{Certification assignment and the complexity}\label{sec: 2-indep-spt-cert-comp}
\paragraph{Heavy-light decomposition and path-encoding}
Let $T$ be a tree rooted at $r$. Denote by $\Psi(T)=\{S_1,\ldots,S_t\}$ the set of segments of the heavy-light decomposition on $T$. For each vertex $v\in T$, define $\seg_T(v)=i$ if $v\in S_i$. {\color{red}Recall that each vertex in $T$ belongs to exactly one segment. Moreover, for each segment $S\in\Psi(T)$, and for a vertex $v\in S$, we define the \emph{rank} of $v$ to be $j$ if $v$ is the $j$-th closest vertex to the root in $S$, denoted as $\rank_T(v)=j$.}

\begin{itemize}
    \item We encode $v$'s position in $T$ by $\eta_T(v)=(\seg_T(v),\rank_T(v))$. This requires $O(\log n)$ bits.% We call $\eta_T(v)$ the \emph{address} of $v$ in $T$.
    \item We encode the root-to-$v$ path, denoted by $P_T(r,v)$, as follows: Suppose that the root-to $v$ path in $T$ overlaps with $l$ segments $S_{i_1},\ldots,S_{i_l}$. For each $j\in[l]$, let $u_{i_j}$ be the vertex in $S_{i_j}\cap P_T(r,v)$ with the largest rank. Then we record the path-encoding $p_T(v)=\{(i_j,u_{i_j}):j\in[l]\}$ on $v$. Note that $l\in O(\log n)$ according to \Cref{fact: heavy-light_fact_0}, therefore, the path-encoding requires $O(\log^2n)$ bits.
\end{itemize}

For each vertex $v$, let $A_T(v)$ be the set of the addresses of all ancestors of $v$ in $T$. $A_T(v)=\{\eta_T(w):w\in P_T(r,v)\}$. Note that $A_T(v)$ can be obtained directly from the path-encoding $p_T(v)$. Let $\alpha_T(v)=(\eta_T(v),p_T(v))$ be the information regarding $v$'s position in $T$.


\paragraph{Certificate assignment}
Observe that to certify the independence of $T_1$ and $T_2$, it suffices for each non-root vertex $u$ to detect whether there exists another non-root vertex $v$ such that $u\in T_1(v)\cap T_2(v)$. For $i \in \{1,2\}$, let $-i$ be the complement of $i$ in the set $\{1,2\}$;  we say that $v$ is a \emph{$T_i$-ancestor} of $u$ if and only if $u\in T_i(v)$. For simplicity, let $\eta_i(v)=\eta_{T_i}(v)$, $p_i(v)=p_{T_i}(v)$, $\alpha_i(v)=\alpha_{T_i}(v)$, $P_i(r,v)=P_{T_i}(r,v)$, and $A_i(v)=A_{T_i}(v)$. We say that $\alpha_i(v)$ is the \emph{$T_i$-address} of $v$. The certificate assignment is constructed as follows:
\begin{itemize}
    \item For each vertex $v$, for all $i \in \{1,2\}$, include the $T_i$-address $(i,\alpha_i(v))$ to the certificate of $v$. Also, include the size of the $T_i$-subtree rooted at $v$, $|T_i(v)|$, to the certificate of $v$.
    \item For each vertex $v$, we choose one of the following certificate assignments. And we will define how to choose between the two options later.
    \begin{itemize}
        \item (Option $1$.) Include $(2,\alpha_2(v))$ in the certificates of all the vertices in $T_1(v)$.
        \item (Option $2$.) Include $(1,\alpha_1(v))$ in the certificates of all the vertices in  $T_2(v)$.
    \end{itemize}
    In other words, for each $i \in \{1,2\}$, each vertex $u$ receives a list of $T_{-i}$-addresses of a subset of its $T_i$-ancestors (including itself). Denote this list by $\Lambda_i(u)$. Let the above choice of $v$ be $\pi(v)$. $\pi(v)=i$ means that we choose Option $i.$ for $v$. We include this choice in the certificate of $v$ as well.
    \item (Cancellation rules.) For two distinct vertices $u,v$ such that $v\in T_1(u)$ and $u\in T_2(v)$, we remove some certificates based on the following rules:
    \begin{itemize}
        \item If $\pi(u)=\pi(v)=1$, then for every vertex $x\in T_1(v)$, we remove $(2,\alpha_2(u))$ from $\Lambda_1(x)$.
        \item If $\pi(u)=\pi(v)=2$, then for every vertex $x\in T_2(u)$, we remove $(1,\alpha_1(v))$ from $\Lambda_2(x)$.
    \end{itemize}
\end{itemize}

For each $i \in \{1,2\}$ and each segment $S\in\Psi(T_i)$, let $V(S)$ be the vertex set of this segment. Then, according to the cancellation rules, we have the following lemma:
\begin{lemma}\label{lem: seg-uniq}
    Given that $T_1$ and $T_2$ are independent. For each $i \in \{1,2\}$ and each segment $S\in\Psi(T_i)$, for any vertex $x\in G$, there exists at most one vertex $v\in V(S)$ such that $(i,\alpha_i(v))\in\Lambda_{-i}(x)$.
\end{lemma}
\begin{proof}
    We assume that $i=2$ without loss of generality. Suppose that for some segment $S\in\Psi(T_2)$, there exist two vertices $u,v\in V(S)$ and some vertex $x\in G$ such that $(2,\alpha_2(u)),(2,\alpha_2(v))\in\Lambda_1(x)$. According to the two options of sending information to children, we know that both $u$ and $v$ are ancestors of $x$ in $T_1$ (that is, $x\in T_1(u)\cap T_1(v)$) and that $\pi(u)=\pi(v)=1$. Assume that $v\in T_1(u)$ without loss of generality. Since $v$ and $u$ belong to the same segment in $T_2$, they must be in the ancestor-descendant relationship. Since $T_1$ and $T_2$ are independent and $u$ is an ancestor of $v$ in $T_1$, it must be the case that $u\in T_2(v)$. According to the cancellation rules, we must remove $(2,\alpha_2(u))$ from $\Lambda_1(x)$. A contradiction.
\end{proof}

Given this lemma, we now describe the rules for deciding the choice $\pi(v)$. 
\begin{itemize}
    \item Let $\tau$ be a threshold that will be defined later. We say that a segment is \emph{long} if its length exceeds $\tau$; otherwise, it is \emph{short}. For any rooted tree $T$, let $\Long(T)$ be the set of vertices that belong to some long segments in $T$, and let $\Short(T)$ be the set of vertices that belong to some short segments in $T$.
    \item If $v\in\Long(T_1)$, then $\pi(v)=2$. Otherwise, $\pi(v)=1$.
\end{itemize}

\paragraph{Complexity}
Intuitively, when a vertex receives the addresses from a set of vertices, we can bound the number of vertices that come from long segments, since there are not many long segments globally. We can bound the number of vertices that come from short segments, since the total number of vertices in each short segment along the path from any vertex to the root is small. More precisely, the following holds:
\begin{itemize}
    \item If $(1,\alpha_1(v))$ occurs in the certificates of $u$, then $v\in\Long(T_1)$. According to \Cref{lem: seg-uniq}, the number of such $v$ is at most the number of long segments in $T_1$, which is $O(\frac{n}{\tau})$.
    \item If $(2,\alpha_2(v))$ occurs in the certificates of $v$, then $\pi(v)=1$ according to our rule, and one of the following holds:
    \begin{itemize}
        \item $v\in\Long(T_2)$. In this case, according to \Cref{lem: seg-uniq}, the number of such $v$ is at most the number of long segments in $T_2$, which is $O(\frac{n}{\tau})$.
        \item Observe that if $v\in\Short(T_2)$ and $\pi(v)=1$, then $v\in\Short(T_1)$ according to our rules. Therefore, $v\in\Short(T_1)\cap P_1(r,u)$. Recall that the number of short segments overlapping with the root-to-$u$ path in $T_1$ is at most $O(\log n)$, and the number of such $v$ is at most $\tau\cdot O(\log n)$. 
    \end{itemize}
\end{itemize}
For each vertex $v$ and each $i \in \{1,2\}$, the set $\Lambda_i(v)$ consists of $O(\frac{n}{\tau}+\tau\cdot O(\log n))$ addresses, each of which need $O(\log^2 n)$ bits to store. Set $\tau=\sqrt{\frac{n}{\log n}}$, we get an $O(\sqrt{n}\log^{2.5}n)$ size bound for our local certification scheme.

%\begin{lemma}\label{lem: 2-indep-spt-compl}
    %The certification assignment for two independent spanning trees described in this section has size $O(\sqrt{n}\cdot\log^{2.5}n)$.
%\end{lemma}
%\begin{proof}
    
%\end{proof}


\subsubsection{Verification algorithm and correctness}\label{sec: 2-indep-spt-vrfy-pf}
\paragraph{Verification algorithm}
Recall that in our certificate assignment, for each $i \in \{1,2\}$, each vertex $v$ receives its own address $(i,\alpha_i(v))$, the choice $\pi(v)$ of which subtree to send its information to, and a list $\Lambda_i(v)$ of the $T_{-i}$-addresses of a set of its $T_i$-ancestors. The verification algorithm is as follows:
\begin{itemize}
    \item Each vertex checks the consistency between the input spanning trees and the heavy-light decomposition.
    \begin{itemize}
        \item Each vertex $v$ checks the consistency between its vertex-encoding $\eta_i(v)$ and the root-to-$v$ path-encoding $p_i(v)$: For each $i \in \{1,2\}$, $\eta_i(v)$ should be in the range of $p_i(v)$.
        \item For each $i \in \{1,2\}$, if a vertex $v$ is a leaf in $T_i$, then $|T_i(v)|=1$; otherwise, $|T_i(v)|$ is the sum of the sizes of its subtrees plus one.
        \item For each $i \in \{1,2\}$, each non-leaf vertex $v$ checks that exactly one of its children $u$ in $T_i$ with the maximum subtree-size belongs to the same segment as $v$, and the rank of $u$ is one higher than $v$.
    \end{itemize}
    %\item Each vertex checks the consistency of certificates. More specifically, for each $i=1,2$, each non-leaf vertex $v$ checks the following:
    \item Each vertex checks that the certificate assignments respect our rules. More specifically, for each $i \in \{1,2\}$, each non-leaf vertex $v$ checks the following:
    \begin{itemize}
        \item (The two options.) Each vertex can tell whether it is in a long segment or a short segment by its path-encoding. If $v\in\Long(T_1)$, then $\pi(v)=2$ and $\alpha_1(v)\in\Lambda_2(v)$. Otherwise, $\pi(v)=1$ and $\alpha_2(v)\in\Lambda_1(v)$.
        \item (The cancellation rules.) For each child $x\in T_i(v)$, the lists of the addresses $\Lambda_i(v)$ and $\Lambda_i(x)$ satisfy the following: ($1.$) $x$'s $T_{-i}$-address does not appear in $\Lambda_i(v)$, that is, $\alpha_{-i}(x)\not\in\Lambda_i(v)$; and ($2.$) if there exists $u$ such that $\alpha_{-i}(u)\in\Lambda_i(v)\setminus\Lambda_i(x)$, then $x$ must be a $T_{-i}$-ancestor of $u$ and $\pi(x)=i$. This can be checked by the path encoding in $\alpha_{-i}(u)$ and the $T_{-i}$-address of $x$.
        %\item Each vertex can tell whether it is in a long segment or a short segment by its path-encoding. If $v\in\Long(T_1)$, then $\pi(v)=2$ and each of its $T_2$-children receives $(1,\alpha_1(v))$. If it is not the case for some child $u$ in $T_2$, then $\pi(u)=\pi(v)=2$ and $u$ is its parent in $T_1$.
        %\item Otherwise, $\pi(v)=1$ and each of its $T_1$-children receives $(2,\alpha_2(v))$. If it is not the case for some child $u$ in $T_1$, then $\pi(u)=\pi(v)=1$ and $u$ is its parent in $T_2$.
        %\item Each vertex $v$ checks, respectively for each $T_i$, that for each of its children $x\in T_i(v)$, the lists of the addresses $\Lambda_i(v)$ and $\Lambda_i(x)$ is consistence with respect to our rules: ($1.$) $x$'s $T_{-i}$-address does not appear in $\Lambda_i(v)$, and ($2.$) if there exists $u$ such that $\alpha_{-i}(u)\in\Lambda_i(v)\setminus\Lambda_i(x)$, then $x$ must be a $T_{-i}$-ancestor of $u$ and $\pi(x)=i$. This can be checked by the path encoding in $\alpha_{-i}(u)$ and the $T_{-i}$-address of $x$.
        %except that $v$'s address may not appear in $\Lambda_i(u)$.
    \end{itemize}
    If any check fails, vertex $v$ outputs \reject.
    \item For each vertex $v$ and each $i \in \{1,2\}$, if there exists a label $(i,\alpha_i(u))$ in the certificate for some $u\neq v$ such that $\eta_i(u)\in A_i(v)$, then output \reject.
    \item The vertex outputs \accept\ if all the above verification passes.
\end{itemize}

\paragraph{Correctness}
Suppose that $T_1$ and $T_2$ are not independent, then there exists vertices $u,v$ such that $v\in T_1(u)\cap T_2(u)$. We assume $\pi(u)=1$ without loss of generality. Let $w$ be the vertex with the largest rank in $T_1$ that satisfies $\pi(w)=1$, $u\in T_2(w)$ and $v\in T_1(w)$. Such a vertex $w$ exists since we can take $w=u$. $w\neq v$ since otherwise $v\in T_1(u)\cap T_2(u)$ and $u\in T_2(w)$ will give us a contradiction to the fact that $T_{-i}$ is a tree. 

We claim that $(2,\alpha_2(w))$ must be added to the set $\Lambda_1(v)$. Suppose not, since $\pi(w)=1$, $(2,\alpha_2(w))\in\Lambda_1(w)$, we can find two vertices $y,z$ along the $w$--$v$ path in $T_1$ such that $y$ is the parent of $z$ and $(2,\alpha_2(w))\in\Lambda_1(y)\setminus\Lambda_1(z)$. According to our verification algorithm, this means that $z$ must be an $T_2$-ancestor of $w$ and $\pi(z)=i$, otherwise $y$ will output \reject. However, $z$ has a larger rank than $w$ in $T_i$, contradicting the way we chose $w$.

Since $v\in T_1(u)\cap T_1(w)$, $v\in T_2(u)$ and $u\in T_2(w)$, we have $v\in T_1(w)\cap T_2(w)$. According to our path encoding, $w$ belongs to $A_2(v)$, and $v$ will detect that $\eta_2(w)\in A_2(v)$ with the certificates $\alpha_2(w)$ and $\alpha_2(v)$, which make $v$ output \reject\ according to our verification algorithm. 



%Suppose that $T_1$ and $T_2$ are not independent, then there exists vertices $u,v$ such that $v\in T_1(u)\cap T_2(u)$. Suppose that $\pi(u)=i$. Let $w$ be the vertex with the largest rank in $T_i$ that satisfies $\pi(w)=i$, $u\in T_{-i}(w)$ and $v\in T_i(w)$. Such a vertex $w$ exists since we can take $w=u$. $w\neq v$ since otherwise $v\in T_1(u)\cap T_2(u)$ and $u\in T_{-i}(w)$ will give us a contradiction to the fact that $T_{-i}$ is a tree. 

%We claim that $(-i,\alpha_{-i}(w))$ must be added to the set $\Lambda_i(v)$. Suppose not, since $\pi(w)=i$, $(-i,\alpha_{-i}(w))\in\Lambda_i(w)$, we can find two vertices $y,z$ along the $w$--$v$ path in $T_1$ such that $y$ is the parent of $z$ and $(-i,\alpha_{-i}(w))\in\Lambda_i(y)\setminus\Lambda_i(z)$. According to our verification algorithm, this means that $z$ must be an $T_{-i}$-ancestor of $u$ and $\pi(z)=i$, otherwise $y$ will output \reject. However, $z$ has a larger rank than $w$ in $T_i$, contradicting the way we chose $w$.

%{\color{red}need to consider the case prover cheat}According to our certification scheme and the way we choose $w$, $(-i,\alpha_{-i}(w))$ will be added to the set $\Lambda_i(v)$ and will not be removed from it. 

%Note that since $v\in T_i(u)\cap T_i(w)$, $v\in T_{-i}(u)$ and $u\in T_{-i}(w)$, we have $v\in T_i(w)\cap T_{-i}(w)$. According to our path encoding, $w$ belongs to $A_{-i}(v)$, and $v$ will detect that $\eta_{-i}(w)\in A_{-i}(v)$, which make $v$ output \reject\ according to our verification algorithm. 



\subsection{Lower bound for certifying two independent spanning trees}\label{sec:lower-2indst}
%{\color{red}Not complete yet.}
Since the upper bound for $k$-vertex-connectivity is $\Tilde{O}_k(\sqrt{n})$, while the lower bound we get in~\Cref{sec: lower} is $\Omega_k(\log n)$, a natural question to ask is whether we can do better using the independent tree approach. In this section, we show that certifying the independence of two prescribed spanning trees rooted at the same vertex requires $\Omega(\sqrt{n})$ bits. More formally, each vertex in the network receives its parents' IDs in both spanning trees as input, and the task is to verify that the two spanning trees are independent. We construct the lower bound by a reduction from the two-party communication complexity of the Set-Disjointness problem.

Let $s$ be an integer. For every instance $(x,y)$ of a Set-Disjointness problem over $s^2$ elements, we define an instance $G_{x,y}$ on $n=(2(s+1)s+5)$ vertices. See \Cref{fig: 2-indep-st-lower} for an illustration.

%which is depicted in \Cref{fig: 2-indep-st-lower}.

\begin{itemize}
    \item The underlying graph is constructed as follows:
    \begin{itemize}
        \item The vertex set $V(G)=A\cup B\cup P\cup Q\cup\{v_1,v_2,u_1,u_2,r\}$, where $A=\{a_{i,j} : i,j\in[s]\}$, $B=\{b_{i,j} : i,j\in[s]\}$, $P=\{p_j:j\in[s]\}$, and $Q=\{q_i:i\in[s]\}$.
        \item $A$ forms a grid-like structure where each column is a clique of size $s$: For each $j\in[s]$, let $A_j=\{a_{i,j}:i\in[s]\}$, then $A_j$ induces a $K_s$. For each $i\in[s]$, $\{a_{i,j},a_{i,j+1}\}\in E(G)$ for all $j\in[s-1]$.
        \item $B$ forms a grid-like structure where each row is a clique of size $s$: For each $i\in[s]$, let $B_i=\{b_{i,j}:j\in[s]\}$, then $B_i$ induces a $K_s$. For each $j\in[s]$, $\{b_{i,j},b_{i+1,j}\}\in E(G)$ for all $i\in[s-1]$.
        \item For each $j\in[s]$, the vertex $p_j$ is connected to each vertex in $A_j\cup\{b_{1,j}\}$ with an edge. For each $i\in[s]$, the vertex $q_i$ is connected to each vertex in $B_i\cup\{a_{i,s}\}$ with an edge.
        \item The vertex $v_1$ is connected to each vertex in $P\cup\{v_2,r\}$ with an edge, and $v_2$ is connected to each vertex in $A\cup\{v_1,r\}$ with an edge. The vertex $u_1$ is connected to each vertex in $B\cup Q\cup\{u_2,r\}$, and $u_2$ is connected to each vertex in $Q\cup B_s\cup\{u_1,r\}$.
    \end{itemize}
    \item The two spanning trees on the graph $G_{x,y}$ are constructed as follows:
    \begin{itemize}
        \item For each $i\in[s]$, $(a_{i,j},a_{i,j+1})\in T_1$ for all $i\in[s-1]$ and $(a_{i,s},q_i)\in T_1$. For each $j\in[s]$, $(p_j,v_1)\in T_1$. Also, $(v_1,r)\in T_1$ and $(u_1,r)\in T_1$.
        \item For each $j\in[s]$, $(b_{i,j},b_{i+1,j})\in T_2$ for all $i\in [s-1]$ and $(p_j,b_{1,j}),(b_{s,j},u_2)\in T_2$. For each $i\in[s]$, $(q_i,u_2)\in T_2$. Also, $(v_2,r)\in T_2$ and $(u_2,r)\in T_2$.
        \item For each $i,j\in[s]$, if $x_{i,j}=0$, then $(a_{i,j},v_2)\in T_2$. For each $j\in[s]$, let $A'_j=A_j\cap\{a_{i,j}:x_{i,j}=1\}$. Let $|A'_j|=\nu_j$, for each $t\in[\nu_j]$, denote by $A'[t]$ the $t$-th element in $A'_j$ sorted by the $i$-index. Then $(A'_j[t],A'_j[t-1])\in T_2$ for all $t\in\{2,\ldots,\nu_j\}$ and $(A'_j[1],p_j)\in T_2$.
        \item For each $i,j\in[s]$, if $y_{i,j}=0$, then $(b_{i,j},u_1)\in T_1$. For each $i\in[s]$, let $B'_i=B_i\cap\{b_{i,j}:y_{i,j}=1\}$. Let $|B'_i|=\mu_i$, for each $t\in[\mu_i]$, denote by $B'_i[t]$ the $t$-th element in $B'_i$ sorted by the $j$-index. Then $(q_i,B'_i[1])\in T_1$, $(B'_i[t-1],B'_i[t])\in T_1$ for all $t\in\{2,\ldots,\mu_i\}$, and $(B'_i[\mu_i],u_1)\in T_1$.
    \end{itemize}
\end{itemize}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{2-indep-st-lower_cropped.pdf}
    \caption{Lower bound construction for certifying two independent spanning trees.}
    \label{fig: 2-indep-st-lower}
\end{figure}

\begin{lemma}\label{lem: DISJ-to-indep-st}
    $T_1$ and $T_2$ are independent if and only if $\DISJ(x,y)=\true$.
\end{lemma}
\begin{proof}
    ($\Rightarrow$) If $\DISJ(x,y)=\false$, then there exists an index $(i,j)$ such that $x_{i,j}=y_{i,j}$. According to our construction of $G_{x,y}$, there exists a path from $a_{i,j}$ to $p_{j}$ and then to $b_{i,j}$ in $T_2$; on the other hand, there is also a path from $a_{i,j}$ to $q_i$ to $b_{i,j}$ in $T_1$. Therefore, the root-to-$a_{i,j}$ path in $T_1$ and $T_2$ intersect at $b_{i,j}$, which implies that $T_1$ and $T_2$ are not independent.

    ($\Leftarrow$) We prove that if $T_1$ and $T_2$ are not independent, then $\DISJ(x,y)=\false$.
    If there exists two distinct non-root vertices $\alpha$ and $\beta$ such that the root-to-$\alpha$ paths in $T_1$ and $T_2$ intersect at $\beta$, then $\beta$ must have one outgoing edge in $T_1$, one outgoing edge in $T_2$, and at least one incoming edge in both $T_1$ and $T_2$ according to our construction of $G_{x,y}$, which implies that $\beta\in A\cup B$. Observe that $\alpha$ should also belong to $A\cup B$. (If $\alpha\in P\cup Q\cup\{v_1,v_2,u_1,u_2,r\}$, then the only possible choice of $\beta$ is $r$, which is not allowed.) It is not possible that both $\alpha,\beta$ belong to $A$: Suppose that $\alpha=a_{i,j}$, then from the $T_1$ perspective, $\beta$ must have a same $i$-index as $\alpha$; from the $T_2$ perspective, $\beta$ must have a same $j$-index as $\alpha$, this would imply $\alpha=\beta$, a contradiction. Similarly, it is impossible that both $\alpha,\beta\in B$. Therefore, we know that $\alpha\in A$ and $\beta\in B$. Suppose that $\alpha=a_{i,j}$ and $\beta=b_{i',j'}$, then $\beta$ is in the root-to-$\alpha$ path in $T_1$ if and only if $i'=i$ and there exists a path from $q_i$ to $\beta$ in $T_1$, which implies that $y_{i',j'}=1$. On the other hand, $\beta$ is in the root-to-$\alpha$ path in $T_2$ if and only if $j'=j$, and there exists a path from $a_{i,j}$ to $p_j$, which implies that $x_{i,j}=1$. In conclusion, we must have $x_{i,j}=1=y_{i',j'}=y_{i,j}$ since $i'=i$ and $j'=j$. 
\end{proof}

\thmIndepST*
%\begin{theorem}\label{thm: indep-st-lower}
   %Given a graph $G$ and two spanning trees $T_1$ and $T_2$ rooted at the same vertex $r$, certifying $T_1$ and $T_2$ are independent requires $\Omega(\sqrt{n})$ bits.
%\end{theorem}
\begin{proof}
    Consider any local certification scheme for certifying two independent spanning trees. We construct a nondeterministic protocol for $\DISJ(x,y)$ as follows:
    Alice and Bob are given the input $x$ and $y$, respectively. They then construct $G_{x,y}$ based on their inputs. Also, they are both given an advising string that consists of all the certificates along the cut $(A\cup P\cup\{v_1,v_2\},B\cup Q\cup\{u_1,u_2,r\})$ in $G_{x,y}$. Each player then enumerates all the possible labelings of the vertices that it simulates. If there exists a labeling such that all vertices in its part output \accept, then it outputs \accept.

    According to \Cref{lem: DISJ-to-indep-st}, the protocol computes the output $\true$ of $\DISJ$ correctly -- if $\DISJ(x,y)=\true$, then there exists an advising string along the cut that both Alice and Bob can fill in their part and \accept; on the other hand, if $\DISJ(x,y)=\false$, then there is no such advising string. By \Cref{fact: DISJ-com}, we know that the advising string must have length $\Omega(s^2)$. However, the number of vertices along the cut  $(A\cup P\cup\{v_1,v_2\},B\cup Q\cup\{u_1,u_2,r\})$ is $(4s+3)$, therefore, the complexity of any local certification scheme for certifying two independent spanning trees is $\Omega(\frac{s^2}{4s+3})=\Omega(\sqrt{n})$.
\end{proof}    
    %Alice and Bob are given the input $x$ and $y$, respectively. Also, they are both given an advising string that consists of the certificates along the cut $(A\cup P\cup\{v_1,v_2\},B\cup Q\cup\{u_1,u_2,r\})$. Alice then enumerates all the possible labelings of the vertices it simulates. If there exists a labeling such that all vertices output \accept, then Alice output \accept.
    %\begin{itemize}
        %\item Alice and Bob simulate the verification of independence of $T_1$ and $T_2$ as follows: Alice simulates the vertices in $A\cup P\cup\{v_1,v_2\}$, and Bob simulates the vertices in $B\cup Q\cup\{u_1,u_2,r\}$.
        %\item Alice and Bob, respectively, choose the labels of their nodes as their auxiliary bit-strings nondeterministically. They then exchange the labels along the cut, which is $A_s\cup P$ for Alice and $Q\cup B_1$ for Bob. 
        %\item Let $a$ and $b$ be the conjunction of the output values of the nodes simulated by Alice and Bob, respectively. Alice will compute $a$ and send it to Bob, while Bob will compute $b$ and send it to Alice. Both of them output the value $a\land b$.
    %\end{itemize}
    %According to \Cref{lem: DISJ-to-indep-st}, the protocol decides the value of $\DISJ(x,y)$ correctly. By \Cref{fact: DISJ-com}, we know that Alice and Bob must exchange $s^2$ bits of information, and the number of edges induced by the cut $(A\cup P\cup\{v_1,v_2\}, B\cup Q\cup\{u_1,u_2,r\})$ is $(2s+2)$. Therefore, the complexity of any local certification scheme for certifying two independent spanning trees is $\Omega(s)=\Omega(\sqrt{n})$.


==> lower.tex <==
\section{Lower bounds for $k$-connectivity for any $k\geq 3$}\label{sec: lower}
In this section, we prove that for any $k\geq 3$, certifying $k$-vertex-connectivity and $k$-edge-connectivity both require $\Omega(\log n)$ bits. 

Intuitively, we can find a $k$-(edge or vertex)-connected graph $H$ where there exists a special edge $\{u,v\}$ whose two endpoints are of bounded degree. We select $\poly(n)$ copies of the graph on distinct identifier sets. Suppose that there exists an $o(\log n)$ local certification, then there exist two instances $H_1$ and $H_2$ where the local views of the special edges $\{u_1,v_1\}$ and $\{u_2,v_2\}$ are the same. Then we can do the crossing technique, where edges $\{u_1,v_1\}$ and $\{u_2,v_2\}$ are ``kicked out'' and $u_1$ is reconnected to $v_2$ while $u_2$ is reconnected to $v_1$. The local view of each vertex remains the same if we don't consider the IDs of its neighbors. In~\cite{GS16}, they use a slightly more complicated crossing technique and prove several $\Omega(\log n)$ lower bounds even when the neighbors' IDs are taken into account. In particular, they show that one can ``glue'' two cycles where all vertices output \accept to get one long cycle that does not satisfy the property where all vertices still output accept. We adapt their technique to prove the lower bound for certifying connectivity where the local view of each vertex contains the IDs of its neighbors. 

We first state a lemma to construct lower bounds for a wider class of properties. A graph property $\Pcal$ is a set of graphs (recall that the property we consider should be closed under isomorphism). Let $G=(V,E)$ be a graph, for each vertex $v\in G$, denote by $N(v)$ the neighbors of $v$ in $G$ (not including $v$). We use $\ID(v)$ to represent the identifier of $v$.

\begin{lemma}\label{lem: general-lower-bound}
    If there exists a class of graphs $\Gcal\subseteq\Pcal$, an integer $\beta$, and a constant $n_0$ such that for each $n\geq n_0$, there exists a graph $G\in\Gcal$ where $G$ is of size at least $n$ and the following properties hold for $G$, then it requires $\Omega(\frac{\log n}{\beta})$ bits to certify $\Pcal$.
    \begin{itemize}
        \item [$(i.)$] There exists an edge $\{u,v\}\in E(G)$ such that $|N(u)|,|N(v)|\leq\beta$, and $N(u)\cap N(v)=\emptyset$.
        \item [$(ii.)$] Let $G_1$, $G_2$ be two copies of $G$ and $\{u_1,v_1\}\in E(G_1), \{u_2,v_2\}\in E(G_2)$ be the edges that correspond to $\{u,v\}$ in $G_1,G_2$ respectively. Let $G'$ be the graph obtained by removing two edges $\{u_1,v_1\},\{u_2,v_2\}$ and adding two edges $\{u_1,v_2\},\{v_1,u_2\}$. Then $G'\not\in\Pcal$.
    \end{itemize}
\end{lemma}
\begin{proof}
    Given graph $G$ and edge $\{u,v\}\in E(G)$ as in \Cref{lem: general-lower-bound}. Since the property $\Pcal$ is closed under isomorphism, we assume that the $\ID(u)=1,\ID(v)=n$, the IDs of $N(u)$ belong to $\{2,\ldots,|N(u)|+1\}$, and the IDs of $N(v)$ belong to $\{n-|N(v)|,\ldots,n-1\}$.

    Suppose the space of identifiers is $I=\{1, \ldots, n^{1+c}\}$ for some constant $c$. Let $N=n^c$. Consider any partition of $I$ into size-$\frac{n}{2}$ subsets $A_1, \cdots, A_N, B_1, \cdots, B_N$. For each identifier set $S$ defined above, we use $S[i]$ to denote the $i$-th identifier in $S$ in the natural order.

    For each pair of $(i,j)\in[N]^2$, we define a graph $C(i,j)$ that is isomorphic to $G$ (and therefore satisfies property $\Pcal$) on the identifier set $A_i\cup B_j$, such that for each $t=1,\ldots,\frac{n}{2}$, $A_i[t]$ is mapped to vertex $t$ in $G$ and $B_j[t]$ is mapped to vertex $\frac{n}{2}+t$ in $G$ under the isomorphism. For convenience, we denote $u_i=A_i[1]$ and $v_j=B_j[n]$.

    Let $c(i,j)$ be the ordered label sequence in the view of $u$ and $v$.
    \[c(i,j)=(A_i[|N(u)|+1],\ldots,A_i[1]=u_i,v_j=B_j[n],\ldots,B_j[n-|N(v)|]).\]
    Suppose that there exists four distinct indices $i,j,i',j'$ such that $c(i,j)=c(i',j')=c(i,j')=c(i',j)$, then we construct a graph $G'$ of size $n$ by gluing the graphs $C(i,j)$ and $C(i',j')$ together: We first remove the edge $(u_i,v_j)$ in $C(i,j)$ and the edge $(u_{i'},v_{j'})$ in $C(i',j')$, and then add two edges $(u_i,v_{j'})$ and $(u_{i'},v_j)$. We assign the certificates to vertices in $G'$ as in $C(i,j)$ and $C(i',j')$. One can make the following observations of $G'$:
    \begin{itemize}
        \item The local view of $u_i$ in $G'$ is the same as its local view in $C(i,j')$ since $c(i,j)=c(i,j')$. 
        \item The local view of $v_j$ in $G'$ is the same as its local view in $C(i',j)$ since $c(i,j)=c(i',j)$. 
        \item The local view of $u_{i'}$ in $G'$ is the same as its local view in $C(i',j)$ since $c(i',j')=c(i',j)$. 
        \item The local view of $v_{j'}$ in $G'$ is the same as its local view in $C(i,j')$ since $c(i',j')=c(i,j')$. 
        \item For all other vertices in $G'$, their local views are the same as in $C(i,j)$ or $C(i',j')$ depending on where they from.
    \end{itemize}
    Therefore, if there exists a certification scheme where all vertices in $C(i,j)$, $C(i,j')$, $C(i',j)$, and $C(i',j')$ output accept, all the vertices in $G'$ should output accept under our certification assignment, a contradiction. See figure \Cref{fig: crossing-tech}.

    It remains to show that such indices $(i,j,i',j')$ exist.

    Consider a complete bipartite graph $H=K_{N,N}$ on vertices $A \cup B$. Color the edge $(A[i],B[j])$ with $c(i,j)$. Suppose that we have a $o(\frac{\log n}{\beta})$ certification scheme, the information contains in $c(i,j)$ is less than $\frac{1}{\lambda}\cdot(|N(u)|+|N(v)|+2)\cdot\frac{\log n}{\beta}\leq 4\frac{\log n}{\lambda}$ for arbitrary constant $\lambda$ when $n$ sufficiently large. Pick $\lambda=\frac{4}{c}$, the number of different colors is less than $2^{\frac{c\log n}{3}}=N^{\frac{1}{3}}$. Therefore, by the pigeonhole theorem, we have a subset of edges $E'\subseteq E(H)$ of size at least $\frac{N^2}{N^{\frac{1}{3}}}=N^\frac{5}{3}$ with the same color. According to \cite{BS74}, a length-4 cycle can be found in $E'$, which is a monochromatic cycle $A[i], B[j], A[i'], B[j']$ in $H$ for some $i,j,i',j'$, then $c(i,j)=c(i',j')=c(i,j')=c(i',j)$.
\end{proof}

\begin{figure}[H]
    \centering
    \begin{minipage}[b]{0.38\textwidth}
        \centering
        \includegraphics[width=\textwidth]{crossing_figure_cropped.pdf}
        \caption{The crossing technique}
        \label{fig: crossing-tech}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.58\textwidth}
        \begin{figure}[H]
            \centering
            \begin{subfigure}{0.36\textwidth}
                \centering
                \includegraphics[width=\textwidth]{diamond-gadget_cropped.pdf}
                \caption{Diamond gadget}
                \label{fig: diamond-gadget}
            \end{subfigure}
            \hfill
            \begin{subfigure}{0.52\textwidth}
                \centering
                \includegraphics[width=\textwidth]{5-vc-planar_cropped.pdf}
                \caption{$5$-connected planar graph}
                \label{fig: 5-vc-planar}
            \end{subfigure}
            \caption{$5$-connected planar graph of arbitrary large size}
            \label{fig: 5-vc-planar-construction}
        \end{figure}
    \end{minipage}
\end{figure}

\yijun{The figures are beautiful! Figure 1 is a bit too small. Maybe display Figures 1 and 2 separately (and not horizontally)?}

Now we apply \Cref{lem: general-lower-bound} to prove lower bounds for certifying $k$-connectivity.

Observe that the connectivity of the graph $G'$ constructed in \Cref{lem: general-lower-bound} is at most $2$ and property \textit{$(ii.)$} is satisfied. Therefore, our goal is to find the $k$-edge-connected (or $k$-vertex-connected) graph class $\Gcal\subseteq\Pcal$ that satisfies property \textit{$(i.)$} in \Cref{lem: general-lower-bound}. Let $n_0$ be a constant greater than $2k$, for any $n\geq n_0$, we construct a graph $G$ of size at least $n$ which is $k$-edge-connected (or $k$-vertex-connected) as follows: 
\begin{itemize}
    \item Pick any $k$-edge-connected ($k$-vertex-connected, resp.) graph $H$ of size at least $(n-2)$.
    \item Add two vertices $u,v\not\in H$. Pick two disjoint sets of $(k-1)$ vertices $S_u$ and $S_v$ in $H$. Connect each vertex in $S_u$ to $u$ with an edge, connect each vertex in $S_v$ to $v$ with an edge, and connect $u,v$ with an edge.
\end{itemize}
{\color{red}should i prove $G$ is $k$-connected?}

For any $k$-edge-connected ($k$-vertex-connected, resp.) graph $H$ of size at least $2(k-1)$, denote the graph $G$ obtained as above as $\varphi(H)$.\yijun{I am ok with not proving that $G$ is $k$-connected, it looks obvious. But adding an explanation is also a good idea. Maybe change $\Phi()$ to something else -- $\Phi()$ is commonly used to denote the graph/cut conductance or some potential function}


\begin{theorem}
    For any integer $k\geq 3$, certifying $k$-edge-connectivity and $k$-vertex-connectivity both require $\Omega(\log n)$ bits.\yijun{Optional: You can get the dependence on $k$ in $\Omega\left(\frac{\log n}{k}\right)$ if you consider an upper bound on $|N(u)|$ and $|N(v)|$ as a parameter in the lemma. Right now in order to apply the lemma you have to assume $k$ is a constant.}
\end{theorem}
\begin{proof}
    Pick $\Gcal=\{\varphi(K_{n-2}):n\geq 2k\}$ in \Cref{lem: general-lower-bound}.\yijun{Put the above discussion in to the proof environment here.}
\end{proof}

When restricting to planar graphs, the connectivity is at most $5$. We prove that distinguishing $5$-edge-connectivity ($5$-vertex-connectivity, resp.) and $2$-edge-connectivity ($2$-vertex-connectivity, resp.) requires $\Omega(\log n)$ bits.

\begin{theorem}
    For any integer $3\leq k\leq 5$, certifying $k$-edge-connectivity and $k$-vertex-connectivity for planar graphs require $\Omega(\log n)$ bits.
\end{theorem}
\begin{proof}
    When applying the above framework, we require the graph $H$ and the graph $\varphi(H)$ to have planar embeddings. Observe that if $H$ is a planar graph such that there exists a planar embedding where there exists at least $2(k-1)$ vertices in the contour of the outer face, then we can construct $G$ by selecting $S_u$ to be the first $(k-1)$ vertices in the contour in the clockwise order, and $S_v$ the last $(k-1)$ vertices. We embed $u$ and $v$ in the outer face of $H$ and connect them to $S_u$ and $S_v$ respectively.

    Therefore, it remains to show that such $H$ exists. We adapt a $5$-vertex-connected planar graph described in~\cite{ALW25}. The idea is to place the diamond gadget in \Cref{fig: diamond-gadget} in a cycle ordering, identifying the ``apexes'' of the diamonds, and connecting each diamond gadget to the next one by two edges in the inner part of the cycle and two in the outer part of the cycle.
\end{proof}


\section{Discussion}
If we consider the dependency on $k$ in our lower bound for certifying $k$-connectivity for general graphs, the bound is $\Omega(\frac{\log n}{k})$, while our upper bound is $O(k\log n)$. Whether the gap can be closed is left as an open question.





\yijun{Why is it important that we consider 4 indices? It seems overly complicated at first sight. Can we just do something like build two thick cycles $C_1$ and $C_2$, and then argue that there are two indices that are labeled the same (by pigeonhole), so you can do the edge crossing trick. If I remember correctly from our discussion, here you want to prove something stronger: you want the lower bound to hold even with the knowledge of ID of the neighbors. Maybe explain a bit the limitation of the naive construction with two cycles and then go on to say intuitively how the more complicated construction can bypass this limitation.}
\yijun{Additional questions: (1) Can we make the lower bound work for planar graphs (when $k \leq 5$)? (2) for $2$-edge-connectivity we have an $O(1)$ upper bound for bounded-degree graphs -- what about $2$-vertex-connectivity (on bounded-degree graphs)? Do we get an $\Omega(\log n)$ lower bound  or and $O(1)$ upper bound?}



==> planar-vc.tex <==
\section{Certifying $k$-vertex-connectivity in planar graphs in $O(\log n)$ bits}

In this section, we prove the following theorem. 

\thmPlanarVC*

Since we already know that $3$-vertex-connectivity can be certified with $O(\log n)$ bits, throughout the section, we may focus on $3$-vertex-connected planar graphs $G$, although some definitions and results also work for general planar graphs. By Whitney’s unique embedding theorem, $G$ admits a unique planar embedding up to homeomorphism of the sphere. In particular, the set of faces $F(G)$ is well-defined. Throughout, all references to faces are with respect to this unique embedding. Unless otherwise stated, all paths and cycles considered in this section are \emph{simple} in that there are no repeated vertices.

 \subsection{Radial graphs}

A key ingredient in our $O(\log n)$-bit local certification scheme is a characterization
of vertex connectivity in terms of cycles in the radial graph $\Lambda(G)$.
Intuitively, the radial graph records which vertices of $G$ are incident to which
faces. While it discards the edges of $G$, it preserves the combinatorial structure
of the embedding.

Throughout, a \emph{plane graph} refers to a planar graph equipped with a fixed
combinatorial embedding, so that the face set $F(G)$ is well defined.

\begin{definition}[Radial graph]
The {radial graph} of a plane graph $G$, denoted by $\Lambda(G)$, is the bipartite
plane graph defined by
\begin{align*}
V(\Lambda(G)) \;&=\; V(G) \cup F(G),\\
E(\Lambda(G)) \;&=\; \bigl\{\, \{v,f\} \;\bigm|\; v \in V(G),\; f \in F(G),\;
\text{$v$ is incident to $f$} \,\bigr\}.
\end{align*}
In the combinatorial embedding of $\Lambda(G)$, each vertex $f\in F(G)$ is drawn in
the interior of the corresponding face of $G$.
\end{definition}

Since $\Lambda(G)$ is bipartite, every simple path or cycle in $\Lambda(G)$
alternates between vertices of $G$ and faces of $G$.

\begin{definition}[Vertex set $V_G(W)$]
Let $W$ be a simple path or cycle in $\Lambda(G)$.
We define
\[
V_G(W) \;:=\; V(W) \cap V(G)
\]
to be the set of vertices of $G$ that appear on $W$.
\end{definition}

It is well-known~\cite{Eppstein1999SubgraphJGAA} that the vertex connectivity of $G$
equals $|C|/2$, where $C$ is a shortest cycle in $\Lambda(G)$ that separates two
vertices of $G$.
Formally, we say that a cycle $C\in\Lambda(G)$ is \emph{$G$-separating} if there exist
two vertices $u,v\in V(G)$ such that $u$ lies in the interior of $C$ and $v$ lies in
the exterior of $C$.
The following lemma captures this correspondence.

\begin{lemma}[Minimum vertex cuts $\leftrightarrow$ minimum separating cycles~{\cite{Eppstein1999SubgraphJGAA}}]
\label{lem:separating}
For any minimum vertex cut $S$ of $G$, there exists a $G$-separating cycle
$C\in\Lambda(G)$ such that $S = V_G(C)$.
Conversely, for any $G$-separating cycle $C\in\Lambda(G)$, the set
$S = V_G(C)$ is a vertex cut of $G$.
\end{lemma}

Directly handling separating cycles in local certification is
challenging.
Instead, in the remainder of this section we introduce a refined notion that is
better suited to our setting, particularly when $G$ is $3$-vertex-connected.

Let $W = (x_0,x_1,\dots,x_\ell)$ be a simple path or cycle in $\Lambda(G)$.
As we traverse $W$, every time we see a subsequence of the form
\[
x_i = v,\quad x_{i+1} = f,\quad x_{i+2} = v'
\]
with $v,v'\in V(G)$ and $f\in F(G)$, we read this as recording that the face $f$
lies between the vertices $v$ and $v'$ along $W$.
When $W$ is a cycle, indices are taken modulo $\ell+1$.

Intuitively, an edge of $G$ between two vertices of $V_G(W)$ is compatible with this
structure only if it connects two consecutive vertices $v,v'$ that appear with a
face $f$ between them on $W$, and the edge $\{v,v'\}$ lies on the boundary of $f$.

\begin{definition}[$W$-facial edges]
Let $W = (x_0,x_1,\dots,x_\ell)$ be a path or cycle in $\Lambda(G)$.
An edge $e = \{u,w\} \in E(G)$ with $u,w \in V_G(W)$ is called {$W$-facial} if
there exists an index $i$ with $0 \le i \le \ell-2$ and a face $f \in F(G)$ such that
\[
(x_i,x_{i+1},x_{i+2}) = (u,f,w)
\]
and the edge $\{u,w\}$ lies on the boundary of the face $f$.
\end{definition}


Any edge of $G$ between two vertices of $V_G(W)$ that is not $W$-facial introduces an
adjacency not recorded by $W$, and hence forms a shortcut in the boundary structure
induced by $W$.

\begin{definition}[$G$-chordless paths and cycles]
A path or cycle $W$ in $\Lambda(G)$ is called {$G$-chordless} if every
edge of $G$ whose endpoints both lie in $V_G(W)$ is $W$-facial.
\end{definition}


To characterize vertex connectivity via cycles in $\Lambda(G)$, we must also exclude
cycles that are confined to a single face of $G$.
For any $f\in F(G)$, let $\partial f$ denote the boundary cycle of $f$.

\begin{definition}[$G$-facial cycles]\label{def:Gfacial}
A cycle $C$ in $\Lambda(G)$ is called {$G$-facial} if there exists a face
$f\in F(G)$ such that
\[
V_G(C) \;\subseteq\; \partial f.
\]
\end{definition}

Equivalently, $C$ is $G$-facial if all vertices of $G$ appearing on $C$ lie on the
boundary of a single face.
When $G$ is $3$-vertex-connected, such cycles are never $G$-separating in the sense
of \Cref{lem:separating}, and can therefore be excluded.

\begin{lemma}[Excluding $G$-facial cycles]\label{lem:nonsep}
If $G$ is $3$-vertex-connected, then every $G$-facial cycle $C$ in $\Lambda(G)$ is not
$G$-separating.
\end{lemma}

\begin{proof}
Fix a $G$-facial cycle $C\subseteq\Lambda(G)$.
By definition, there exists a face $f\in F(G)$ such that
\[
S \;:=\; V_G(C) \;\subseteq\; \partial f.
\]
Suppose for contradiction that $C$ is $G$-separating.
Then there exist vertices $u,v\in V(G)$ such that $u$ lies in the interior of $C$ and
$v$ lies in the exterior of $C$.
In particular, $u,v\notin S$, and $S$ is a vertex cut separating $u$ and $v$.

\paragraph{Choosing three attachment vertices on $\partial f$.}
Since $G$ is $3$-vertex-connected, Menger’s theorem guarantees the existence of three
internally vertex-disjoint $u$--$v$ paths $P_1,P_2,P_3$.
Each path $P_i$ must intersect $S$, and since $u,v\notin S$ and the paths are
internally disjoint, we may choose distinct vertices
$x_1,x_2,x_3\in S$ such that $x_i\in P_i$ for each $i$.

\paragraph{Adding a face-apex vertex.}
Let $G^\star$ be the plane graph obtained from $G$ by adding a new vertex $a_f$ in the
interior of the face $f$ and connecting it to every vertex of $\partial f$ by edges
drawn entirely inside $f$.
This operation preserves planarity.

We now exhibit a $K_{3,3}$-minor in $G^\star$.
Let
\[
L \;:=\; \{u,v,a_f\}
\qquad\text{and}\qquad
R \;:=\; \{x_1,x_2,x_3\}.
\]
For each $i$, the edge $\{a_f,x_i\}$ is present since $x_i\in\partial f$.
Let $Q_i^u$ and $Q_i^v$ denote the subpaths of $P_i$ from $u$ to $x_i$ and from $v$ to
$x_i$, respectively.
By construction, the six paths
$Q_1^u,Q_2^u,Q_3^u,Q_1^v,Q_2^v,Q_3^v$ are internally vertex-disjoint, with intersections
only at their endpoints.

Together, these paths and edges realize a $K_{3,3}$-minor in $G^\star$, contradicting
the planarity of $G^\star$.
Hence, $C$ cannot be $G$-separating.
\end{proof}

\subsection{A characterization of vertex connectivity}

Building on \Cref{lem:nonsep}, we now establish a precise characterization of vertex
connectivity in terms of cycles in the radial graph.

\begin{lemma}[Vertex connectivity via cycles in $\Lambda(G)$]\label{thm:kappa-radial}
For any $3$-vertex-connected planar graph $G$, the vertex connectivity of $G$ equals
\[
\frac12 \cdot
\min\Bigl\{\,|C| \;\bigm|\; C \text{ is a $G$-chordless and non-$G$-facial cycle in }
\Lambda(G)\Bigr\}.
\]
\end{lemma}

\Cref{thm:kappa-radial} follows by establishing a tight correspondence between minimum vertex
cuts of $G$ and a restricted class of cycles in the radial graph.
In one direction, we show that every $G$-chordless, non-$G$-facial cycle induces a
vertex cut whose size equals the number of vertices of $G$ appearing on the cycle.
In the other direction, we show that every minimum vertex cut gives rise to such a
cycle.
Combining these two directions yields the claimed characterization.

\begin{lemma}[Cycles $\rightarrow$ cuts]\label{lem:cycle-to-cut}
For any cycle $C$ in $\Lambda(G)$ that is $G$-chordless and non-$G$-facial, the set
$S = V_G(C)$ is a vertex cut of $G$.
\end{lemma}

\begin{proof}
Write
\[
C = (v_1,f_1,v_2,f_2,\dots,v_k,f_k,v_1)
\qquad\text{and}\qquad
S := V_G(C) = \{v_1,\dots,v_k\}.
\]

We first realize $C$ as a simple closed curve that intersects the drawing of $G$
only at the vertices of $S$ and along $C$-facial edges.
For each index $i$, we choose an arc $\alpha_i$ as follows.
\begin{itemize}
    \item If $\{v_i,v_{i+1}\}$ is a $C$-facial edge, let $\alpha_i$ be the drawing of
    this edge.
    \item Otherwise, choose an arc $\alpha_i$ contained in the interior of the face
    $f_i$ that connects $v_i$ to $v_{i+1}$ and intersects the drawing of $G$ only at
    its endpoints. This is possible since both vertices are incident to $f_i$.
\end{itemize}

Let $\gamma := \alpha_1 \cup \cdots \cup \alpha_k$.
By construction, $\gamma$ is a simple closed curve.
Let $\mathcal{D}_1$ and $\mathcal{D}_2$ denote the two connected components of the
sphere minus $\gamma$.

We claim that both $\mathcal{D}_1$ and $\mathcal{D}_2$ contain at least one vertex of
$G$.
Suppose for contradiction that one component, say $\mathcal{D}_1$, contains no
vertex of $G$.
If there exists an edge $\{v_i,v_j\}\in E(G)$ between two vertices of $S$ whose
drawing, excluding endpoints, lies entirely in $\mathcal{D}_1$, then this edge is
not $C$-facial, contradicting the assumption that $C$ is $G$-chordless.
Thus, no such edge exists.

It follows that all vertices of $S$ are incident to a common face of $G$, implying
that $C$ is $G$-facial, a contradiction.
Therefore, both $\mathcal{D}_1$ and $\mathcal{D}_2$ must contain vertices of $G$.

Choose vertices $x \in \mathcal{D}_1 \cap V(G)$ and $y \in \mathcal{D}_2 \cap V(G)$.
Consider any $x$--$y$ path $P$ in $G$.
If $P$ avoids $S$, then its drawing is disjoint from $\gamma$, since $\gamma$
intersects the drawing of $G$ only at vertices in $S$.
This is impossible, as a connected set disjoint from a simple closed curve cannot
connect points in different components of the sphere minus that curve.
Hence every $x$--$y$ path intersects $S$, and $S$ is a vertex cut of $G$.
\end{proof}

\begin{lemma}[Cuts $\rightarrow$ cycles]\label{lem:make-chordless}
Let $S$ be a minimum vertex cut of $G$.
Then there exists a $G$-chordless and non-$G$-facial cycle $C$ in $\Lambda(G)$ such
that $V_G(C)=S$.
\end{lemma}

\begin{proof}
By \Cref{lem:separating}, there exists a $G$-separating cycle
$C \in \Lambda(G)$ with $V_G(C)=S$.
By \Cref{lem:nonsep}, this cycle is non-$G$-facial.
It therefore suffices to show that $C$ can be chosen to be $G$-chordless.

Write
\[
C = (v_1,f_1,v_2,f_2,\dots,v_k,f_k,v_1).
\]
Suppose for contradiction that $C$ is not $G$-chordless.
Then there exists an edge $e=\{v_i,v_j\}\in E(G)$ with $j\notin\{i-1,i+1\}$ (indices
taken modulo $k$).
Let $P_1$ and $P_2$ denote the two subpaths of $C$ between $v_i$ and $v_j$.
Let $C_1$ and $C_2$ be the cycles obtained by combining $e$ with $P_1$ and $P_2$,
respectively.

Consider a drawing of $\Lambda(G)$ in which the edge $e$ lies in the interior of $C$.
Since $C$ is $G$-separating, at least one of $C_1$ or $C_2$ is $G$-separating.
Moreover, the set of vertices of $G$ appearing on such a cycle is a strict subset
of $S$.
This yields a vertex cut of size strictly smaller than $|S|$, contradicting the
minimality of $S$.
Hence $C$ must be $G$-chordless.
\end{proof}

We now combine the two directions to prove the main theorem.

\begin{proof}[Proof of \Cref{thm:kappa-radial}]
Let $\kappa(G)$ denote the vertex connectivity of $G$, and let
$\kappa^\star(G)$ be the minimum length of a $G$-chordless, non-$G$-facial cycle in
$\Lambda(G)$.
By \Cref{lem:cycle-to-cut}, we have $\kappa(G) \le \kappa^\star(G)/2$.
Conversely, \Cref{lem:make-chordless} implies $\kappa(G) \ge \kappa^\star(G)/2$.
Therefore, $\kappa(G) = \kappa^\star(G)/2$, as required.
\end{proof}

\subsection{Potentially problematic faces and paths}

Our goal is to find a shortest $G$-chordless, non-$G$-facial cycle $C$ in $\Lambda(G)$ using a dynamic programming approach. In this framework, each subproblem is solved by computing collections of $G$-chordless paths that may eventually be combined to form the desired cycle $C$. The principal challenge is enforcing the non-$G$-facial condition: in the worst case, determining whether a cycle is $G$-facial requires knowledge of the entire cycle. Consequently, when working with partial solutions consisting only of paths, it is unclear what information must be retained in order to rule out $G$-facial cycles.

In this section, we develop the key tools needed to overcome this difficulty. Specifically, we show that for any given path $P$, ensuring that $P$ does not extend to a $G$-facial cycle requires avoiding only a bounded number of \emph{potentially problematic} faces and subpaths.

\begin{lemma}[Faces shared by two vertices]\label{clm:two-vertices-two-faces_v2}
Let $G$ be a $3$-vertex-connected plane graph, and let $a,b\in V(G)$ be distinct
vertices. Then there are at most two faces $g\in F(G)$ such that $a,b\in \partial g$.
\end{lemma}

\begin{proof}
Suppose for contradiction that there exist three distinct faces $g_1,g_2,g_3$ such
that $a,b\in \partial g_i$ for all $i\in\{1,2,3\}$.

For each $i$, draw a simple curve $P_i$ from $a$ to $b$ entirely in the interior of
$g_i$, except for its endpoints $a$ and $b$.
The three curves
$P_1,P_2,P_3$ are pairwise internally disjoint, and they only intersect $G$ at $a$
and $b$.
The union $P_1 \cup P_2 \cup P_3 \cup \{a,b\}$ consists of three internally disjoint
curves from $a$ to $b$ and partitions the sphere into three regions.

Because $G$ is simple, at most one of these regions can have boundary consisting of a
single edge $\{a,b\}$.
Hence at least two of the regions contain vertices of $G$ other than $a$ and $b$.
Therefore, $G-\{a,b\}$ is disconnected, so $\{a,b\}$ is a vertex cut of size $2$,
contradicting the assumption that $G$ is $3$-vertex-connected.
\end{proof}


\begin{lemma}[Potentially problematic faces]\label{lem:badfaces}
Let $G$ be a $3$-vertex-connected plane graph, and let $P$ be a path of length at least one in $\Lambda(G)$.
Then there are at most $3$ faces $g \in F(G)$ for which there exists a $G$-facial cycle
$C$ in $\Lambda(G)$ that contains $P$ as a subpath and satisfies
$V_G(C)\subseteq \partial g$.
\end{lemma}

\begin{proof}
Write
\[
P=(x_0,x_1,\dots,x_\ell),
\]
and let
\[
X := V(G)\cap \{x_0,x_1,\dots,x_\ell\}
\]
be the set of vertices of $G$ appearing on $P$. Since $P$ has length at least one, $X\neq\emptyset$.

We say that a face $g\in F(G)$ is \emph{witnessing} if there exists a $G$-facial cycle
$C$ containing $P$ as a subpath and satisfying $V_G(C)\subseteq \partial g$.
We have
\[
X \subseteq V_G(C) \subseteq \partial g,
\]
so every vertex of $G$ appearing on $P$ lies on $\partial g$.
We now distinguish cases and show that the number of witnessing faces is at most $3$.

\paragraph{Case 1: $|X|\ge 2$.}
Let $a$ and $b$ be two distinct vertices of $G$ on $P$. Then any witnessing face $g$
must satisfy $a,b\in \partial g$.
By \Cref{clm:two-vertices-two-faces_v2}, there are at most two such faces.
Hence there are at most $2$ witnessing faces in this case.

\paragraph{Case 2: $|X|=1$.}
Let $X=\{a\}$. Since $\Lambda(G)$ is bipartite, the path $P$ has length at most two, and must be of one of the following forms:
\[
(a,f),\quad (f,a),\quad\text{or}\quad (f_1,a,f_2),
\]
where $f,f_1,f_2$ are faces incident to $a$.
It suffices to consider the case $P=(a,f)$, since the case $(f,a)$ is symmetric and the case $(f_1,a,f_2)$ contains a subpath of this form.

Fix $P=(a,f)$. Let $g$ be a witnessing face, witnessed by a $G$-facial cycle $C$ with
$V_G(C)\subseteq \partial g$ and containing $(a,f)$ as a subpath.
In $C$, the subpath $(a,f)$ indicates that the cycle uses the incidence of $a$ with the face $f$.

Because $G$ is $3$-vertex-connected, every facial boundary is a simple cycle. Hence the vertex $a$ appears exactly once on $\partial f$ and is incident there with exactly two edges; denote them by $e_1$ and $e_2$.
Let $g_1$ and $g_2$ be the (unique) faces on the other side of $e_1$ and $e_2$, respectively.

We claim that any witnessing face $g$ must lie in $\{f,g_1,g_2\}$.
Indeed, for a $G$-facial cycle $C$ supported on $\partial g$ to include the subpath $(a,f)$, the traversal of $C$ through $a$ must be compatible with the boundary walk of $\partial g$ at $a$.
At $a$, the boundary $\partial g$ uses exactly two incident edges; if neither is $e_1$ nor $e_2$, then $(a,f)$ cannot occur as a subpath of $C$.
Thus $\partial g$ must use at least one of $e_1,e_2$ at $a$, forcing $g$ to be either $f$, $g_1$, or $g_2$.
Hence there are at most $3$ witnessing faces in this case.
\end{proof}

\begin{lemma}[Potentially problematic subpaths]\label{lem:badpaths}
Let $P$ be a path of length at least one in $\Lambda(G)$.
Let $u$ and $v$ be distinct vertices of $\Lambda(G)$, and let $\ell$ be a positive integer.
Then there are at most $36$ distinct paths $P'$ satisfying the following conditions:
\begin{itemize}
    \item The length of $P'$ is $\ell$.
    \item $P'$ starts at $u$ and ends at $v$.
    \item There exists a $G$-facial cycle $C$ in $\Lambda(G)$ of length at most $10$
    that contains both $P$ and $P'$ as subpaths.
\end{itemize}
\end{lemma}

\begin{proof}
Let $P'$ be a path from $u$ to $v$ of length $\ell$ such that there exists a
$G$-facial cycle $C$ in $\Lambda(G)$ of length at most $10$ containing both $P$
and $P'$ as subpaths.
By \Cref{def:Gfacial}, there exists a face $g\in F(G)$ such that
\[
V_G(C)\subseteq \partial g,
\]
that is, all vertices of $G$ used by $C$ lie on the boundary of a single face $g$.
By \Cref{lem:badfaces}, for the fixed path $P$ there are at most three such
faces $g$. We fix one such face and bound the number of possible paths $P'$ arising
from cycles supported on it. Multiplying the bound by $3$ will then give the desired
result.

 Since $G$ is $3$-vertex-connected,
$\partial g$ is a simple cycle.
We also use the standard fact that in a $3$-vertex-connected plane graph, any two
distinct faces share at most one edge; otherwise, selecting one endpoint from each
of two shared edges would yield a vertex separator of size at most $2$, contradicting
$3$-vertex-connectivity.

\paragraph{Structure of a cycle $C$ with $V_G(C)\subseteq \partial g$.}
Let
\[
C=(a_1,f_1,a_2,f_2,\dots,a_t,f_t,a_1)
\]
be a $G$-facial cycle of length at most $10$ with $V_G(C)\subseteq \partial g$.
Since $\Lambda(G)$ is bipartite, $|C|=2t\le 10$, and therefore
\[
t=|V_G(C)|\le 5.
\]
Let $S:=V_G(C)\subseteq \partial g$ be the set of vertices of $G$ appearing on $C$.

We now explain the two possible ways in which $C$ can move between vertices of $B$.

\paragraph{Standard moves.}
Consider a subpath of $C$ of the form $(a_i,f,a_{i+1})$ with $f\neq g$.
In this situation, the cycle moves from the vertex $a_i$ to the vertex $a_{i+1}$
through a face $f$ that is distinct from $g$.
Since both $a_i$ and $a_{i+1}$ lie on the boundaries of $f$ and $g$, they lie on the
common boundary of these two faces.
Because distinct faces share at most one edge, $a_i$ and $a_{i+1}$ must be consecutive
vertices on $\partial g$, and the step from $a_i$ to $a_{i+1}$ corresponds exactly to traversing
that single boundary edge of $\partial g$.
Thus, a standard move advances the cycle by one edge along $\partial g$.

\paragraph{Special moves.}
Now consider a subpath of $C$ of the form $(a_i,g,a_j)$.
Here the cycle moves from $a_i$ to $a_j$ through the face $g$ itself.
Since $C$ is simple, the face $g$ can appear at most once on $C$, and hence there is
at most one such subpath.
Unlike a standard move, this step is not constrained to consecutive vertices of $\partial g$:
the vertices $a_i$ and $a_j$ may be separated by several edges along $\partial g$.
In terms of the boundary cycle $\partial g$, this corresponds to a single \emph{jump} that skips
over an entire interval of $\partial g$.

\paragraph{Summary.} When the vertices of $S$ are listed in their cyclic order along $\partial g$, the
cycle $C$ proceeds by moving along consecutive vertices using standard moves, with
the possibility of at most one special move that jumps across a contiguous segment
of $\partial g$.
Since $|S|\le 5$, there are at most $5$ such moves in total.

\paragraph{Counting admissible paths $P'$.}
We now count the number of possible paths $P'$ of length $\ell$ from $u$ to $v$ that may arise as subpaths of a cycle $C$ as described above. Since $C$ is entirely supported on $\partial g$, every vertex of $P'$ must either belong to $\partial g$ or correspond to a face incident with an edge of $\partial g$. If this condition fails for either $u$ or $v$, then no such path $P'$ exists. We therefore restrict our attention to the case where both $u$ and $v$ satisfy this condition.



\paragraph{Case 1: neither $u$ nor $v$ equals $g$.}
Along the cycle $C$, the path $P'$ corresponds to a
contiguous segment of the traversal of $\partial g$, possibly containing a
special move.

There are two possible directions:
clockwise or counterclockwise.
We fix one orientation and count the number of admissible paths in that direction;
the final bound will then be doubled.

Suppose first that $P'$ uses only standard moves.
Recall that a standard move advances by exactly one edge $e$ along $B$ via the face $f \neq g$ incident to $e$.
Thus, starting from $u$, repeated standard moves uniquely determine the
next vertex at each step.
Hence, for the fixed orientation, there is exactly one path from $u$
to $v$ consisting entirely of standard moves.
If the length of the path is exactly $\ell$,
then this yields exactly one admissible path $P'$.
Otherwise, no path of length $\ell$
using only standard moves exists. 

Now consider paths that use the special move.
Recall that there is at most one special move on $C$, and that
$C$ contains at most $5$ moves in total.
Therefore, along the traversal from $u$ to $v$, there are at most
$5$ possible positions at which the special move could occur.
Once we choose the position at which the special move is used,
the remainder of the path is determined uniquely, as $u$ and $v$ are fixed:
before the special move, the path follows standard moves along $\partial g$,
then it performs the jump via $g$,
and afterwards it again continues with standard moves along $\partial g$
until it reaches $v$.
Thus, for the fixed orientation, there are at most $5$ admissible
paths that use the special move.

Combining the possibilities, for the fixed orientation, there are
at most $1+5=6$ admissible paths $P'$.
Since there are two orientations of $\partial g$, the total number of
admissible paths in this case is at most $12$.

\paragraph{Case 2: one of $u$ and $v$ equals $g$.}
Without loss of generality, assume that $v=g$.
Then any admissible path $P'$ must end with the special move,
since $g$ can only be reached through a subpath of the form
$(a_i,g,a_j)$.
Consequently, the final step of $P'$ is uniquely determined:
it must be the unique special move of $C$.

Before this final step, $P'$ can only consist of standard moves
along $\partial g$.
As in Case~1, once we fix an orientation of $\partial g$,
the sequence of standard moves from $u$ is uniquely determined.
Thus, for a fixed orientation, there is at most one admissible path
ending at $g$.
Since there are two possible orientations of $\partial g$, the total number
of admissible paths in this case is at most $2$.


Therefore, for a fixed face $g$, there are at most $12$ admissible paths $P'$.
Since there are at most $3$ possible choices for $g$, the total number of such paths
is at most $36$.
\end{proof}





\subsection{Dynamic programming on treedepth decompositions}
 

\paragraph{Treedepth.}
A \emph{treedepth decomposition} of a graph $G=(V,E)$ is a rooted forest $F$
with vertex set $V$ such that for every edge $\{u,v\}\in E$,
one of $u$ and $v$ is an ancestor of the other in $F$.
The \emph{height} of $F$ is the maximum number of vertices on a root--to--leaf path.

The \emph{treedepth} of $G$, denoted by $\td(G)$,
is the minimum height of a treedepth decomposition of $G$.
Equivalently, $\td(G)$ is the smallest integer $h$
such that $G$ is a subgraph of the closure of a rooted forest of height $h$,
where the closure connects every vertex to all of its ancestors.

\paragraph{Low-treedepth colorings.}
Let $\mathcal G$ be a class of graphs.
We say that $\mathcal G$ \emph{admits low-treedepth colorings}
if there exist functions
\[
f \colon \mathbb N \to \mathbb N
\qquad\text{and}\qquad
k \colon \mathbb N \to \mathbb N
\]
such that for every integer $p \ge 1$ and every graph $G \in \mathcal G$,
there exists a vertex coloring
\[
\varphi \colon V(G) \to [k(p)]
\]
with the following property:
for every subset $X \subseteq [k(p)]$ with $|X| \le p$,
the subgraph of $G$ induced by vertices whose colors lie in $X$
has treedepth at most $f(p)$.

We recall the following fundamental characterization.

\begin{theorem}[Ne\v{s}et\v{r}il--Ossona de Mendez~\cite{nesetril-odm-sparsity}]
A class of graphs has bounded expansion if and only if it admits
low-treedepth colorings.
\end{theorem}

It is well known that planar graphs form a class of bounded expansion.
Consequently, planar graphs admit low-treedepth colorings.

 
Recall that the minimum degree of any planar graph is at most $5$, so the vertex
connectivity of any planar graph is at most $5$.
Therefore, by \Cref{thm:kappa-radial}, it suffices to consider $G$-chordless and
non-$G$-facial cycles in $\Lambda(G)$ of length at most $10$.

\paragraph{Reduction to bounded treedepth components.}
For our dynamic programming algorithm, we work with the plane graph obtained by adding the edges of
$G$ to the radial graph $\Lambda(G)$.
Formally, let
\[
R(G)
\]
be the graph with vertex set $V(\Lambda(G)) = V(G) \cup F(G)$ and edge set
$E(\Lambda(G)) \cup E(G)$.

We apply a low-treedepth coloring to $R(G)$ with parameter $p=10$, and let
\[
\varphi \colon V(R(G)) \to [k(10)]
\]
be the resulting coloring.
For every choice of $10$ colors $X \subseteq [k(10)]$, consider the induced subgraph
\[
K_X := R(G)\bigl[\varphi^{-1}(X)\bigr].
\]
By definition of low-treedepth colorings, each $K_X$ has treedepth at most $f(10)$,
which is a constant.

Any $G$-chordless and non-$G$-facial cycle $C$ in $\Lambda(G)$ of length at most $10$
uses at most $10$ vertices of $R(G)$.
All these vertices receive colors under $\varphi$, so there exists a set
$X \subseteq [k(10)]$ of size $10$ such that every vertex of $C$ has color in $X$.
Consequently, $C$ is entirely contained in the induced subgraph $K_X$, and its edges
belong to the radial part $\Lambda(G)$ of $K_X$.

Therefore, it suffices to search for a shortest $G$-chordless and non-$G$-facial
cycle independently inside each $K_X$.
From now on, we fix one such color set $X$, and focus on a single connected component $H$ of $K_X$.


\paragraph{Treedepth notation.}
Fix a treedepth decomposition $T$ of $H$.
Since $H$ is connected, $T$ is a rooted tree.
For a vertex $v \in V(T)$, we write
\[
A(v)
\]
for the set of ancestors of $v$ in $T$ (excluding $v$ itself),
and
\[
D(v)
\]
for the set of vertices in the subtree of $T$
rooted at $v$ (including $v$). Because the height of $T$ is bounded by a constant,
the sets $A(v)$ have constant size. 

Our goal is to design a dynamic programming algorithm over the decomposition $T$ that
finds a shortest $G$-chordless and non-$G$-facial cycle contained in $H$, restricted
to cycles of length at most $10$ and uses only the edges in $\Lambda(G)$.
Moreover, the algorithm must be structured so that its execution can be certified
using $O(\log n)$-bit labels.

\paragraph{High-level overview.}
In our dynamic programming table at each vertex $v$, we enumerate all guesses for the
positions of the ancestors $A(v)$ on the final cycle $C$, and for each such pattern
we store possible partial realizations of $C$ using subpaths whose internal vertices
lie in $D(v)$.
When we merge solutions from different child subtrees of $v$, no new chords can
appear between them, since the definition of a treedepth decomposition forbids edges
between internal vertices of distinct child subtrees.
The non-$G$-facial condition is handled indirectly: for each boundary configuration
we keep up to a constant number $\tau$ of partial solutions, and \Cref{lem:badpaths}
guarantees that if the partial solution corresponding to $C$ is not stored, then among
the stored candidates there is one that yields a non-$G$-facial cycle.



\subsubsection{Dynamic programming tables}

Fix the constant
\[
\tau \;:=\; 36^5 + 1.
\]

For a vertex $v \in V(T)$, we describe partial realizations of a cycle $C$ in
$\Lambda(G)$ by specifying how $C$ meets the ancestor set $A(v)$ and which portions
between ancestors are already realized using vertices in $D(v)$.

\paragraph{Cycle pattern.} A \emph{cycle pattern at $v$} is a cyclic sequence
\[
  (y_1,y_2,\dots,y_m)
\]
of length $m \in \{6,8,10\}$, where each $y_j$ is either a vertex of $A(v)$ or the
special symbol $\bot$.
We require that every vertex of $A(v)$ appears at most once in the sequence, whereas
$\bot$ may appear multiple times.
Intuitively, the entries from $A(v)$ are exactly the ancestors that lie on the cycle
$C$, listed in their cyclic order along $C$, and the symbol $\bot$ marks positions
occupied by vertices outside $A(v)$.

\paragraph{Intervals.} Within the cyclic sequence $(y_1,\dots,y_m)$, we consider all maximal subsequences of
the form
\[
  I = (y_p,y_{p+1},\dots,y_q)
\]
such that $y_p,y_q \in A(v)$, every internal term $y_{p+1},\dots,y_{q-1}$ equals
$\bot$, and $q \geq p+2$ (indices are taken modulo $m$).
We call these subsequences the \emph{intervals} of the pattern.
For such an interval $I = (y_p,\dots,y_q)$, its endpoints are $x := y_p$ and
$x' := y_q$, and its \emph{length} is
\[
  L(I) \;:=\; q-p \geq 2,
\]
The set of intervals of a pattern $\Pi$ is denoted by $\mathcal I(\Pi)$.

\paragraph{State descriptor.} Let $\Pi$ be a cycle pattern at $v$.
A \emph{state descriptor at $v$} is a pair $(\Pi,J)$, where
$J$ is a non-empty subset of $\mathcal I(\Pi)$.
Intuitively, $J$ specifies which intervals of the pattern are already realized using
vertices in $D(v)$; the remaining intervals in $\mathcal I(\Pi)\setminus J$ must be
realized outside $D(v)$.

\paragraph{Solution.} For a given state descriptor $(\Pi,J)$, a \emph{solution at $v$ for $(\Pi,J)$} is a
collection $\mathcal Q$ of paths in $H$ with the following
properties:

\begin{description}
  \item[Interval constraints.]
        For every interval
        \[
          I = (y_p,\dots,y_q) \in J
        \]
        with endpoints $x := y_p$ and $x' := y_q$, the collection $\mathcal Q$
        contains exactly one path $P_I$ from $x$ to $x'$ in $\Lambda(G)$ of length
        $L(I)$.

  \item[Vertex constraints.]
        Every internal vertex of every path $P_I$ lies in $D(v)$, and the endpoints
        $x,x'$ lie in $A(v)$.
        In particular, all vertices of the paths lie in $A(v)\cup D(v)$, and no
        ancestor appears as an internal vertex of any $P_I$.

  \item[Chordlessness.]
        Consider the cyclic order of vertices specified by the pattern $\Pi$, and
        modify it by inserting, for each $I \in J$, the internal vertices of the
        realized path $P_I$ in the natural order between its endpoints.
        Among the vertices of $G$ that appear on this partial cycle, we forbid any
        edge of $G$ that would become a chord of any cycle consistent with $\Pi$.
        This condition depends only on the cyclic order given by $\Pi$ and on the
        realized internal vertices, and is therefore independent of how the remaining
        $\bot$-positions are later filled.
\end{description}

For each state descriptor $(\Pi,J)$ at $v$, we store in the table at $v$ an arbitrary
subset of at most $\tau$ distinct solutions.
If there are fewer than $\tau$ solutions for $(\Pi,J)$, then all of them are stored.


Many state descriptors $(\Pi,J)$ are infeasible and thus admit no solutions. For example, an edge of $G$ between two ancestors would inevitably become
a chord for any cycle consistent with the pattern.

The total length of all paths in $\mathcal Q$ is at most $10$.
Thus every stored solution has constant size.
Because the height of $T$ is bounded by $f(10)$, the sets $A(v)$ also have constant
size, and the number of possible patterns and state descriptors at $v$ is bounded by
a constant.
Therefore, each table entry at $v$ can be encoded using $O(\log n)$ bits, and the
entire table at $v$ also admits an $O(\log n)$-bit encoding.

We denote by $\mathcal S(v)$ the dynamic programming table stored at vertex $v$.

In addition to $\mathcal S(v)$, we store at $v$ a value $\ell(v)$ defined as
\begin{align*}
\ell(v)
:= \min\Bigl\{
  10,\;
  |C|
  \;\Bigm|\;&
  C \subseteq A(v)\cup D(v),\\
  &C \text{ is a $G$-chordless and non-$G$-facial cycle in $\Lambda(G)$}
\Bigr\}.
\end{align*}
Our ultimate goal is to compute $\ell(r)$ for the root $r$ of $T$.

\subsubsection{Tables for prefixes of the children}


For a vertex $v \in V(T)$, let $\children(v)$ be the number of children of $v$, and
fix an arbitrary ordering
\[
  \child_1(v),\dots,\child_{\children(v)}(v).
\]
For $i \in \{1,\dots,\children(v)\}$, let
\[
  D_i(v) \;:=\; \bigcup_{j=1}^i D\bigl(\child_j(v)\bigr),
\]
so that $D(v) = \{v\} \cup D_{\children(v)}(v)$.
For each child $u = \child_i(v)$ we have
\[
  A(u) \;=\; A(v) \cup \{v\},
\]
and hence all children of $v$ share the same ancestor set and therefore the same
collection of state descriptors $(\Pi,J)$ in their
tables $\mathcal S(u)$.

For $i \in \{1,\dots,\children(v)\}$, we define a partial table $\mathcal S_i(v)$
indexed by the same state descriptors $(\Pi,J)$ as for the children of $v$.
For a fixed $(\Pi,J)$, the entry $\mathcal S_i(v)[\Pi,J]$ is a set of solutions
defined exactly as in the global table, with the only change that internal vertices
are restricted to $D_i(v)$:
each solution is a collection $\mathcal Q$ of paths that

\begin{itemize}
  \item realizes every interval in $J$ by a single path of the prescribed length in
        $\Lambda(G)$ between its endpoints in $A(v)\cup\{v\}$;
  \item uses only vertices of $D_i(v)$ as internal vertices, with endpoints in
        $A(v)\cup\{v\}$; and
  \item satisfies the same chordlessness condition with respect to the pattern $\Pi$
        as in the definition of $\mathcal S(v)$.
\end{itemize}

For each $(\Pi,J)$, the table $\mathcal S_i(v)$ stores at most $\tau$ distinct
solutions; if fewer than $\tau$ exist, all of them are stored.
Note that for $i=1$ the table $\mathcal S_1(v)$ coincides with the table of $\child_1(v)$ , and as $i$
increases we simply allow internal vertices to come from the union of the first $i$
child subtrees.

\paragraph{Partial cycle lengths.}

For $v \in V(T)$ and $i \in \{1,\dots,\children(v)\}$, we also define
\begin{align*}
\ell_i(v)
:= \min\Bigl\{
  10,\;
  |C|
  \;\Bigm|\;&
  C \subseteq A(v)\cup\{v\}\cup D_i(v),\\
  &C \text{ is a $G$-chordless and non-$G$-facial cycle in $\Lambda(G)$}
\Bigr\},
\end{align*}
with the convention that $\ell_i(v)=10$ if no such cycle exists.
Thus $\ell_i(v)$ is the length (capped at $10$) of the shortest relevant cycle that
can already be formed using $v$, its ancestors, and vertices in the subtrees of the
first $i$ children.
Later, after processing all children and the vertex $v$ itself, we will obtain
$\ell(v)$ from the values $\ell_i(v)$.

\subsubsection{Filling the tables}

We now explain how the tables are computed along the treedepth decomposition $T$.
We show that leaves can compute their tables locally, that the tables of the children
of a vertex $v$ can be merged sequentially to obtain the partial tables
$\mathcal S_i(v)$ and values $\ell_i(v)$, and that after all children of $v$ have
been processed, $v$ can incorporate itself to obtain $\mathcal S(v)$ and $\ell(v)$.
Throughout this discussion, we assume that when processing a vertex $v$, its local
knowledge includes:

\begin{itemize}
  \item The ancestor set $A(v)$.
  \item All edges of $H$ (both edges of $\Lambda(G)$ and edges of $G$) whose endpoints
        lie in $A(v)\cup\{v\}$.
\end{itemize}

\begin{lemma}[Base case]\label{lem-dp-base}
Each leaf $v \in V(T)$ can locally compute $\mathcal S(v)$
and $\ell(v)$.
\end{lemma}
\begin{proof}
If $v$ is a leaf, then $D(v) = \{v\}$.
By our assumptions on local knowledge, $v$ knows $A(v)$ and all edges of $H$ whose
endpoints lie in $A(v)\cup\{v\}$.
Since $A(v)$ has constant size, the induced subgraph of $H$ on $A(v)\cup\{v\}$ is also
of constant size.

For the table $\mathcal S(v)$, we simply go over all state descriptors $(\Pi,J)$ and,
for each, enumerate all collections of paths that could realize the intervals in $J$
using only internal vertices in $D(v)=\{v\}$.
Any such path has length at most $2$, and whether it exists and satisfies the
chordlessness condition depends only on the edges of $H$ induced by $A(v)\cup\{v\}$,
which are known to~$v$.
For each $(\Pi,J)$ we keep at most $\tau$ such collections.

For $\ell(v)$, any cycle contributing to the minimum is a $G$-chordless and
non-$G$-facial cycle in $\Lambda(G)$ of length at most $10$ contained in
$A(v)\cup\{v\}$.
Again, this is a constant-size induced subgraph that $v$ knows completely, so $v$ can
enumerate all simple cycles of length at most $10$, test the two properties, and take
the minimum length (or $10$ if none exist).
\end{proof}


\begin{lemma}[Merging children solutions]\label{lem-merge-children}
Let $v \in V(T)$ be a non-leaf. Let $u := \child_i(v)$, for some $i \in \{2,\dots,\children(v)\}$.
\begin{itemize}
    \item Given $\mathcal S_{i-1}(v)$ and $\mathcal S(u)$, vertex $v$ can locally
          compute $\mathcal S_i(v)$.
    \item Given $\ell_{i-1}(v)$, $\ell(u)$, $\mathcal S_{i-1}(v)$, and $\mathcal S(u)$,
          vertex $v$ can locally compute $\ell_i(v)$.
\end{itemize}
\end{lemma}

\begin{proof}
Recall that $A(u) = A(v) \cup \{v\}$, and all children of $v$ share the same ancestor
set, and hence the same collection of state descriptors $(\Pi,J)$ in their tables.

\paragraph{Computing $\mathcal S_i(v)$.}
Fix a state descriptor $(\Pi,J)$ at $v$.
To construct the entry $\mathcal S_i(v)[\Pi,J]$, we consider all partitions
\[
  J = J' \uplus J'',
\]
where $J'$ and $J''$ are (possibly empty) disjoint subsets of $\mathcal I(\Pi)$.
For each such partition, and for each pair of solutions
\[
  \mathcal Q' \in \mathcal S_{i-1}(v)[\Pi,J']
  \qquad\text{and}\qquad
  \mathcal Q'' \in \mathcal S(u)[\Pi,J''],
\]
we form the union
\[
  \mathcal Q := \mathcal Q' \cup \mathcal Q''.
\]
By construction, $\mathcal Q$ realizes exactly the intervals in $J$ (those in $J'$
via $\mathcal Q'$ and those in $J''$ via $\mathcal Q''$), all internal vertices lie
in $D_i(v) = D_{i-1}(v) \cup D(u)$, and all endpoints lie in $A(v)\cup\{v\}$.
Because there is no edge between $D_{i-1}(v)$ and $D(u)$, and both
$\mathcal Q'$ and $\mathcal Q''$ are already chordless with respect to the pattern
$\Pi$, no new chord of the pattern can be introduced by taking the union:
any edge of $G$ with both endpoints among the vertices of $G$ appearing in the
partial cycle was already present and already tested in one of the two subproblems.
Thus $\mathcal Q$ satisfies the same chordlessness condition and is a valid solution
for $(\Pi,J)$ with internal vertices in $D_i(v)$.

For each $(\Pi,J)$, we keep an arbitrary subset of at most $\tau$ such merged
solutions; if fewer than $\tau$ exist, we store all of them.
This defines $\mathcal S_i(v)$ from $\mathcal S_{i-1}(v)$ and $\mathcal S(u)$.

\paragraph{Computing $\ell_i(v)$.}
By definition, $\ell_i(v)$ is the minimum (capped at $10$) length of a
$G$-chordless and non-$G$-facial cycle $C$ in $\Lambda(G)$ contained in
$A(v)\cup\{v\}\cup D_i(v)$.
Such a cycle $C$ falls into one of three types:

\begin{itemize}
  \item $C$ is contained in $A(v)\cup\{v\}\cup D_{i-1}(v)$: then $|C|$ is accounted
        for in $\ell_{i-1}(v)$.
  \item $C$ is contained in $A(v)\cup\{v\}\cup D(u)$: then $|C|$ is accounted for
        in $\ell(u)$.
  \item $C$ uses vertices from both $D_{i-1}(v)$ and $D(u)$.
\end{itemize}

The first two cases are handled by taking
\[
  \min\{\ell_{i-1}(v),\; \ell(u)\}.
\]
We now explain how cycles of the third type are captured by the merged tables.

Fix a shortest $G$-chordless and non-$G$-facial cycle $C$ of the third type with
$|C|\le 10$.
Let $\Pi$ be the cycle pattern at $v$ obtained from the cyclic order of $C$ by
marking vertices in $A(v)\cup\{v\}$ explicitly and all other vertices by~$\bot$.
This pattern has length $m = |C| \in \{6,8,10\}$, and its intervals correspond to
subpaths of $C$ whose internal vertices lie strictly below $v$ in $T$.
Each such subpath is entirely contained in either $D_{i-1}(v)$ or $D(u)$, so we
obtain a partition
\[
  J = J' \uplus J''
\]
of the set $J \subseteq \mathcal I(\Pi)$ of intervals used by $C$, where $J'$ are
the intervals realized inside $D_{i-1}(v)$ and $J''$ those realized inside $D(u)$.
The subpaths of $C$ inside $D_{i-1}(v)$ and $D(u)$ together define solutions
\[
  \mathcal Q'_C \in \mathcal S_{i-1}(v)[\Pi,J']
  \qquad\text{and}\qquad
  \mathcal Q''_C \in \mathcal S(u)[\Pi,J''],
\]
in the ideal (untruncated) tables.

Since each interval of $\Pi$ has length at least $2$ and $|C|\le 10$, the set $J$
contains at most $5$ intervals.
By \Cref{lem:badpaths}, for any fixed pattern $\Pi$, partition $J=J'\uplus J''$, and
fixed choices of paths for all but one interval, there are at most $36$ paths for the
remaining interval that can participate simultaneously in a $G$-facial cycle of
length at most $10$.
Thus, if for every $(\Pi,J')$ and $(\Pi,J'')$ the number of solutions in
$\mathcal S_{i-1}(v)$ and $\mathcal S(u)$ is strictly less than $\tau = 36^5+1$, then
the particular solutions corresponding to the cycle $C$ are stored and will be merged
at $v$, so $C$ is explicitly represented and its length is taken into account.

Otherwise, suppose that for some state descriptor $(\Pi,J')$ or $(\Pi,J'')$ the
number of solutions reaches $\tau$.
Since $|J|\le 5$, by the pigeonhole principle there exists an interval for which
more than $36$ different paths are stored among these solutions.
No matter how the paths for the other intervals are chosen (from the other side and
from the remaining intervals), \Cref{lem:badpaths} guarantees that at least one of
these $>36$ candidates cannot participate in any $G$-facial cycle of length at most
$10$ together with the fixed choices.
In other words, even if the exact paths used by $C$ are not stored, the merged tables
still contain a combination of paths that yields a $G$-chordless cycle of length at
most $|C|$ that is not $G$-facial.
Hence, when $v$ inspects all merges of solutions in $\mathcal S_{i-1}(v)$ and
$\mathcal S(u)$ for the pattern $\Pi$ and all partitions $J=J'\uplus J''$, it will
find a cycle of length at most $|C|$ of the third type.
\end{proof}



\begin{lemma}[Children $\rightarrow$ parent]\label{lem-merge-parent}
Let $v \in V(T)$ be a non-leaf.
\begin{itemize}
  \item Given $\mathcal S_{\children(v)}(v)$, vertex $v$ can locally compute
        $\mathcal S(v)$.
  \item $\ell(v) = \ell_{\children(v)}(v)$.
\end{itemize}
\end{lemma}

\begin{proof}
In $\mathcal S_{\children(v)}(v)$, patterns use boundary vertices in
$A(v)\cup\{v\}$ and internal vertices in $D_{\children(v)}(v)=D(v)\setminus\{v\}$.
To obtain $\mathcal S(v)$ from $\mathcal S_{\children(v)}(v)$, it suffices to reinterpret $v$ as an
internal vertex. 
For each state descriptor $(\Pi,J)$, $v$ keeps at most $\tau$ solutions.

For the second claim, observe that
\[
  A(v)\cup D(v)
  = A(v)\cup\{v\}\cup D_{\children(v)}(v),
\]
so the definitions of $\ell(v)$ and $\ell_{\children(v)}(v)$ take the minimum (capped
at $10$) over exactly the same set of cycles.
Hence $\ell(v) = \ell_{\children(v)}(v)$.
\end{proof}





\subsection{Local certification}

 Now we prove \Cref{thm:planar-vc} by describing an $O(\log n)$-bit local certification
scheme to certify our dynamic programming algorithm.

\begin{proof}[Proof of \Cref{thm:planar-vc}]
It was already known~\cite{BFP21} that for $k \in \{2,3\}$, $k$-vertex-connectivity
can be certified with $O(\log n)$-bit labels.
Therefore, we may assume that the input planar graph $G$ is already certified to be
$3$-vertex-connected and focus on certifying whether it is $k$-vertex-connected for
$k \in \{4,5\}$.

Planar graphs have bounded degeneracy, so by {\color{red} some known technique},\yijun{note} we may
assign $O(\log n)$-bit labels to edges as well as to vertices without changing the
asymptotic label size.
We use edge labels only to encode local embedding information.

\paragraph{Certifying the embedding and the radial structure.}
We first certify a combinatorial embedding of $G$.
Following Esperet and Lévêque~\cite{esperet2022local}, the prover assigns labels that encode the circular
ordering of incident edges around each vertex and around each face, and a distinct
identifier to each face.
The local verifier checks that these circular orderings are consistent, that every
edge appears twice on face boundaries, and that Euler's
formula $|V(G)|-|E(G)|+|F(G)|=2$ holds.
The last check is carried out by aggregating the numbers of vertices, edges, and
faces along a spanning tree, whose correctness can itself be certified with
$O(\log n)$ bits.
If all checks succeed, the embedding is valid and uniquely determines the radial
graph $\Lambda(G)$ and the augmented graph $R(G)$ with vertex set
$V(G)\cup F(G)$ and edge set $E(\Lambda(G))\cup E(G)$.

\paragraph{Simulating faces.}
In $R(G)$, every face $f \in F(G)$ is a vertex adjacent to all vertices on
$\partial f$.
In the underlying network only the vertices of $G$ are present, so we simulate the
vertex $f$ by replicating its label on all vertices of $\partial f$.
These vertices check locally that they all store identical information for $f$ and
that the neighbors of $f$ in $R(G)$ are exactly the vertices of $\partial f$.
Thus the simulated vertex $f$ behaves like an ordinary vertex of $R(G)$ in all
subsequent checks.

\paragraph{Certifying treedepth decompositions.}
We color $R(G)$ with a low-treedepth coloring with parameter $p=10$, and obtain a
coloring $\varphi \colon V(R(G)) \to [k(10)]$.
For every choice of $10$ colors $X \subseteq [k(10)]$, we consider the induced
subgraph
\[
  K_X := R(G)\bigl[\varphi^{-1}(X)\bigr],
\]
and its connected components $H$.
By definition of low-treedepth colorings, each $K_X$ has treedepth at most $f(10)$,
which is a constant.

For each fixed $X$ and each component $H$ of $K_X$, the prover provides a treedepth
decomposition $T$ of $H$.
Each (real or simulated) vertex $v \in V(H)$ stores the following information:
\begin{itemize}
  \item The identity of its parent in $T$ (or a special symbol if $v$ is a root).
  \item Its depth in $T$.
  \item The ancestor set $A(v)$.
  \item The list of all edges of $H$ 
        whose endpoints lie in $A(v)\cup\{v\}$.
\end{itemize}
Because the height of $T$ is at most $f(10)$, each set $A(v)$ has constant size,
and the above information fits in $O(\log n)$ bits.
The standard local checks~\cite{feuilloley2022can} ensure that $T$ is a valid
treedepth decomposition of $H$, in particular that every edge of $H$ joins an
ancestor--descendant pair.

When $v$ corresponds to a face $f \in F(G)$, the vertices of $\partial f$ all store
the same treedepth label for $f$ and check consistency along $\partial f$.

\paragraph{Encoding the dynamic programming tables.}
For each component $H$ and its treedepth decomposition $T$, the prover simulates the
dynamic programming described earlier and stores its outcome in the certificates.

For every vertex $v\in V(T)$, the certificate of $v$ contains:
\begin{itemize}
  \item The table $\mathcal{S}(v)$ consisting of at most $\tau$ solutions for each
        state descriptor $(\Pi,J)$.
  \item The value $\ell(v)$.
\end{itemize}
If $v$ is a simulated face $f\in F(G)$, then this information is duplicated on all
vertices in $\partial f$.

In addition, for each face $f$ with children
\[
  \child_1(f),\dots,\child_{\children(f)}(f)
\]
ordered according to the circular order of $\partial f$, the certificates on
$\partial f$ also store the partial tables $\mathcal{S}_i(f)$ and values $\ell_i(f)$
for all $i\in\{1,\dots,\children(f)\}$.
Each vertex of $\partial f$ stores the records corresponding to the prefixes that end
at its position in the cyclic order.
Vertices on $\partial f$ check consistency of these records along the boundary.


\paragraph{Local verification of the dynamic programming.}
We now explain how the local verifier checks that the stored tables and values are
consistent with the dynamic programming.

\begin{itemize}
  \item For each leaf $v$ of $T$, the verifier at $v$ recomputes $\mathcal{S}(v)$ and
        $\ell(v)$ from its local view of $A(v)\cup\{v\}$ and the edges of $H$ induced
        by this set.
        This is exactly the situation of \Cref{lem-dp-base}.
        If the recomputed values differ from the stored ones, then $v$ outputs
        $\reject$.
  \item For each non-leaf $v$ and each child $u=\child_i(v)$, the verifier checks that
        the merge step of \Cref{lem-merge-children} is correctly implemented.
        We distinguish two cases.
        If $v\in V(G)$, then $v$ does not store the partial tables
        $\mathcal{S}_{i-1}(v)$ and $\mathcal{S}_i(v)$ explicitly: instead, it
        reconstructs them on the fly from the tables of its children and from its
        local view of $A(v)\cup\{v\}$ and the edges induced by this set using the merging rules
        of \Cref{lem-merge-children}.
        If $v$ is a face $f\in F(G)$, then the partial tables
        $\mathcal{S}_i(f)$ and values $\ell_i(f)$ are distributed among the vertices
        of $\partial f$, ordered according to the circular order on $\partial f$; each
        vertex on $\partial f$ checks that its local piece of the partial tables and
        the pieces stored by its neighbors on $\partial f$ together implement the
        merge step prescribed by \Cref{lem-merge-children}. In particular, the consistency check for the partial tables $\mathcal{S}_i(f)$ and
        $\ell_i(f)$ is performed by $\child_i(f) \in \partial f$.
        If any of these consistency checks fails, then the corresponding vertex
        outputs $\reject$.

  \item For each non-leaf $v$, the verifier checks that
        $\mathcal{S}(v)$ is obtained from $\mathcal{S}_{\children(v)}(v)$ and that
        $\ell(v)=\ell_{\children(v)}(v)$, as in \Cref{lem-merge-parent}.
        If this fails, then $v$ outputs $\reject$.
\end{itemize}
 

\paragraph{Aggregation.}
For each color set $X \subseteq [k(10)]$ of size $10$ and each connected component
$H$ of $K_X$, the preceding checks ensure that the labels correctly describe the
execution of the dynamic program on $(H,T)$.
In particular, for the root $r_H$ of $T$, the value $\ell(r_H)$ is the length capped
at $10$ of the shortest $G$-chordless and non-$G$-facial cycle in $\Lambda(G)$
contained in $H$.

To combine these values, we use a spanning tree of $G$ certified with $O(\log n)$
bits.
Along this spanning tree, we aggregate, for each $X$, the minimum of the values
$\ell(r_H)$ over all components $H$ of $K_X$, and then take the minimum over all
$X$.  

Let $L^\star$ be the global minimum value, which equals the 
minimum, capped at $10$, of the lengths of all $G$-chordless and non-$G$-facial
cycles in $\Lambda(G)$.
By \Cref{thm:kappa-radial}, the vertex connectivity of $G$ is equal to $L^\star/2$.

\paragraph{Final local decision.}
The parameter $k\in\{4,5\}$ is fixed in advance.
Each vertex compares $L^\star$ with $2k$.
If $L^\star \ge 2k$, then the vertex outputs $\accept$.
If $L^\star < 2k$, then the vertex outputs $\reject$.

\paragraph{Completeness.}
Suppose that $G$ is planar and $k$-vertex-connected with $k\in\{4,5\}$.
The prover chooses the following:
\begin{itemize}
  \item A valid combinatorial embedding certificate for $G$.
  \item A low-treedepth coloring of $R(G)$ with parameter $p=10$.
  \item For every $10$-color set $X$ and component $H$ of $K_X$, a treedepth
        decomposition $T$ of $H$.
  \item The tables $\mathcal{S}(v)$, $\ell(v)$ produced by the dynamic programming
        on $(H,T)$.
  \item For faces, the partial
        tables $\mathcal{S}_i(f)$, $\ell_i(f)$ produced by the dynamic programming
        on $(H,T)$.
  \item A spanning-tree aggregation certificate showing that $L^\star$ is the minimum
        of all $\ell$-values.
\end{itemize}
All local checks then succeed, and \Cref{thm:kappa-radial} implies that
$L^\star \geq 2k$, so every vertex outputs $\accept$.

\paragraph{Soundness.}
Suppose that $G$ is not $k$-vertex-connected.
If $G$ is not $3$-vertex-connected, then the separate scheme of~\cite{BFP21} already
forces some vertex to output $\reject$, independently of the labels used here.
We may thus assume that $G$ is $3$-vertex-connected but has vertex connectivity
$\kappa(G) < k$.

By \Cref{thm:kappa-radial}, there exists a $G$-chordless and non-$G$-facial cycle
$C\subseteq\Lambda(G)$ with $|C| = 2\kappa(G) < 2k$.
This cycle uses at most $10$ vertices of $R(G)$, so all its vertices receive colors
within some $10$-element set $X$.
Hence $C$ is contained in the induced subgraph $K_X$ and in some component $H$ of
$K_X$.

If all local embedding and treedepth checks pass, and if all dynamic-programming checks
pass, then the stored tables coincide with the result of a correct execution of the
dynamic programming on $(H,T)$, and the root $r_H$ must satisfy
\[
\ell(r_H) \le |C| < 2k.
\]
Consequently, the global aggregation must satisfy $L^\star \le \ell(r_H) < 2k$.
In that case, every vertex outputs $\reject$ in the final comparison step.

If the prover assigns certificates that are inconsistent with the embedding,
the low-treedepth coloring, the treedepth decomposition, or the dynamic
programming recurrences, then at least one local check fails and some vertex outputs
$\reject$.
Thus no assignment of $O(\log n)$-bit certificates can make all vertices output
$\accept$ when $G$ is not $k$-vertex-connected.
\end{proof}



==> prel-PODC_vers.tex <==
\section{Preliminaries}\label{sec:Pre}
\yx{some notes: only keep the standard edge-certification lemmas and BFS certification here. Put others in the corresponding section.
}

Throughout the paper, we use $\tilde{O}(\cdot)$, $\tilde{\Omega}(\cdot)$, and $\tilde{\Theta}(\cdot)$ to suppress factors of the form $\log^{\pm O(1)} n$, where $n$ denotes the number of vertices in the original graph $G$. We also use a subscript $k$ to suppress factors depending only on $k$, writing $O_k(\cdot)$, $\Omega_k(\cdot)$, and $\Theta_k(\cdot)$. For example, the bound $O(k^3 \sqrt{n} \log^{2.5} n)$ can be expressed as $\tilde{O}_k(\sqrt{n})$.

\subsection{Local certification}\label{sec:Pre-LocalCert}
We mainly follow the definitions of the local certification scheme in \cite{BFZ25, Feu21}.


%Consider a family $\Fcal$ of labeled graphs, where vertices are equipped with some inputs from the label set $L$. 
%\yx{i changed a bit since we don't really specify the label set in the following section?}
Consider a family $\Fcal$ of (possibly labeled) graphs. In this paper, we consider $\Fcal$ to be a subset of all connected graphs. A local certification scheme allows vertices to verify some property $\Pcal$ using only their local views. It can be described as an external prover and a verifier. The prover puts some certificates on each vertex, and the verifier, which is a distributed algorithm, decides whether to accept locally.

There are several models of local certification. In this paper, we consider the \emph{proof labeling scheme}. Each vertex in the graph is associated with a unique identifier (ID) of length $O(\log n)$. A \emph{certificate assignment} of $G$ of length $s$ is a mapping from $V(G)$ to the set of $s$-bit strings. The \emph{view} of a vertex consists of all information in its neighborhood (including itself), including the induced graph topology and certificate assignments of these vertices, as well as the inputs and ID of itself. The \emph{verifier} takes as input the view of a vertex and outputs accept or reject.


%There are several models of local certification. In this paper, we consider the \emph{locally checkable proofs}. Each node in the graph is associated with a unique identifier (ID) of length $O(\log n)$. A \emph{certificate assignment} of $G$ of length $s$ is a mapping from $V(G)$ to the set of $s$-bit strings. The \emph{view} of a vertex at distance $r$ consists of all information about its $r$-hop neighborhood (including itself), including the induced graph topology, certificate assignments, and the inputs and IDs of these vertices. The \emph{verifier} takes as input the view at distance $r$ of a vertex and outputs accept or reject. Here $r$ is said to be the \emph{local horizon} of the verifier. In this paper, we only consider verifiers of local horizon $1$.


The property $\Pcal$ that we want to certify should be independent of IDs. We say that $\Pcal$ admits a \emph{certification scheme} of size $s$ if there exists a verifier that satisfies \emph{completeness} and \emph{soundness}:

\begin{itemize}
    \item \emph{completeness}: For any $n$-vertex graph $G\in\Pcal$, and any ID assignment of $G$, there exists a certificate assignment of size $s(n)$ such that all vertices output accept.
    \item \emph{soundness}: For every $G\not\in\Pcal$, for every ID assignment of $G$, for any certificate assignment of any size, there exists at least one vertex that outputs reject.
\end{itemize}

{\color{red} 
In the \emph{edge certification scheme}~\cite{BFP21, FFM+23}, the setting is the same as in a proof-labeling scheme, except that a certificate assignment of length $s$ for a graph $G$ is a mapping from $V(G) \cup E(G)$, rather than only $V(G)$, to the set of $s$-bit strings. Accordingly, the view of each vertex is enlarged to include the certificates assigned to its incident edges. We will adapt some results from the edge certification scheme to the proof-labeling scheme and use them as building blocks for our main algorithms.
}

%think how to write this paragraph
In the literature, there is another form of local certification called \emph{locally checkable proofs}. Locally checkable proof is similar to the proof-labeling scheme described above, except that the view of a vertex may consist of all information about its $r$-hop neighborhood (including itself), including the induced graph topology, certificate assignments, and the inputs and IDs of these vertices. The verifier\mtt{verifier has been defined, so we do not need to emphasize it again while we use it.}\yx{edited} takes as input the view at distance $r$ of a vertex and outputs accept or reject. Here $r$ is said to be the \emph{local horizon} of the verifier.

Although we focus on proof labeling schemes in this paper, our lower bounds also work in the locally checkable proofs with local horizon $r=1$. \mtt{Is the proof labeling scheme exactly locally checkable proofs with $r=1$? I am not sure why we need this paragraph.}\yx{also in the locally checkable proof, each vertex sees the id of its neighbors (in the proof-labeling scheme only labels)}
Also, when we talk about a proof labeling scheme of size $\Omega(\log n)$, we can assume for simplicity that the view of each vertex contains the IDs of its neighbors, as otherwise the prover can always write the ID of a vertex in its own certificate and let the vertex verify the consistency.
%Although we focus on proof labeling schemes in this paper, our lower bounds also work in the locally checkable proofs, where vertices have access to their neighbors' IDs. Also, when we talk about a proof labeling scheme of size $\Omega(\log n)$, we can assume for simplicity that the view of each vertex contains the IDs of its neighbors, as otherwise the prover can always write the ID of a vertex in its own certificate and let the vertex verify the consistency.

%In the literature, there is another form of local certification called \emph{locally checkable proofs}. Locally checkable proof is similar to the proof-labeling scheme described above, except that the view of a vertex may consist of all information about its $r$-hop neighborhood (including itself), including the induced graph topology, certificate assignments, and the inputs and IDs of these vertices. The \emph{verifier} takes as input the view at distance $r$ of a vertex and outputs accept or reject. Here $r$ is said to be the \emph{local horizon} of the verifier.


{\color{orange} There are other related models of local certification, such as non-deterministic local decision, where the certificates should not depend on the identifier assignments, and the anonymous model, where the vertices are not equipped with identifiers. See~\cite{Feu21, BFZ25} and the references therein for more discussion on these models.} \mtt{This paragraph looks redudant to me.}\yx{now we have lower bound for 1-vc in the anonymous model, so need to think hos to give the background here.}

\subsubsection{Edge certification and degeneracy}\label{sec:Pre-EdgeCert}
\yx{I change the order of the subsection of certifying spanning tree with the edge certification scheme and remove the definition for edge-certification scheme there (leave the one after defining local certification scheme.)}

%In this paper, we also work on a variant of the certification scheme described above, called \emph{edge certification scheme}~\cite{BFP21, FFM+23}, proposed by~\cite{FFM+23}. 
%under the name \emph{line proof labeling scheme}.\yx{i don't know whether to mention this since i want to use the name edge certification as in BFP21}\mtt{I guess no.} 
%Edge certification scheme is a proof labeling scheme where the prover can put the certificates on both vertices and edges, and the verifier at a vertex is allowed to take not only its certificates and the certificates assigned on the adjacent vertices, but also the certificates on the incident edges. This model is also a commonly used building block for designing vertex certification, see~\cite{BFP21, FFM+23} for more applications.
%\yx{should we remove the definition of edge-certification in this paragraph, and in the description after definition of local certification scheme, we refer to this subsubsection for properties of edge certification scheme?}


{\color{red}Edge certification scheme is a commonly used building block for designing vertex certification. In the following, we state two well-known results for transforming edge-certification schemes to vertex-certification in restricted graph classes. See~\cite{BFP21, FFM+23} for more applications.}
For bounded-degree graphs with maximum degree at most $\Delta$, we can transform any edge certification to a vertex certification with only a constant blow-up. The idea is to do a $2$-hop coloring on the vertices, and for each vertex, assign a copy of the certificate on each incident edge, along with the color on the other endpoint of that edge. Then each vertex knows which edge each certificate belongs to. See also~\cite[Proposition 4]{BFVZ26}.
%\yx{for bounded degree graph, need to cite the DISC submission}
\begin{lemma}\label{lem: edge-cert-bdd-deg}
    Consider an edge certification of size $f(n)$ for a graph family $\Fcal$. If $\Fcal$ has bounded degree $\Delta$, then there exists a (vertex) certification of size {\color{red}$O(\Delta (f(n)+\log\Delta))$}.
\end{lemma}

%For bounded-degree graphs, we can transform any edge certification to a node certification with only a constant blow-up. The idea is to do a $2$-hop coloring on the vertices, and for each node, assign a copy of the certificate on each incident edge, along with the color on the other endpoint of that edge. Then each node knows which edge each certificate belongs to.
%\begin{lemma}\label{lem: edge-cert-bdd-deg}
    %Consider an edge certification of size $f(n)$ for a graph family $\Fcal$. If $\Fcal$ has bounded degree $\Delta$, then there exists a (node) certification of size $O(f(n))$.
%\end{lemma}

{\color{red}A similar result has been established for sparse graphs with bounded degeneracy. The \emph{degeneracy} of a graph $G$ is defined to be the minimum number $k$ where $G$ admits an ordering of the vertices such that every vertex has at most $k$ neighbors that are earlier in the ordering. Note that if a graph is of bounded degeneracy, then the number of edges is linear in the number of vertices. Such ordering also provides an edge-orientation of the graph where every vertex has a bounded out-degree. After certifying such an orientation, each vertex takes the responsibility of carrying the certificates on its incident outgoing edges. By doing so, one can ``re-distribute'' the certificates on edges to the vertices uniformly.} The following Lemma gives a transformation from edge certification to vertex certification on bounded-degeneracy graphs.

%For bounded-arboricity graphs, one can also ``re-distribute'' the edge certificates to the vertices with lower degree. The following Lemma gives a transformation from edge certification to vertex certification on bounded-arboricity graphs.

%\begin{lemma}[{\cite{FFM+23}}]\label{lem:EdgeCert-degeneracy}
%    Consider an edge certification of size $f(n)$ for a graph family $\Fcal$. If $f(n)\in\Omega(\log n)$ and $\Fcal$ has bounded degeneracy $d$, then there exists a (vertex) certification of size $d\cdot f(n)$.
%\end{lemma}
\begin{lemma}[{\cite{FFM+23}}]\label{lem:EdgeCert-degeneracy}
    Consider an edge certification of size $f(n)$ for a graph family $\Fcal$. If every graph in $\Fcal$ has degeneracy at most $d$, then there is a (vertex) certification of size $O(d ( f(n)+\log n))$.
\end{lemma}


\yx{Now all the background of kVC is here in the prel, but other than that we mentioned the tools in the corresponding section, should we unify this?}


\subsubsection{Certifying BFS spanning tree}
\begin{lemma}[{\cite{KKP05}}]\label{lem: BFS-cert}
    Let $G$ be a connected graph. Certifying a BFS spanning tree can be done in $O(\log n)$ bits.
\end{lemma}
%It is known that certifying a BFS spanning tree can be done in $O(\log n)$ bits~\cite{KKP05,CHPP20}. Let $G=(V,E)$ be a connected graph. We briefly describe the certification scheme of a BFS spanning tree on $G$:
\begin{proof}
For completeness, we briefly describe the certification scheme and its verification procedure.
    \begin{itemize}
        \item Pick any vertex $r\in V$ to be the root. For each vertex $v\in V$, the certificate $c(v)$ contains three fields $(r, p(v), \dist(v,r))$, where $r$ is the root's $\ID$, $p(v)$ is the parent's $\ID$, and $\dist(v,r)$ is the distance from $v$ to root $r$.
        \item The verification process contains the following parts:
        \begin{itemize}
            \item (All distances are consistent.) Each vertex $v$ checks that the distance from each of its neighbors to the root differs from itself by at most $1$. That is, for each $u\in N(v)$, $\dist(u,r)\in\{\dist(v,r)-1,\dist(v,r),\dist(v,r)+1\}$. 
            \item (There exists a root.) Each vertex $v$ with $\dist(v,r)>0$ checks that its parent is closer to the root. This can be done using $p(v)$ in the certificate of $v$, and $\dist(\cdot,v)$ in the certificates of its neighbors. 
            \item (The root is unique.) Each vertex checks that all its neighbors receive the same root $\ID$. For vertex $v$ such that $\dist(v,r)=0$, $v$ itself is the root. Therefore, we have $v$ check that $r=\ID(v)$.\qedhere
        \end{itemize}
    \end{itemize}
\end{proof}
%Using this scheme, one can certify a spanning forest on a (not necessarily connected) graph $G$ by certifying a spanning tree on each connected component of $G$.
%\yx{I remove certifying spanning forest here as we no longer use it?}


\subsection{Graph connectivity}
Let $G$ be a graph and $r$ be a vertex of $G$. Two spanning trees $T$ and $T'$ of $G$ are said to be \emph{independent} if for any vertex $v$ in $G$, the $v$--$r$ path in $T$ and the $v$--$r$ path in $T'$ are internally vertex-disjoint. We say that $G$ admits $k$ independent spanning trees rooted at $r$ if there exist $k$ spanning trees of $G$ rooted at $r$, say $T_1,\ldots,T_k$, that are pairwise independent.

For $k=4$, it is known that $4$-vertex-connectivity is equivalent to having $4$ independent spanning trees rooted at every vertex.
\begin{lemma}[\cite{CLY06}]
    Let $G$ be a $4$-vertex-connected graph, and let $r\in V(G)$. Then there exist four independent spanning trees of $G$ rooted at $r$.
\end{lemma}

Itai and Zehavi~\cite{ZI89} conjectured that the equivalence also holds for $k\geq 5$.
\begin{conjecture}[{Itai--Zehavi conjecture~\cite{ZI89}}]\label{conj: Itai--Zehavi}
    A graph $G$ is $k$-vertex-connected if and only if for every vertex $r\in V(G)$, there exist $k$ independent spanning trees rooted at $r$.
\end{conjecture}
%Itai--Zehavi conjecture implies that a graph $G$ is $k$-vertex connected if and only if there exist $k$ different vertices $r_1,\ldots,r_k$ in $G$ such that for each $i\in [k]$, there exist $k$ independent spanning trees rooted at $r_i$. Indeed, if we can remove fewer than $k$ vertices to disconnect the graph, this cut separates at least one of the vertices in $\{r_i : i \in [k]\}$ from some vertex $x \notin \{r_i : i \in [k]\}$. This yields a contradiction since $x$ and $r$ are connected by $k$ internally disjoint paths.
{\color{red}We note that, by a simple observation, the }
Itai--Zehavi conjecture implies that a graph $G$ is $k$-vertex-connected if and only if there exist $k$ distinct vertices $r_1,\ldots,r_k \in V(G)$ (rather than all vertices) such that, for each $i \in [k]$, $G$ contains $k$ independent spanning trees rooted at $r_i$. Suppose that $G$ contains such roots but is not $k$-vertex-connected, then there exists a vertex cut $C$ with $|C|<k$ such that $G-C$ is disconnected. Since $C$ has size less than $k$, it cannot contain all of $r_1,\ldots,r_k$, so some root $r^*$ remains in $G-C$. {\color{red}Since $G-C$ is disconnected, there exists a vertex $x$ that belongs to a component of $G-C$ different from the one containing $r^*$ }
%Let $x$ be a vertex in a component of $G-C$ different from the one containing $r^*$. 
This contradicts the existence of $k$ independent spanning trees in $G$ rooted at $r^*$, which implies that there are $k$ internally vertex-disjoint paths between $r^*$ and $x$, and hence no vertex cut of size less than $k$ can separate them.


%\mtt{This implication may need a short explanation.}
%\yx{edited}


\subsection{Heavy-light decomposition}
\begin{definition}[{Heavy-light decomposition~\cite{SLEATOR1983362_heavy-light}}]
    The heavy-light decomposition of a rooted tree $T$ is a partition of its edges into heavy and light edges, such that each non-leaf vertex has one heavy edge to one of its children, which is the child with the largest number of vertices in its subtree.
\end{definition}
The heavy edges in $T$ induce a set of paths, called \emph{segments}. {\color{red}Each leaf in $T$ that is not adjacent to any heavy edge is treated as a segment of length $0$.} 
%For each leaf in $T$ that is not adjacent to any heavy edge, treat it as a segment of length $0$. 
This way, each vertex belongs to exactly one segment.
\begin{fact}\label{fact: heavy-light_fact_0}
    Consider any vertex in the tree $T$, the root-to-$v$ path can overlap with at most $O(\log n)$ segments.
\end{fact}


\subsection{Two-party communication complexity}
\paragraph{The Set-Disjointness problem}
Let $x,y\in\{0,1\}^s$ be two $s$-bit strings, each of which can be viewed as an indicator vector of a set. We say that $x$ and $y$ are not disjoint if and only if there exists an index $i\in[s]$ such that $x_i=y_i=1$. The truth value of whether $x$ and $y$ are disjoint is denoted as $\DISJ(x,y)$. The two-party communication problem of Set-Disjointness ($\DISJ$) is defined as follows. Two players called Alice and Bob, are given inputs $x,y\in\{0,1\}^s$ respectively, and they communicate via a deterministic protocol to decide whether $\DISJ(x,y)=\true$ or $\DISJ(x,y)=\false$. The cost of a given protocol is the worst-case number of bits that the players need to communicate when using this protocol. The communication complexity of $\DISJ$ is the minimum cost among all the protocols.

\paragraph{Nondeterministic communication complexity}
In a nondeterministic protocol, each player receives, in addition to its input, an advising string provided by a third party that sees both the inputs of Alice and Bob. We say that the nondeterministic protocol solves some Boolean function $f$ if the following holds:
\begin{itemize}
    \item For each $\true$-instance, there exists an advising string such that the players output \accept.
    \item For each $\false$-instance, for any advising string, some player outputs \reject.
\end{itemize}
The cost of a nondeterministic protocol is the worst-case length of the advising string. The nondeterministic communication complexity of $f$ is the minimum cost among all the nondeterministic protocols that solve $f$.

For example, the nondeterministic communication complexity of $\overline{\DISJ}$ is $O(\log s)$ as we can pick the advising string to be the index $i$ where $x[i]=y[i]=1$. Each player can check that the $i$-th bit of their input is indeed $1$.

In contrast, it is known that the nondeterministic complexity of $\DISJ$ is $\Omega(s)$.
\begin{fact}[{\cite{Kushilevitz_Nisan_1996}}]\label{fact: DISJ-com}
    The nondeterministic communication complexity of $\DISJ(x,y)$ is $\Omega(s)$.
\end{fact}

The nondeterministic communication complexity has been widely used to obtain lower bounds for local certification schemes~\cite{GS16, CHPP20, FFH+21}.



%When applying to proving the lower bounds for the local certification scheme, we consider the \emph{nondeterministic communication complexity}, which is defined as follows: Let $f:X\times Y\to\{0,1\}$ be a Boolean function. Alice is given input $x\in X$ and Bob is given input $y\in Y$. A prover (a third party) that sees both the inputs $x$ and $y$ provides an \emph{advising string} $p$ to both Alice and Bob. Each player then decides whether to accept based on its input and the proof $p$. The protocol is said to compute an output $z\in\{0,1\}$ of the function $f$ if $f(x,y)=z$ if and only if there exists a proof that both Alice and Bob accept. The nondeterministic communication complexity of $f$ and the output $z$ is the worst-case length of the proof.

%{\color{red} As I checked, the literature of the local certification scheme often uses the auxiliary string definition. Here, I use the definition in the book {Communication Complexity for Algorithm Designers}}


%\yijun{this paragraph is not clear enough to me... after reading it I still don't understand the meaning of the nondeterministic communication complexity. Maybe make it a bit more precise?}



==> sparse_cert.tex <==
\section{Sparse certificate for $k$-connectivity}
In this Section, we provide a local certification for sparse certificates for $k$-edge-connectivity (or $k$-vertex-connectivity).

Let $G=(V,E)$ be a graph, a \emph{certificate} for $k$-edge-connectivity ($k$-vertex-connectivity, resp.) of $G$ is a subset of edges $E'\subseteq E$ such that the subgraph induced by $E'$, $G'=(V,E')$ is $k$-edge-connected ($k$-vertex-connectivity, resp.) if and only if $G$ is $k$-edge-connected ($k$-vertex-connectivity, resp.).

It has been shown that for both $k$-edge-connectivity and $k$-vertex-connectivity, there exists a certificate of arboricity at most $k$~\cite{NI92,CT90}.

Let $G$ be a graph. A BFS (breadth-first search) spanning forest of $G$ contains a BFS spanning tree for each connected component on an arbitrary root.

\begin{lemma}[\cite{NI92,CT90}]\label{lem: sparse-cert-iff}
    Let $G=(V,E)$ be a graph, and for $i=1,\ldots,k$, let $F_i$ be the edge set of a BFS spanning forest of $G\setminus(\cup_{j=1}^{i-1}F_j)$. Then $\cup_{i=1}^k F_i$ is a certificate for both $k$-edge-connectivity and $k$-vertex-connectivity. 
\end{lemma}

\paragraph{Certifying the sparse certificate of $k$-connectivity.}
In this section, we show that there exists a compact local certification scheme for certifying the sparse certificate of $k$-connectivity.

\lemSparseCert*
%\begin{lemma}\label{lem: sparse-cert}
    %There exists an $O(k\log n)$-bit local certification scheme for a sparse certificate of both $k$-edge-connectivity and $k$-vertex-connectivity.
%\end{lemma}
\begin{proof}
    According to \Cref{lem: sparse-cert-iff}, to certify a sparse certificate of $k$-edge-connectivity or $k$-vertex-connectivity, we need to certify a BFS spanning forest iteratively. Let $E_i=E\setminus(\cup_{j=1}^{i-1}F_j)$ be the remaining edge after removing the first $i-1$ BFS spanning forests, and let $G_i=(V,E_i)$ be the graph induced by $E_i$. For each $i=1,\ldots,k$, we certify a BFS spanning tree on each connected component of $G_i$ using \Cref{lem: BFS-cert}. Denote the certificate assigned to node $v$ on $G_i$ by $c_i(v)=(r_i,p_i(v),\dist_i(v,r_i))$.

    The certification for the sparse certificate of both $k$-edge-connectivity and $k$-vertex-connectivity is just the combination of the $k$ BFS spanning trees certification on graphs $G_1,\ldots,G_k$, $c(v)=(c_1(v),c_2(v),\ldots,c_k(v))$. Each node then iteratively verifies that $c_i(v)$ is a certificate of a BFS spanning forest on $G_i$ by running the verification algorithm in %\Cref{lem: sparse-cert} 
    \cref{lem: BFS-cert} \mtt{This citation was broken. Please check whether this fix is correct. }
    pretending that the edges $\{\{v,p_j(v)\}\}_{j=1}^{i-1}$ are not present in the graph.
\end{proof}

As a corollary, we obtain a local certification scheme for $3$-vertex-connectivity using $O(\log n)$ bits, which improves the result of~\cite{BFP21}.

In~\cite{BFP21}, they proved that certifying $3$-vertex-connectivity can be done in $O(\log n)$ bits on vertices and $O(1)$ bits on edges.
\begin{lemma}[{\cite[Corollary 24]{BFP21}}]\label{lem: 3-vc-prev}
    $3$-vertex-connectivity can be certified with $O(\log n)$ bits on vertices and $O(1)$ bits on edges.
\end{lemma}

\corThreeVC*
\begin{proof}
    We first apply the local certification scheme for a sparse certificate of $3$-vertex-connectivity described in \Cref{lem: cert-sparse-cert} using $O(\log n)$ bits. The sparse certificate has arboricity $3$, and we apply the local certification scheme described in \Cref{lem: 3-vc-prev} to the sparse certificate by transforming it into a local certification scheme using $O(\log n)$ bits on vertices, according to \Cref{lem:EdgeCert-degeneracy}.
\end{proof}
